SE(3)-Equivariant Robot Learning and Control: A Tutorial Survey

Recent advances in deep learning and Transformers have driven major breakthroughs in robotics by employing techniques such as imitation learning, reinforcement learning, and LLM-based multimodal perception and decision-making. However, conventional deep learning and Transformer models often struggle to process data with inherent symmetries and invariances, typically relying on large datasets or extensive data augmentation. Equivariant neural networks overcome these limitations by explicitly integrating symmetry and invariance into their architectures, leading to improved efficiency and generalization. This tutorial survey reviews a wide range of equivariant deep learning and control methods for robotics, from classic to state-of-the-art, with a focus on SE(3)-equivariant models that leverage the natural 3D rotational and translational symmetries in visual robotic manipulation and control design. Using unified mathematical notation, we begin by reviewing key concepts from group theory, along with matrix Lie groups and Lie algebras. We then introduce foundational group-equivariant neural network design and show how the group-equivariance can be obtained through their structure. Next, we discuss the applications of SE(3)-equivariant neural networks in robotics in terms of imitation learning and reinforcement learning. The SE(3)-equivariant control design is also reviewed from the perspective of geometric control. Finally, we highlight the challenges and future directions of equivariant methods in developing more robust, sample-efficient, and multi-modal real-world robotic systems.

==> Old/Section2_RelatedWorks.tex <==
\subsection{Group Equivariant Neural Networks}\label{genn}
Convolutional neural networks are advantageous due to their translation-equivariant property. However, these equivariant properties are not guaranteed for other geometric symmetries, such as rotation or reflection. To address this limitation and extend CNNs to a broader range of symmetries, Group-equivariant Convolution Neural Networks (G-CNNs)\cite{cohen2016group} are proposed. They introduce the group equivariant convolution layer $\Phi: X \to Y$, which satisfies the condition $\Phi(\rho_X(g) \cdot x)=\rho_Y(g) \cdot \Phi(x)$, where $x \in X$, $y \in Y$. Here $\rho_X(g)$ and $\rho_Y(g)$ are group representations of the group $G$, satisfying $\rho(gh)=\rho(g)\rho(h)$, $\forall g, h \in G$. The convolution (i.e., correlation) in G-CNNs can be divided into the lifting convolution, which is the first layer convolution, and the full Group convolution (G-convolution). Lifting and full G-convolution can be represented as follows:
% \JS{We use $\rho(g)$ for the group representation, so please change accordingly, but it seems that the other also needs to be unified. What we should use is actually define space, $x \in X$, $y \in Y$, and use notation $\rho_X(g)$, $\rho_Y(g)$, with $\Phi: X \to Y$. In this notation, $\rho_X(g)$ is representation of group element $g$ acting on the set $X$.} \HA{Revised all the notation correctly.}
%
\[
\begin{split}
    y(g) &= \sum_{x \in X} \W (g^{-1} \circoo x) f(x), \quad 
    \text{Lifting convolution} \\
    y(g) &= \sum_{g \in G} \W (g^{-1} \circoo g) f(g), \quad 
    \text{Full G-convolution} \\
\end{split}
\]
%
Where $\W$ and $f$ are kernels and feature maps, respectively. In the case of G-CNNs, the process of lifting correlations results in high-dimensional feature maps, which increases the computational cost and makes it challenging to handle groups with high dimensions.
% \JS{what is ``large'' group? The meaning is very unclear. Is the large for computational power or a number of dimensions?} 
% \HA{Revised clearly.} 
% \JS{Too long sentence and hard to understand->} \HA{Revised for easy understanding, more details will be updated.} 
To address this issue, Steerable CNNs \cite{cohen2016steerable} utilize the fact that the space of the feature map is a vector space. They do not use lifting correlations, instead using kernels as linear maps between the input features and output features. To ensure that the output feature is steerable, the kernels are designed with the constraint such that $\rho_{out}(g) \W = \W \rho_{in}(g)$. Since the equivariance constraint is linear in $\W$, the kernel space forms a vector space as well.

G-CNNs and Steerable CNNs introduced equivariant neural networks for discrete groups in two-dimensional space. 
% \JS{Does steerable CNN also assume discrete group action in the 2D image?} \HA{They mentioned it is possible to develop in a more general setting, but for simplicity, they only consider steerability with respect to discrete groups.} 
In the field of robotics, however, many applications involve transformations in three-dimensional space, raising the necessity of network designs that can accurately represent transformations in three-dimensional space. Tensor Field Networks (TFNs) \cite{thomas2018tensor} address this issue using SE(3)-equivariant graph neural networks specifically designed for the SE(3) group. These networks can represent rigid body transformations in three-dimensional space with point clouds as input. \JS{We first keep the TFN and SE(3)-transformer here without much description. There are more details in the later sections, but let's merge them after reformatting.} The convolution process in TFN is formulated as:
\[
\begin{split}
{f}_{(out)}&( {x}|\dX)=\int{d^3 {y}} \; {W}( {x}- {y}) {f}_{(in)}( {y}|\dX)
\end{split}
\]

SE(3)-transformers \cite{se3t} enhance the TFN by incorporating self-attention mechanisms into their convolution process: 
\[
\begin{split}
    {f}_{(out),i}=\sum_{j\neq i}\alpha_{ij} {W}( {x}- {x}_j) {f}_{j}+\bigoplus_{n'}^{N'}\sum_{n=1}^{N} {W}_{(S)}^{n'n} {f}_{j}^{(n)}
\end{split}
\]
\JS{The details of the TFN and SE(3)-transformer will be elaborated in the later section after introducing the required concepts.}

\subsection{Imitation Learning}\label{il}
The equivariant neural networks in section \ref{genn} can be utilized for symmetry in robot manipulation tasks. Recently, numerous robot learning researchers have leveraged symmetry in SE(3) \cite{zeng, huang2022equivariant, fourtran, ndf, ryu2022equivariant, ryu2024diffusion}.  NDFs\cite{ndf} implements object representation with a category-level descriptor using Vector Neurons \cite{deng2021vector}, but NDFs requires pre-trained object segmentation. On the other hand, EDFs\cite{ryu2022equivariant} achieves local equivariance by utilizing the locality of Equiformer\cite{liao2022equiformer} and SE(3)-Transformer\cite{se3t}. This enables EDFs to perform end-to-end training without pre-training and object segmentation. Furthermore, EDFs introduces a bi-equivariant energy-based model on SE(3) for the pick and place problem. The bi-equivariant energy-based model on SE(3) is written as :
\[
P(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) = \frac{\exp{[-E(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp})]}}{Z}
\]
\[
Z = \int_{SE(3)} dg \exp[-E(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp})]
\]
where $P$ is an energy-based model on the $\text{SE}(3)$ manifold, $E$ is an energy function and $g = (p, R) \in \text{SE}(3), p \in \Real^3, R \in \text{SO}(3)$.
By addressing the equivariance both on the scene and the grasp, EDFs could achieve high sample efficiency and robustness for out-of-distribution data. The bi-equivariance condition of the model can be written as follows: 
\[
\begin{split}
P(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) &= P(\Delta g_w g | \Delta g_w \cdot \mathcal{O}^{scene},\mathcal{O}^{grasp}) \\
&= P(g \Delta g_e^{-1}|\mathcal{O}^{scene}, \Delta g_e \cdot \mathcal{O}^{grasp})
\end{split}
\]
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/bi_equiv_ed.jpg}
    \caption{Bi-equivariance. (a) The scene equivariance and (b) grasp equivariance consider the transformation of world and grasped object. The end-effector pose should be transformed equivariantly with the transformation.}
    \label{fig:biequiv}
\end{figure}
The energy-based model consists of $SE(3)$-equivariant type-$l_n$ vector field generated by observation.
\[
E(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) =
\]
\[
\int_{\mathbb{R}^3} d^3 x \; \rho(x|\mathcal{O}^{grasp})||\varphi(gx|\mathcal{O}^{scene})-D(R)\psi(x|\mathcal{O}^{grasp}) ||^2
\]
\\
Diffusion-EDFs\cite{ryu2024diffusion} improved training time of EDFs, maintaining end-to-end training manner and data-efficiency utilizing the bi-equivariance and locality of robotic manipulation. Diffusion-EDFs proposed a bi-equivariant score function given as follows:
\[
s(\Delta g g | \Delta g \cdot \mathcal{O}^{scene}, \mathcal{O}^{grasp}) = s(g | \mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
\[
s(g\Delta g^{-1}|\mathcal{O}^{scene}, \Delta g \cdot \mathcal{O}^{grasp}) = [\Ad_{\Delta g}]^{-T}s(g | \mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]

\[
\quad \Ad_g = \begin{bmatrix}
            R & \hat{p} R \\
            0 & R
            \end{bmatrix}\\
\]
where $R \in \text{SO}(3)$, $p \in \Real^3$ and $\hat{p}$ is the skew-symmetric matrix of $p$.
Diffusion-EDFs split the score model into translation and rotational parts and propose the models of each part satisfying equivariance conditions.
\[
s_t(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) = [s_{\nu;t}\oplus s_{\omega ; t}](g|\mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
\[
s_{\nu ; t}(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) =
\]
\[
 \int_{\mathbb{R}^3} d^3 x \; \rho_{\nu ; t}(x|\mathcal{O}^{grasp})\Tilde{s}_{\nu ; t}(g, x|\mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
\[
 s_{\omega ; t}(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) =
\]
\[
\int_{\mathbb{R}^3} d^3 x \; \rho_{\omega ; t}(x|\mathcal{O}^{grasp})\Tilde{s}_{\omega;t}(g, x|\mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
\[
+ \int_{\mathbb{R}^3} d^3 x \; \rho_{\nu ; t}(x|\mathcal{O}^{grasp})x \wedge \Tilde{s}_{\nu;t}(g, x|\mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
The details of  bi-equivariant score model and diffusion-based learning on the SE(3) manifold for visual robotic manipulation are provided in Diffusion-EDFs.

RiEMann\cite{girolami2011riemann} is the near real-time SE(3)-equivariant robot manipulation framework. RiEMann learns an affordance map with one type-0 vector field to get a point cloud ball $B_{ROI}$ with SE(3)-Transformer \cite{se3t}.
\[
f_{in}(x) = \bigoplus_{i=0}^{3}f_0^{i}(x)
\]
The region is extracted from the affordance map with predefined radius. This leads to reduction of computation complexity and memory usage. Position and orientation network use the points in the region. RiEMann designed the output feature of translation and rotation matrix with 1 type-0 vector field and 3 type-1 vector field each.
\[
f_{out}(x) = f_0(x) + \bigoplus_{j=0}^{3}f_1^j(x)
\]

Fourier Transporter \cite{fourtran} proposed SE(3) bi-equivariant model using 3D convolutions and a Fourier representation of rotation for pick and place problems. 
Similar to EDFs \cite{ryu2022equivariant} and Diffusion-EDFs \cite{ryu2024diffusion} the proposed method utilize coupled SE($d$)$\times$SE($d$)-symmetries for the problem. 
Let's assume $d = 3$, the 3D pick and place problem. The policy for pick and place is formulated as $p(a_t|o_t) = p(a_{place}|o_t, a_{pick})p(a_{pick}|o_t)$. 
The SE(3)-equivariant pick network is a function $f_{pick} : o_t \mapsto p(a_{pick}|o_t)$, where $p(a_{pick}|o_t)$ is a steerable field. 
The base space of the steerable field determines the pick location $\Real^3$, and the fiber space encodes the distribution of pick orientations $\text{SO}(3)$. We can represent the distribution $p(a|o_t)$ as $\Real^3 \rightarrow \{\text{SO}(3) \rightarrow \Real \}$. Especially, $L_g(p)(h) = p(g^{-1} \circ h)$ is the transformation of the distribution with left-action. $L_g$ notation is a left-regular representation of group element $g$ to distribution, and $\circ$ is a group action of $g$ with respect to $h$ -- See Sec.~\ref{sec:left_regular_representation} for the details.

The pick pose distribution should follow a transformation on observation.
\[
f_{pick}(g\cdot o_t) = \text{Ind}_{\rho_L}(g) f_{pick}(o_t), \quad \forall g \in \text{SE}(3)
\]
The action of $g$ via representation $\rho$ on steerable feature vector fields $f$ is defined as $\text{Ind}_{\rho}(g)(f)(x) = \rho(g)\cdot f(\rho_1 (g)^{-1} x)$. $\rho(g)$ is the fiber action which transforms the pick orientation and the base space action $\beta (g)f(x) = f(\rho_1 (g)^{-1}x)$ rotates the pick location. The standard representation $\rho_1$ of $\text{SO}(3)$ for one group element is a standard $3 \times 3$ rotation matrix . The irreducible representation $\rho_1$ of $\text{SO}(3)$ is the Wigner D-matrix $D^1 (\alpha, \beta , \gamma)$, a $3 \times 3$ matrix when expressed in terms of Euler angles. \JS{I believe $D^1(\alpha, \beta, \gamma)$ is a standard rotation matrix with $\alpha, \beta, \gamma$ notation. - Please check and confirm this.} The grasped object can be represented as a voxel patch centered on the pick location with the assumption that the object does not move or deform. The place network is $f_{place}: (c, o_t) \to p(a_{place}|o_t, a_{pick})$ where $c$ is the cropped image centered at the pock location. The network should satisfy the bi-equivariance constraint in the pick and place problem. 
\[
\begin{split}
    &f_{place}(g_1 \cdot c, g_2 \cdot o_t) = \text{Ind}_{\rho_L}(g_2)\rho_{R}(g_1^{-1})f_{place}(c, o_t), \\
    &\forall g_1, g_2 \in \text{SE}(3)
\end{split}
\]

The place action should transform equivariantly with actions on the picked object and actions on the observation. The template matching method is used to realize place symmetry. The cross correlation between a dynamic kernel $\kappa(c)$ and a feature map $\phi(o_t)$ is used for pick action probability as $f_{place}(c, o_t) = \kappa(c) \star \phi(o_t)$, where $\star$ denotes the cross-correlation.

The dynamic kernel $\kappa(c)$ is introduced and utilized to perform convolutions on the Fourier space. The dynamic kernel is composed of dense feature maps, which are lifted with a finite number of rotations and Fourier transforms to the channel space. The dense feature map of crop $c$ is  $\psi(c)$. We rotate the dense feature map with a finite number of rotations $\Tilde{G} = \{g_i | g_i \in \text{SO}(3)\}_{i=1}^m$ and stack the rotated feature maps. The stack of fully rotated signals can be defined as follows:
% A stack of rotated feature maps 
\[
\begin{split}
    &\mathcal{L}^{\uparrow}[f](x) = \{ f(g_1^{-1}x), f(g_2^{-1}x) \dots , f(g_m^{-1}x)\},\\
    &\forall x \in \mathbb{R}^n , g_i \in \Tilde{G},
\end{split}
\]
The stack of fully rotated dense feature maps of the cropped image is $\mathcal{L}^{\uparrow}(\psi(c))$.

The Fourier transform over $\text{SO}(3)$ is defined as $\mathcal{F}(f) = (\hat{f}^l)_{l=0}^{\infty}$ where 
\[
\forall g \in \text{SO}(3), \quad f(g) = \sum_{l=0}^{\infty}\sum_{k,k'=-l}^{l}\hat{f}^l_{kk'}D^l_{kk'}(g)
\]
and $f : \text{SO}(3) \rightarrow \Real$, $D^l$ are the Wigner D-matrices.
Let $\mathcal{F}^{+}$ denote Fourier transform to the channel-space. Then, $\mathcal{F}^{+}$ is applied to $\mathcal{L}^{\uparrow}(\psi(c))$ . Finally, the dynamic kernel becomes $\kappa (c) = \mathcal{F}^{+} [\mathcal{L}^{\uparrow} (\psi(c))] $.

The cross correlation between the feature map $\phi(o_t)$ and the dynamic kernel $\kappa(c)$ is performed in the Fourier space. The place network is bi-equivariant if the $\psi(c)$ and the $\phi(o_t)$ satisfy the equivariant property and $\kappa(c)$ is a steerable convolutional kernel with $\rho_0$-type input. The details of SO(3)-Fourier Transform and proof of propositions are provided in Fourier Transporter \cite{fourtran}.

\subsection{Equivariant Reinforcement Learning}\label{rl}
\begin{figure}%[h!]
  \centering
\includegraphics[width=.8\linewidth]{Figures/GinvMDP.png}
  \caption{\textbf{Group-invariant MDP}. In a robot manipulation task, if the reward is 1 when the gripper achieves the goal, the group invariant MDP preserves the reward function and transition probability invariance under group actions.}
  \label{gimdp}
\end{figure}
Reinforcement learning (RL) is a powerful method, especially for robotics, due to its adaptability to complex and unpredictable environments, ability to achieve optimal policies through trial and error, and scalability to high-dimensional state and action spaces. However, RL has notable limitations, one of which is its sample inefficiency due to extensive trial and error from scratch. This inefficiency can be mitigated by utilizing group equivariance. This approach has shown promise in RL, as demonstrated in prior works that successfully combine these methods
\cite{rl1, rl3, finzi2021residual, theile2024equivariant, wang2022so, kohler2023symmetric, wang2022robot, wang2022equivariant, nguyen2023equivariant, tangri2024equivariant}.\\

Many equivariant reinforcement learning methods are based on the fundamental concept of group-invariant Markov decision process (MDP) \cite{wang2022so}, denoted as $\mathcal{M}_G=(S,A,P,R,G)$. 
% \JC{Added how the contraction is enabled}
It is based on the MDP homomorphisms \cite{ravindran2001symmetries, ravindran2004approximate}, a mapping that relates the original MDP, $M=(S,A,P,R,\gamma)$, to another abstract MDP, $M'=(S',A',P',R',\gamma)$. This homomorphism consists of two subjective functions $\alpha: S\rightarrow S'$ and $\beta: A\rightarrow A'$, which relate the state and action space of $M$ to the corresponding abstractions in $M'$. The policy in $M'$ can be utilized to derive a corresponding policy in $M$, which is given by:
\[
\begin{split}
    \pi(a|s)=\frac{\pi'(a'|\alpha(s))}{|\beta^{-1}(a')|}
\end{split}
\]
where $s\in S, a\in A, a'\in A'$ and $\pi'$ is the policy from the abstract MDP $M'$. Previous work has shown that if the abstract policy $\pi'$ is optimal, it can be used to derive the optimal policy in the original MDP, $M$ \cite{ravindran2001symmetries}.
Moreover, when the homomorphism follows a group framework, the optimal policy derived from the group-transformed MDP can be mapped back to induce the optimal policy in the original MDP. This approach leverages the symmetry within the problem to improve learning efficiency. The group-invariant MDP maintains its properties under the group-invariance of both the transition probability and the reward function, which can be expressed as:
\begin{itemize}
    \item Reward function: $R(s,a) = R(\rho_s(g) s,\rho_a(g)a)$
    \item Transition probability: \\
    \hspace*{\fill}
    $P(s'|s,a)=P(\rho_s(g)s'|\rho_s(g)s,\rho_a(g)a)$
\end{itemize}
where $g$ represents the group action in any group $G$. Due to the invariances, the optimal $Q$ function $Q^*(s,a)$ also becomes group-invariant and the optimal policy $\pi^*(s)$ is equivariant, which can be expressed as:
\begin{itemize}
    \item Q function: $Q^*(s,a)=Q^*(\rho_s(g)s,\rho_a(g)a)$
    \item Policy: $\pi^*(\rho_s(g)s)=\rho_{a}(g)\pi^*(s)$
\end{itemize}

Consider the Bellman optimality equation: 
\[
Q^*(s,a)=R(s,a)+\gamma\; \sup_{a'}\int_{s'}ds'P(s'|s,a)Q^*(s',a').
\]
Then, $Q^*$ of the transformed state-action pair, i.e., \\$Q^*(\rho_s(g)s', \rho_a(g)a')$ is given as:\\
\[
\begin{split}
    &Q^*(\rho_s(g)s,\rho_a(g)a)=R(\rho_s(g)s, \rho_a(g)a)\\ &+\gamma\; \sup_{a'}\int_{s'}ds'P(\rho_s(g)s'|\rho_s(g)s,\rho_a(g)a)Q^*(\rho_s(g)s', \rho_a(g)a').
\end{split}
\]
The reward function and transition probabilities are group-invariant, we can reindex the integral by setting $s'=\rho_s(g)s''$. Under the re-indexing, the optimal $Q^*$ function for the transformed state-action pair can be rewritten as 
\[
\begin{split}
    &Q^*(\rho_s(g)s,\rho_a(g)a)=R(\rho_s(g)s, \rho_a(g)a)\\
    &+\gamma\;\sup_{a'}\int_{s'}ds'P(\rho_s(g)s'|\rho_s(g)s, \rho_a(g)a)Q^*(\rho_s(g)s', \rho_a(g)a')\\
    &=R(s, a)+\gamma\;\sup_{a'}\int_{s'}ds'P(s'|s, a)Q^*(\rho_s(g)s', \rho_a(g)a')
\end{split}
\]
Introducing a new function $\bar{Q}(s,a)=Q(\rho_s(g)s, \rho_a(g)a)$, it follows that 
\[
\begin{split}
    \bar{Q}^*(s,a)=R(s, a) +\gamma\;\sup_{a'}\int_{s'}ds'P(s'|s, a)\bar{Q}^*(s', a')
\end{split}
\] Note that $Q^*(s,a)=Q^*(\rho_s(g)s, \rho_a(g)a)$ by the uniqueness of the Bellman optimal equation. Now, consider the optimal policy $\pi$ that maximizes $Q^*(s,a)$: $\pi^*(s)=\arg\max_{a}Q^*(s,a)$. One can relate this to the transformed state $\rho_s(g)s$. The policy in the transformed state is given by: 
\[
    \pi^*(\rho_s(g)s)=\arg\max_{a}Q^*(\rho_s(g)s,a)
\]
Using the fact that $Q^*(\rho_s(g)s,a)=Q^*(s,\rho_a(g^{-1})a)$, as implied from the uniqueness of the Bellman equation, we can rewrite: 
\[
    \pi^*(\rho_s(g)s)=\arg\max_{a}Q^*(s,\rho_a(g^{-1})a).
\] 
Letting $a=\rho_a(g)\bar{a}$, the equation can be expressed as: 
\[
\begin{split}
    \pi^*(\rho_s(g)s)&=\rho_a(g) \arg\max_{\bar{a}}Q^*(s,\rho_a(g^{-1})\rho_a(g)\bar{a})\\
    &=\rho_a(g)\pi^*(s)
\end{split}    
\]

Based on the group-invariant MDP, the authors in the prior work \cite{wang2022so} propose $SO(2)$-equivariant $Q$ learning methods. To construct group-invariant and equivariant layers for group-invariant vision-based $Q$ networks, they employ the networks from \cite{weiler2019general}, which encode the equivariant constraint on the kernel to achieve the equivariance. Using these equivariant networks, they construct equivariant networks for Deep $Q$-Networks (DQN), and both group-invariant critics and equivariant policies for Soft Actor-Critic (SAC). Experimental results demonstrate that the equivariant RL achieves superior sample efficiency compared to vanilla Q-learning methods, even when data augmentation or the auxiliary methods \cite{laskin2020reinforcement, kostrikov2020image, laskin2020curl} are employed. Additionally, the prior work shows better generalization over the group actions, outperforming other methods when given a fixed orientation of the input image rather than a random orientation.\\ 

In another prior work \cite{kohler2023symmetric} build upon the work by \cite{wang2022so} to propose an equivariant policy for the visual-force problems. Their approach utilizes the force input in addition to the visual input to facilitate equivariant policy learning. Experimental results demonstrate that their proposed method outperforms the baseline approaches. Furthermore, an ablation study reveals that incorporating additional sensory inputs, such as force or proprioception, enhances sample efficiency and performance, although this improvement is task-dependent. Finally, they also show that even when visual input quality is poor, the force input can compensate for it.\\

In \cite{nguyen2023equivariant}, the authors extend the equivariance to partially observable Markov decision process (POMDP), denoted as $\mathcal{P}_G=(S,A,P,R,\Omega,O,b_0)$. Here, $S,A,P,$ and $R$ represent the state space, action space, transition probability, and reward function, respectively, which are equivalent to those in $\mathcal{M}_G$. However, $\mathcal{P}_G$ includes additional components: $\Omega$, which denotes the observation space; $O$, the stochastic observation function; and $b_0$ the initial belief. The reward function $R$ and the transition probability $P$ adhere to the definitions in $\mathcal{M}_G$. Moreover, $\mathcal{P}_G$ introduces group-invariant conditions in the observation and initial belief:
\begin{itemize}
    \item Observation function: $O(\rho_a(g)a, \rho_s(g)s',\rho_o(g)o)$
    \item Initial belief: $b_0(\rho_s(g)s)=b_0(s)$
\end{itemize}

They also define that the history $h_t=(o_0,a_0,...,a_{t-1},o_t)$ maintains the invariant property under the group action $g\in G$, such that $\rho_h(g)h_t=(\rho_o(g)o_0,\rho_a(g)a_0,...,\rho_o(g)o_t)$. With these group-invariant properties in $\mathcal{P}_G$, they demonstrate that the optimal value function $V^*(h)=V^*(\rho_h(g)h)$ exhibits a similar group-invariant property, $V^*(h)=V^*(\rho_h(g)h)$, and that the optimal policy $\pi^*$ has an equivariant property, $\pi^*(\rho_h(g)h)=\rho_{\pi}(g)\pi^*(h)$. Utilizing their novel equivariant actor-critic architecture, they prove the performance of their method through simulations, showing it outperforms non-equivariant methods. Additionally, they validate their approach in a real hardware setting by successfully transferring the policy trained in simulation to the hardware in a zero-shot manner.\\

Equivariant networks have also been applied to offline reinforcement learning \cite{tangri2024equivariant}. This work leverages equivariant networks within specific methods like Conservative Q-Learning \cite{kumar2020conservative} and Implicit Q-Learning \cite{kostrikov2021offline} and addresses the challenge of outperforming the behavior policy used to generate the offline datasets. Through simulations involving robot manipulation tasks, they show their approach's enhanced sample efficiency and performance.


==> Old/Section3_Preliminaries.tex <==
\subsection{Group}
A group is defined by a set $\G$ along with a group product (a binary operator) $``\cdot"$  
that satisfies  the axioms:
\begin{itemize}
\item $\forall h, g \in \G$ we have $h \cdot g \in \G$ (Closure);
\item  $\exists \Id \in \G$  such that $\Id \cdot g = g \cdot \Id =  g$ (Identity); 
\item 
$\forall g \in \G$, $\exists$  $g^{-1} \in \G$ such that
$g^{-1} \cdot g = g\cdot g^{-1}= \Id$ (Inverse);
\item  $\forall g, h, f\in \G$ we have $(g \cdot h) \cdot  f = g\cdot (h\cdot f)$ (Associativity).
\end{itemize}

The translation group consists of the set of translation vectors in $\mathbb{R}^n$ equipped with the group product and inverse given by $g_1 \cdot g_2 = x_1 + x_2$ and $g^{-1}=(-x)$, for group elements $g_1=(x_1)$, and $g_2=(x_2)$.
The general linear group over $\Real$, denoted by  $GL(n, \mathbb{R})$ consists of the set of $n \times n$ matrices with real entries that can be inverted  $GL(n,\mathbb{R}):= \{ A \in \mathbb{R}^{n \times n} |\det (A) \neq 0\},$
together with the operation of matrix multiplication. With a stronger restriction that the determinant be positive real numbers, we have  $GL^+(n, \mathbb{R}):= \{ A \in \mathbb{R}^{n \times n} |\det (A) >0\}$, which is a subgroup of $GL(n, \mathbb R)$. A subgroup is a subset of a group $(H \subseteq G)$, which is itself a group that is closed under
the group operation of $G$.
 The unitary group is a  subset of $GL(n,\mathbb{C})$ that consists of  unitary matrices    
$U(n):=\{A \in \mathbb{C}^{n \times n} | AA^* = {\Id}\} \subset GL (n,\mathbb C),$
together with the matrix multiplication. The orthogonal group consists of  real matrices    
$O(n):=\{A \in \mathbb{R}^{n \times n} | AA^T = {\Id}\}$.
With an additional constraint $\det (R)=+1$, the orthogonal group forms the rotation group, i.e., a special orthogonal group denoted by $G=SO(n)$. It is a Lie group\footnote{A Lie group is a continuous group that is also a
differentiable manifold.} that consists of the set of rotation matrices 
$\{ R \in \mathbb{R}^{n \times n} | R^TR=RR^T={\Id}, \det (R)=+1 \},$
  together with the group
product and inverse are given respectively by the matrix product and inverse 
  $g_1 \cdot g_2 := (R_1 R_2)$,  $g^{-1}:= (R^{-1})$ for $g_1=(R_1)$ and $g_2 = (R_2)$.
We now introduce the rotation-translation group, i.e., a special Euclidean motion group denoted by 
$G=SE(n)$. It consists of the set  $\mathbb{R}^n \times SO(n)$ of translation vectors in  $\mathbb{R}^n$ and rotations in $SO(n)$, together with the group product and inverse given respectively by
$g_1 \cdot g_2 = (R_1x_2 + x_1, R_1R_2)$ and  $g^{-1}=(-R^{-1}x, R^{-1}),$
where $g_1=(x_1,R_1)$ and $g_2=(x_2, R_2)$.

\subsection{Smooth Manifolds}
Note that knowledge of smooth manifolds is not mandatory for understanding geometric deep learning and geometric control. However, as the concept of smooth manifolds provide fundamental theoretical background, we include them for the completeness of the paper.
\begin{figure}[!t]
\centering
\resizebox{\columnwidth}{!}{
\input{Figures/Tangent_vectors.tex}
}
\caption{Tangent vectors in a coordinate chart}
\label{fig:Chart}
\end{figure}

\subsubsection{Tangent and Cotangent Spaces} The tangent space $T_pM$ at a point $p$ on a smooth manifold $M$ is defined as the set of all tangent vectors to $M$ at $p$.  $T_pM = \{v \in M : v\text{ is a tangent vector to }M\text{ at }p\}.$
The elements of the tangent space are tangent vectors. Assume that there is a coordinate chart on $M$ with local
coordinates $(x^1, \cdots, x^n)$. The set of derivations  $\{ \frac{\partial }{\partial x^1}, \cdots, \frac{\partial }{\partial x^n} \}$ then form a basis
for $T_pM$, i.e.,
\[
X_p=\sum_{i=1}^nX^i\frac{\partial }{\partial x^i} = X^i\frac{\partial }{\partial x^i}.
\]
where $X^i$ is the component of the tangent vector $X_p$ at $p$ along the derivation $\frac{\partial }{\partial x_i}$.
In the second term of the equation, we have eliminated the summation sign by following the so-called Einstein convention:  if the same index name (such as $i$ in the expression above) appears exactly twice in any monomial term, once as an upper index and once as a lower index, that term is understood to be summed over all possible values of that index, generally from 1 to the dimension of the space in question. We also interpret that an upper index in a denominator becomes a lower index, i.e. the index $i$ in $\frac{\partial }{\partial x^i}$ is considered a lower index.

% For any linear operation $f : X \rightarrow Y$ over vector spaces $X$ and $Y$,  define its dual such as $f^*:Y^*\rightarrow X^*$, with the property: \JS{Lacks too much details, what is $X^*$ and $Y^*$? A dual space of $X$ and $Y$ I guess, but what is dual space? Inner product not defined}
% \[
% \langle y, f(x) \rangle = \langle f^* (y), x \rangle, \quad \forall x \in X,  y \in Y^*
% \]

The cotangent space $T^*_pM$ at a point $p$ on a smooth manifold $M$ is defined as the dual space of the tangent space at $p$, i.e.,  
${\displaystyle T_{p}^{*}\!{{M}}=(T_{p}{{M}})^{*}}$.
It consists of all linear functionals on the tangent space at $p$. i.e., 
%, and is also a vector space over $\mathbb{R}$, i.e.,
$T^*_pM = \{\alpha : T_pM \rightarrow \mathbb{R}, \; \alpha\text{ is linear}\}.$
The element  of $T_p^{*}M$ are called
a dual vector, cotangent vector or, in the context of differential
forms, a one-form at $p$.
%
% cotangent vectors,  tangent covectors, or just covectors, or  one-forms,  at $p$.
The action of a cotangent vector $\alpha_p \in T_p^*M$ on a tangent
vector $X_p\in T_pM$ is denoted by $  \alpha_p, (X_p)  .$ The dual basis   for $T_p^*M$ are given by
$\{dx^1, \cdots, dx^n\}$, and their actions on the  the basis for $T_p M$ are
\[
 dx^i \left ( \frac{\partial }{\partial x_j} \right )   =\delta^i_j = 
 \left \{ \begin{array}{cc} 1 \:\:\mbox{if} \:\: i=j\\ 0 \:\:\mbox{if}\:\: i\ne j\end{array} \right ., \:\:\quad i, j = 1, \cdots, n.
\]
An arbitrary one-form $\alpha_p$ at point $p$ is written as $\alpha_p= \alpha_i dx^i,$ were again we are following the Einstein summation convention. Therefore,
\[
\alpha_p(X_p) = \alpha_i dx^i ( X^j \frac{\partial}{\partial x^j}) = \alpha_i X^i\,.
\]


Given a smooth function $f: M \rightarrow \Real$, the action of the tangent vector $X_p$ on $f$ is 
\[
X_p(f) = X^i \left . \frac{\partial f(x)}{\partial x_i} \right |_{p}\,.
\]
The differential of $f$, $df_p  = \left . \frac{\partial f(x)}{\partial x_i} \right |_{p} dx^i\in T^*_p M$  satisfies
\[
 df_p(X_p) = X_p(f), \quad X_p \in T_p M.
\]



The tangent
bundle of $M$, denoted by $TM$, is defined as the disjoint union of the tangent spaces at all
points of $M$  such as 
\[TM=\bigsqcup_{p \in M} T_p M,\]
where $\sqcup$ is a disjoint union of sets. The tangent bundle comes equipped with a natural projection map $\pi : T_p M \to M$, which sends each vector in $T _p M$ to the point $p$ at which it is tangent: $\pi(X_p) = p$.
Similarly, the cotangent bundle of $M$ is denoted by   $T^*M$.

% \subsubsection{Differential Forms} 
% \JS{Push forward and pull back is yet to be defined.}
% A smooth differential one-form on a manifold $M$ is a smooth map $\alpha: M \rightarrow T^*M$ with $\pi \circoo \alpha=\Id$ 
% where $\pi : T^*M \rightarrow M$ is the canonical projection. A differential form is represented in local coordinates.
% \[
% \alpha(x)= \alpha_1(x) dx_1+ \cdots + \alpha_n(x) dx_n,
% \]
% where each $\alpha_i$ is a smooth function on $M$.

% Let $\F:M \rightarrow N$ be a smooth mapping and $\beta: N \rightarrow T^*N$ a smooth differential one-form on $N$. We can define a new one form $\alpha: M \rightarrow T^* M$ by
% \[
% \langle \alpha_p, X_p \rangle= \langle (\F^* \beta)_p, X_p \rangle=\langle \beta_{\F(p)}, \F_{*p} X_p \rangle,
% \]
% where  $\alpha:=\F^* \beta$ is called the pullback of $\beta$.



% A simple example of a one-form is the differential $df$ of
% a smooth function $f: M \rightarrow \Real$. 
% %The action of a vector $V$ on $f$ is $V [f]$ =$V_i \frac{\partial f}{ \partial x_i} \in \Real$.
% The action of $df \in T_p^*M$ on $X \in T_p M $ is defined by
% \[
% \langle df, X \rangle = X[f] = X_i \frac{\partial f}{ \partial x_i} \in \Real.
% \]

\subsubsection{The differential of a smooth map} Suppose $M$ and $N$ are smooth manifolds. Let $\F: M \rightarrow N$ be smooth and be a diffeomorphism. Also, let $f: N \to \Real$ be also smooth.
Given  ${\displaystyle p \in M,}$ the differential of 
$\F$  at 
$p$
is a linear map
 \[ {\displaystyle d\F _{p}\colon \ T_{p}M\to T_{\F (p)}N\,}\]
from the tangent space of 
$M$ at 
$p$ (i.e., $T_{p}M)$
 to the tangent space of 
$N$ at 
${\displaystyle \F (p)}$ (i.e., $T_{\F (p)}$) which satisfies
\[
dF_p(X_p)(f) = X_p(f \circ F)
\]
The differential $d\F_p$, is  the best linear approximation of $\F$ near $p$. 
Let $(x^i, \cdots , x^n)$ and $(y^i, \cdots, y^n)$ be respectively  local coordinates of  manifolds  $M$ and $N$. Then the action of $dF_p(X)$ can be expressed in local coordinates as
\begin{equation}
\label{eq:pushforward_coordinates}
dF_p(X_p) =  \left . \left ( \frac{\partial F^j(x)}{\partial x^i} X^i  \right ) \right |_p  \left . \frac{\partial}{\partial y^j} \right |_{F(p)} \:\: \in T_{F(p)}N\,.
\end{equation}
and, for $f : N \to \Real$,
\[
dF_p(X_p)(f) =  \left . \left ( \frac{\partial F^j(x)}{\partial x^i}  X^i \right ) \right |_p  
 \left . \frac{\partial f(y)}{\partial y^j} \right |_{F(p)}  \in \Real\,.
\]





% With  $\F: M \rightarrow N=\Real$, we have a differential that is a cotangent vector $d\F(p) \in T^*_pM$ by
% \[
% \left \langle d\F(p), X_p \right \rangle= X_p (\F), \quad X_p \in T_p M.
% \]
% Assume the local coordinate $x=(x_1, \cdots, x_n)$ for a chart $(\phi, U)$ with $x=\phi(p)$, the differential $d\F$ can be shown as
% \[
% d\F(x)= \frac{\partial \F }{\partial x_1}(x) dx_1 + \cdots + \frac{\partial \F }{\partial x_n}(x) dx_n.
% \]
 
%  The cotangent map of $F$ at $p$ is the linear map $F_p^*: T_{\F(p)}^* N \rightarrow T^*_{p} M$ defined by
%  \[
%  \langle \alpha_{\F(p)}, \F_{*p} X_p\rangle = \langle \F^*_p \alpha_{\F(p)}, X_p \rangle, 
%  \]
% where $\alpha_{\F(p)} \in T^*_{\F(p)} N$ and $X_p \in T_p M.$
% %$T^*_p \F$ denotes the cotangent map of $F$ at $p.$
% The cotangent map of $F$ at $p$ is denoted by $F^*_p$ (or sometimes by $dF_p^*$)  and is called pullback by $F$ at $p$.

% \JS{When $N$ is not $\mathbb{R}$}

\subsubsection{Vector Fields} A smooth vector field $X$ on a manifold $M$ is defined as a smooth map $X: M \rightarrow TM$
 with $\pi \circoo X= \Id$, where $\pi: TM \rightarrow M$ is the previously defined projection map. Let $\mathfrak{X}(M)$ be the set of all smooth vector fields on $M$.
A vector field can be expressed in terms of the local coordinate basis  of a chart $(\phi, U)$ as
\[
X_p= X^i(p) \left . \frac{\partial }{\partial x_i} \right |_p %+ \cdots + X_n(x) \frac{\partial }{\partial x_n},
\]
where each $X^i$ is a smooth function on an open ball of $x=\phi(p)$ 
(see Fig.~\ref{fig:Chart}).


% Let $X$ and $f \in C^{\infty}(M)$ be a smooth vector field and a smooth function on $M$, respectively. \JS{Notation inconsistency} The Lie derivative of $f$ with respect to $X$ is defined as $Xf: M \rightarrow \Real$ by 
% $ Xf(p)=X_p f.$
% With a  coordinate chart $(\phi,U)$ and $X=\sum_{i=1}^{n} X_i(x) \frac{\partial }{\partial x_i}$, we have
% \[
% Xf(x)=\sum_{i=1}^{n} \frac{\partial f}{\partial x_i} \bigg |_{x=\phi(p)} X_i(x).
% \]

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{./Figures/Pushforward} 
\vskip -0.5pc
\caption{The pushforward of the vector field X. 
}\label{fig:Pushforward}
\end{center}
\vskip -1.5pc
\end{figure}


\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{./Figures/Pullback} 
\vskip -0.5pc
\caption{The pullback of the vector field W. 
}\label{fig:Pullback}
\end{center}
\vskip -1.5pc
\end{figure}

\subsubsection{Pushforwards and Pullbacks}
\paragraph*{Pushforward}  Let $F : M \rightarrow N$ be a smooth mapping between manifolds and $X\in \mathfrak{X}(M)$ and $Y \in \mathfrak{X}(N)$ smooth vector fields. $X$ and $Y$ are $\F$-related if 
\[
Y_{F(p)}=dF_p (X_p) 
% = (F_{*})_pX_p.
\]
where $dF_p$ is the differential of $F$ at $p$.
If $F$ is a diffeomorphism (i.e. $F$ has a differentiable inverse in addition to being smooth), for every $X\in \mathfrak{X}(M)$, there is a unique smooth vector field on $N$ that is F -related to $X$ \cite{leesmooth}. This unique  F-related field $Y \in \mathfrak{X}(N)$ is denoted as $Y = F_* X$ and is called the pushforward of $X$ by $F$.


% The image  ${\displaystyle d\F _{p}X}$ of a tangent vector  ${\displaystyle X\in T_{p}M}$ under 
%  ${\displaystyle d\F _{p}}$ is  called the pushforward of $X$ by 
% ${\displaystyle \F}$ denoted by $\F_* X$. 
% Push-forward is a linear approximation of smooth maps on tangent spaces. 
The push-forward takes tangent vectors at $p \in M$  and "pushes" them forward to tangent vectors at the corresponding point $q = F(p)$ in   $N$ as shown in Fig.~\ref{fig:Pushforward}.
 The  formula for the pushforward of $X$ by $\F$ at $q$ is given by 
\[
(\F_\ast X)_q  = dF_{\F^{-1} (q)} ( X_{\F^{-1}(q)} ) = d\F_p(X_p)
% =d \F_{\F^{-1} (q)} ( X_{\F^{-1}(q)} ),  
\]
and is given in explicit coordinates by \eqref{eq:pushforward_coordinates}.
% where $q \in N$,
% which is the composition of the   smooth maps :
% $N  \stackrel{\F^{-1}}{\rightarrow}   M  \stackrel{X}{\rightarrow}    T_pM  \stackrel{d\F }{\rightarrow}    T_qN.$
%  Equivalently, $\forall p \in M$,
% \[
% = d\F_p(X_p).
% \]

\paragraph*{Pullback} 
Let $\F: M \rightarrow N$ be a smooth map between two smooth manifolds $M$ and $N$. The differential 
$dF_p : T_p M \rightarrow T_{F(p)} N$
% of $\F$ at a point $p \in M$,  i.e.,  
induces a dual linear map
$dF^*_{F(p)} : T^*_{F(p)} N \rightarrow T^*_p M  $ called the (pointwise) pullback by $F$ at $F(p)$ or the cotangent map of $F$. Given a one form $\omega \in T^*_{F(p)} N$, and a vector $v \in T_p M$, $dF^*_{F(p)}$ is characterized as
\[
dF^*_{F(p)}(\omega)(v) = \omega (dF_p(v))\,.
\]
In contrast to vector fields, which can only be pushforwarded by diffeomorphisms, covector fields can always be pullback. Given a covector field $\omega  = \omega_i  dy^i \in T^*  N$ we define the covector field $F^* \omega \in T^* M$, called the pullback  of $\omega$ by $F$
\[
(F^* \omega)_p = dF^*_{F(p)}(\omega_{F(p)})\,.
\]
In coordinates,
\[
F^*\omega = F^*(\omega_i dy^i) = (\omega_i \circ F) F^* dy^i = (\omega_i \circ F) d ( y^i \circ F)
\]
which yields 
\[
(F^*\omega)_p =  \left . (\omega_i \circ F) dF^i \right |_p  =  (\omega_i(F(p))) \left . \frac{\partial F^i(x)}{\partial x^j} dx^j \right |_p .
\]
% induces a linear map between the tangent spaces. For any $v \in T_pM$, we have $d\F_p(v) \in T_{\F(p)}N$.
%
% For every vector field $W$ on $N$, the pullback of $W$ along $\F$ is the vector field, $\F^\ast W$ on $M$ given by
% \[
% (\F^\ast W)_p=(\F^{-1}_{\F(p)})_* (W_{\F(p) })=d\F^{-1}_{\F(p)} (W_{\F(p) }),
% \]
% where $p \in M.$  The pullback of the vector field $W$ by $F$ is given in Fig.~\ref{fig:Pullback}.

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{./Figures/Liederiv} 
\vskip -0.5pc
\caption{The Lie derivative of the vector field $W$. 
}\label{LD}
\end{center}
\vskip -1.5pc
\end{figure}

\subsubsection{Lie derivatives on vector fields} 
 Suppose $M$ is a smooth manifold, $V \in \mathfrak{X}(M)$ is a smooth vector field on $M$. Let $J$ be a time interval. A smooth curve $\gamma : J \to M$ determines a tangent vector $\gamma' (t)\in T_{\gamma(t)} M$. $\gamma$ is an integral curve of the vector field $V
$ if the velocity vector $\gamma' (t)
 $ is a tangent vector in $T_{\gamma(t)}M$ and
\[
\gamma' (t) = \dot \gamma^i(t) \left . \frac{\partial}{\partial x^i} \right | _{\gamma (t)} = V_{\gamma(t)} = V^i(\gamma(t)) \left . \frac{\partial}{\partial x^i} \right | _{\gamma (t)},\:\: \forall t \in J\,.
\]
Therefore, $\dot \gamma^i (t) = V^i(\gamma(t))$, $\forall t \in J$.  Suppose now that $V$ has a unique integral curve starting at $p$ and defined for all $t \in \Real$. We call this map $F_t : \Real \times M \to M$  the flow of $V$ on $M$, which sends  $p \in M$ to the point obtained by following this integral curve starting at $p$,  such  that $F_t(p) = F(t,p)$ and $F_0(p) = p$. Therefore, $F_t(p)$ is a one parameter group action
\[
F_t \circ F_s(p) = F_{t+s}(p) = F(t+s,p)
\]
and
\[
V_p = F_0'(p) = \left . \frac{\partial}{\partial t} F(t,p)\right |_{t = 0} \,.
\]
 


% Lie derivatives can be defined on smooth vector fields \cite{leesmooth}. \JS{TBD: Check the Equations!} 
Suppose $M$ is a smooth manifold, $V$ is a smooth vector field on $M$ and $\F$ is the flow of $V$. For any
smooth vector field $W$ on $M$, we define   the Lie derivative of $W$ with respect to $V$ at $p$, denoted by $(\Lie_V W)_p$, is given by
\[
\begin{split}
(\Lie_V W)_p:&= \frac{d}{dt}  d (\F_{-t})_{\F_t(p)}  (W_{\F_t(p)}) \bigg |_{t=0}\\
&=\lim_{t\rightarrow 0} \frac{d(\F_{-t})_{\F_t(p)} (W_{\F_t(p)})-W_p}{t}\\
&=\lim_{t\rightarrow 0} \frac{ (d (\F_{t})_{p})^{-1} (W_{\F_t(p)}) -W_p}{t}\\
&=\lim_{t\rightarrow 0} \frac{ d\F_{-t}  (W (\F_t(p)))-W(p)}{t}\\
&= \frac{d}{dt}   (d\F_{-t}  (W (\F_t(p)))) \bigg |_{t=0}.
 \end{split}
\]
 To consitute the Lie derivative by comparing $W_{\F_{t}(p)}$ and $W_p$,   $W(\F_{t}(p))$  was brought back to  $T_pM$ by applying the pushforward  $d\F_{-t}$ (the tangent map) at $\F(p)$ (see Fig.~\ref{LD}). $-t$ is used to find the inverse of $d\F_t$, and now  both $W_p$ and $d(\F_{-t})_{\F_t(p)} (W_{\F_t(p)})$ are in  $T_pM$.%

Since $(\F_{-t})^{-1}=\F_t$, pushforward or pullback operations can be used to define  Lie derivative as follows. 
\[
\begin{split}
(\Lie_V W)_p:  &=\lim_{t\rightarrow 0} \frac{ d\F_{-t}  (W (\F_t(p)))-W(p)}{t}\\
 &=\lim_{t\rightarrow 0} \frac{  ((\F_{-t})_\ast  W) (p)-W(p)}{t}\\
&= \frac{d}{dt}   ( (\F_{-t})_\ast  W ) (p) \bigg |_{t=0}\\
 &=\lim_{t\rightarrow 0} \frac{  ((\F_{t})^\ast  W) (p)-W(p)}{t}\\
&= \frac{d}{dt}   ( (\F_{t})^\ast  W ) (p) \bigg |_{t=0},
 \end{split}
\]

Finally, it can be shown that
\[
(\Lie_X W)_p=[X, W]_p.
\]

\subsection{Lie Groups and Algebras}
\subsubsection{Lie Groups}
%Lie groups appear as symmetry groups of physical systems, and their Lie algebras, i.e., tangent vectors near the identity $\Id$,   can be viewed as infinitesimal symmetry motions.  
A Lie group is a continuous group that is also a differentiable manifold.  
It  combines the concepts of a group and a smooth manifold. It is a group equipped with a smooth structure that allows continuous transformations and compositions, preserving both the algebraic and geometric properties.  Lie groups play a fundamental role in various areas of mathematics and physics, serving as a framework to study symmetries and transformations in a continuous manner.

Examples of Lie groups include the group of translations in $n$-dimensional space,   the group of invertible $n \times n$ matrices with real entries, i.e.,  general linear group $GL(n,\Real)$, and the group of rotations in $n$-dimensional space, i.e., $SO(n)$.

Lie groups emerge as the symmetry groups governing physical systems, with their corresponding Lie algebras representing infinitesimal symmetry motions as tangent vectors in the vicinity of the identity element $\Id$.
For instance, Lie groups concerning the rigid body motion, i.e., $SE(3)$, represent symmetries in such systems, while their Lie algebras, such as twists, capture infinitesimal motions. In robotics, twists, comprising linear and angular velocity components, represent small incremental movements of a system via robotic arm's joints. This elegant mathematical framework connects Lie groups, Lie algebras, and physical motions, offering a powerful tool to model symmetries and transformations in various robotic applications, which will be further explored in the following subsection.

\subsubsection{Lie Algebra}
An element $g \in \G$  (Lie group) close to the identity $\Id$ can be denoted as $g(\epsilon) = \Id +\epsilon Z$, where $\epsilon$ is a small number and $Z$ is called a generator. These small transformations are called infinitesimal transformations, and they change the object only slightly.  To obtain a finite transformation, one needs to repeat the infinitesimal transformation infinitely often. This can be represented as the limit of the product of the infinitesimal transformations :
\[g(t) = \lim_{N\rightarrow \infty}  \left ({\Id}  + \frac{t}{N}Z \right )^N = \exp(tZ),\]
where  
$Z$ is the generator that generates the finite transformation $g$. The generator is an element of the Lie algebra of the Lie group. The Lie algebra is the tangent space of the Lie group at $\Id$, i.e., its identity element, and it can be viewed as the set of all infinitesimal transformations generated by the Lie group. 
 
For example, a matrix Lie group $(GL(n), \cdot)$ is a group for which the set $GL(n)$ is an analytic manifold (embedded in a higher-dimensional Euclidian space)
where  each $g \in GL(n)$ is an $n \times n$ matrix, the group operation   is matrix multiplication,
and the mappings $g_1 \cdot g_2$ and $g^{-1}$ are both analytic.
Given a matrix Lie group $GL(n)$, elements sufficiently close to $\Id$ are written
as 
\begin{equation}\label{eq:exp}
g =  \exp_m(X)=\sum_{k=0}^{\infty} \frac{X^k}{ k!},
\end{equation}
for $X \in \fg$.
For
any real $n \times n$  matrix  $X \in \fgl(n)$, its matrix exponential $\exp(X)$ is   defined by  the series in \eqref{eq:exp}.
The exponential   maps $X \in \fgl(n)$ into $\exp(X) \in GL(n)$.
The matrix
Lie algebra $\fg$  is  the set of all matrices $X$   such that the exponential of each $X$ results in an element of $GL(n)$, i.e., 
\[
\fg= \{ X \in \fg l(n) | \exp(tX) \in GL(n), \forall t \in \Real \}.
\]

Let 
${\G}$ be a Lie group (i.e., a smooth manifold) and let 
$q \in  {\G}$. Let 
${\displaystyle T_{q}{\G}}$ be the tangent space at 
$q$. The cotangent space at $q$ is then defined as the dual space of 
${\displaystyle T_{x}{\G}}$:
${\displaystyle T_{x}^{*}\!{\G}=(T_{q}{\G})^{*}}$.
 $\fg=T_{\Id} \G$ and $\fg^*=T_{\Id}^*\G$ denote the Lie algebra (i.e., the tangent space of the  Lie group $\G$ at  $q=\Id$) and its dual, respectively (see Fig.~\ref{TG}).

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{./Figures/TG} 
\vskip -0.5pc
\caption{Illustration of   a Lie group $G$ and its tangent spaces.
The Lie algebra $\fg = T_{\Id}G$ is the tangent space at the identity $\Id$.
}\label{TG}
\end{center}
%\vskip -1.5pc
\end{figure}

\subsubsection{Lie Bracket}
 A Lie algebra $\fg$ is a vector space equipped with a Lie bracket operation
$[ \cdot, \cdot ] : \fg \times \fg \rightarrow \fg$ which is bilinear, anti-symmetric, $[a, b] = -[b, a]$, and satisfies the
Jacobi identity
$[a, [b, c]] + [b, [c, a]] + [c, [a, b]]=0.$ 

Let $\mathfrak{X}$ represent the set of smooth vector fields on $\G$. For any smooth function $f :\G\rightarrow \Real$,   the Lie bracket $[\cdot,\cdot]:\mathfrak{X} \times \mathfrak{X}\rightarrow \mathfrak{X}$ is then defined such that $[X,Y](f) := X(Y(f))-Y(X(f))$.

\subsubsection{Exponential Map and Logarithm Map}
\paragraph*{Exponential Map} The exponential map, $\exp: \fg \rightarrow \G$ is a local diffeomorphism defined by 
 \[
 \exp(X):=\gamma(1),
 \] 
 with $\gamma: \Real \rightarrow \G$ with $\dot \gamma(0)=X$. 

 Define the isomorphism of the hat-map such as
 \[
 (\cdot )^{\wedge}: \Real^n \rightarrow \fg,
 \]
 that maps a vector in $\Real$ to $T_{\Id} \G$. Its inverse map vee-map is defined as
 \[
 (\cdot )^\vee: \fg : \rightarrow \Real^n.
 \]
 For $X \in \fg$, the Lie exponential can be denoted by
map as
\[
\exp(\cdot): \Real^n \rightarrow \G, \quad \exp(X)=\exp_m(X^{\wedge}),
\]
 where $\exp_m(\cdot)$ is the exponential of square matrices.
 The exponential map takes an element of the Lie algebra in $\fg =T_{\Id} \G$ and produces an element
of the Lie group $\G$ such as $\exp: \fgl(n) \rightarrow GL(n)$, i.e.,  $\exp(X=\log(g)) = g$.  
\paragraph*{Logarithm Map}
On the other hand, the  logarithm does the opposite $\log: GL(n)\rightarrow \fgl(n)$, i.e., 
$\log( g=\exp X) = X$ (see Fig.~\ref{TG}). 

In summary, we have
\[
\begin{split}
\exp(X)&=\exp_m (X^{\wedge}) =g,\\
\log(g)&=\log_m(g)^\vee =X,
\end{split}
\]
where $\exp_m(\cdot)$ and $\log_m(\cdot)$ are the matrix exponential and logarithm, respectively. 

\subsubsection{Group Representations}
Before introducing group representation, we first introduce special morphisms frequently utilized in Lie Group theory. 
\paragraph*{Diffeomorphisms}
Given two manifolds 
$M$ and $N$, a differentiable map ${ \phi \colon M\rightarrow N}$ is called a diffeomorphism if it is a bijection and its inverse 
${\phi^{-1}\colon N\rightarrow M}$ is differentiable as well.

\paragraph*{Homomorphisms}
A homomorphism is a mapping from one group to a subset of another, $\phi: (G, \circ) \rightarrow (H, \hat \circ)$ such that
\[
\phi(g\circ h) = \phi(g) \, \hat \circ \,  \phi (h).
\]
With $h=\Id,$  we see that 
$\phi(g) = \phi(g\circ \Id) = \phi(g) \, \hat \circ \,  \phi(\Id),$ and
therefore,  $\phi(\Id)=\Id_H$ is  the identity in $H$.

\paragraph*{Isomorphisms}
a\JS{Proper definition as above will be nice}
A structure-preserving mapping between two structures of the same type that can be reversed by an inverse mapping.

\paragraph*{Automorphisms}
a\JS{Proper definition as above will be nice}
An isomorphism from a structure to itself. In linear vector space, it is an identity matrix. 

\paragraph*{Group Representation}
If a linear map is a bijection then it is called a linear isomorphism.
Assume that $V$ is an $n$-dimensional vector space over $\Real$. We define 
\[GL(V ) = \{ A : V \rightarrow V\; |\; A \text{ is a linear isomorphism} \}  \]

Let $\G$ be a Lie group and $V \in \Real^n$ is a vector space. 
A representation of a Lie group is a map   $\rho: \G \rightarrow  GL(V )$ of Lie groups.

\paragraph*{Translations}
Note first that the translations here is different from a translational motion used in the rigid-body dynamics.
Let $g, h \in \G$ be elements of a Lie group $\G$. We define the left translation of $\G$ by $g$ as the map
$L_g : \G \to \G,$ such that  $L_g(h) = gh$,  $\forall h \in \G$, and right translation as the map $R_g: \G \to \G$, such that $R_g(h) = hg$, $\forall h \in \G$. 

It is straightforward  to see that 
\[L_g^{-1} (h)=L_{g^{-1}}(h) \text{ and  } R_g^{-1} (h)=R_{g^{-1}}(h)\]
 since $L_g (L_g)^{-1} (h)=g (g^{-1})h=h$ and  $R_g (R_g)^{-1} (h)=h g (g^{-1})=h.$ 
Henceforth, both $L_g$ and $R_g$ are diffeomorphisms.  In addition, they commute to each other, i.e., $L_g R_h=R_h L_g$.

A left-invariant vector field satisfies the following:
\[
X(gh)=T_h L_g X(h), 
\]
where $T_h L_g$ is the tangent map to $L_g$  at $h$. If $h=\Id,$ $X(g)=T_{\Id} L_g \zeta,$ where $\zeta=X(\Id).$

\subsubsection{Adjoint Representations}
Due to smooth  multiplication and inverse maps,
 $L_g$ and $R_g$ are diffeomorphisms.
The inner automorphism $R_{g^{-1}} \circoo L_g= R_{g^{-1}}L_g$  is then given by  
$\Psi_g(h)=R_{g^{-1}}L_g(h)
 = ghg^{-1}.$

\paragraph*{Adjoint Representation of Lie group $\G$}
The derivative of $\Psi_g=R_{g^{-1}} L_g$ at the identify $\Id$ i.e.,   $d\Psi_g(\Id): \fg \to \fg$  is an isomorphism of Lie algebras, denoted by $\Ad_g: \fg \to GL(\fg)$.

Given an element $X \in \fg$ of the Lie algebra and $g \in \G$ of the Lie group, the large adjoint (Adjoint) operator is then obtained as
\[
\begin{split}
\Ad_g X &:= \frac{d}{dt} (g \cdot \exp(tX) \cdot g^{-1})|_{t=0}\\
&= \frac{d}{dt} \exp (t g Xg^{-1}) |_{t=0} \\
&=gXg^{-1}.
\end{split}
\]

The large adjoint representation of $\G$ 
gives a homomorphism $Ad : \G \rightarrow GL(\fg)$ from the group $\G$ into the set of all invertible
linear transformations of $\fg$ onto itself.  
For all $g \in \G$, and all $X \in \fg$ we have $\Ad_g X=gXg^{-1}.$
This  Lie
algebra isomorphism enables change of frames (see Fig~\ref{fig:Adjoint}).

Note that in the robotics community, a large adjoint representation is often interpreted as a linear operator, i.e., $\Ad_g : \Real^6 \to \Real^6$, where $\Real^6$ is an isomorphic vector space of $\fg \in \se$ and $g \in \SE$. Although it might be confusing, as both adjoint representations are one-to-one, we will not distinguish their notations.

 \paragraph*{Adjoint Representation of Lie algebra  $\fg$}
 The derivative of $\Ad$ at the identity $\Id$, i.e.,  $d(\Ad_{\Id}): \fg \rightarrow \fgl(\fg)$  is the map of Lie algebras, denoted by
  $ad: \fg \rightarrow \fg(\fg)$ called the adjoint representation of $\fg$ with 
\[\ad_X Y=[X,Y].\]

The relationship between $\Ad$ and $\ad$ is given by
\[\Ad_{(\exp tX)}=\exp_m(t \cdot \ad_{(X)}).\]
(as we have $g=\exp (X)$.)

The summary of  Lie algebra and Lie group and their adjoints is illustrated in Fig.~\ref{fig:Summary}.

\begin{figure}[!t]
    \centering
    \centering
    \resizebox{0.9\columnwidth}{!}{
    \input{Figures/Summary.tex}}
    \caption{Summary of Lie algebra and Lie group and their adjoints that take an element of Lie algebra for $(\cdot)$.
    }\label{fig:Summary}    
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\columnwidth]{Figures/adjoint_2.png}
    \caption{An illustration of   a Lie group $\G$ and its Lie algebra  $\fg$ of the tangent space at $\Id$.
    The  Adjoint  of $g$ applied on an element of $\fg$, i.e.,  $v=\frac{d}{ds} \gamma(s)|_{s=0}$ is illustrated.    Note that $Ad_g v \in \fg.$
     $\Psi_g(\Id)=g\Id g^{-1}=\Id$
    implies  that any curve $\gamma(s)$ through $\Id$
     on $\G$
     is mapped by this homomorphism $\Psi_g$ to another  curve  $g \gamma(s) g^{-1}$ on  $\G$ through $\Id$.
     }
     \label{fig:Adjoint}
\end{figure}
The derivative of $L_{g^{-1}}$ at $g$ is a linear
map  from   $T_g \G$ to  $T_\Id \G=\fg$ because $L_{g^{-1}}g=g^{-1}g=\Id$.
Given a differentiable curve $g(t)$ on $\G$ with its velocity $\dot g(t):=\frac{d g(t)}{dt}$, the left differential of $L_{g^{-1}}$, i.e., $dL_{g^{-1}} : T_g \G \rightarrow \fg$ maps $\dot g$ to an element $\fg$ such as 
\[dL_{g^{-1}} (g)(\dot g) =g^{-1} \dot g \in \fg.\]
Similarly, the right differential can be defined as 
\[dR_{g^{-1}}(g) \dot g=\dot g g^{-1} \in \fg.\]

In the next section, we  show that for $g\in SE(3)$,  $g^{-1} \dot g$ and $\dot g g^{-1}$  represent body and spatial velocities, respectively.

\paragraph*{Inverse and Composition Rules}
Recall that $\Ad_g$ can be defined by the inner automorphism $\Psi_g(h) = R_{g^{-1}} L_g(h) = ghg^{-1}$. The adjoint representation is  linear and acts on the Lie algebra $\mathfrak{g}$ of $\G$ defined as:
\[
\Ad_g: \mathfrak{g} \rightarrow \mathfrak{g}, \quad \Ad_g(X) = d(\Psi_g)_\mathrm{\Id}(X),
\]
where $X$ is an element of the Lie algebra $\mathfrak{g}$. 

For $g, h \in \G$, we see that  $(\Psi_g)^{-1}$ shall satisfy  
\[
   \begin{split}
(\Psi_g) (\Psi_g)^{-1}h&=g [ (\Psi_g)^{-1}h] g^{-1}=h,\\
  (\Psi_g)^{-1} (\Psi_g) h&= (\Psi_g)^{-1}  g h g^{-1}=h.
  \end{split}
\]
Therefore, we have
\[
(\Psi_g)^{-1}= \Psi_{g^{-1}}.
\]

For $g, h, k \in \G$,  the composition rule  of inner automorphisms is given by 
\[\Psi_{gh (k)}=\Psi_{g}  \Psi_{h} (k),\]
which shows the homomorphism. This can be shown as follows:
\[
    \begin{split}
    \Psi_{g}  \Psi_{h} (k) &=   
    \Psi_g( \Psi_h (k))\\
    &=R_{g^{-1}}L_g( \Psi_h (k))
     = g  \Psi_h (k) g^{-1}= g h k h^{-1}g^{-1}\\
     &=(gh)k (gh)^{-1}=
    \Psi_{gh}(k).
    \end{split}
\] 

For $X \in \fg,$ we see that $(\Ad_g)^{-1}$ needs to satisfy 
\[
    \begin{split}
(\Ad_g) (\Ad_g)^{-1}X&=g [ (\Ad_g)^{-1}X] g^{-1}=X,\\
  (\Ad_g)^{-1} (\Ad_g) X&=(\Ad_g)^{-1} g X g^{-1}=X.
    \end{split}
\]

As a result, similar to the previous case, we have
\[
(\Ad_g)^{-1}= \Ad_{g^{-1}}
\]

The Adjoint composition rule  can be given by
\begin{equation}\label{eq:Adchain}
 \Ad_{g} \Ad_{h}(X) = \Ad_{gh}(X)   
\end{equation}
 for arbitrary $X$ in the Lie algebra $\mathfrak{g}$.

This can be shown by
\[
\Ad_g \Ad_h(X) = g(hXh^{-1} )g^{-1} = (g h)X(gh)^{-1}= \Ad_{gh}X,
\]
which shows that $Ad_{(\cdot)}$ is a homomorphism.

\paragraph*{Adjoint Representations and Translations}
$\Psi_g(\Id)=g\Id g^{-1}=\Id$
implies that any curve $\gamma(s)$ through $\Id$
on $\G$
is mapped by this homomorphism $\Psi_g$ to another curve $g \gamma(s) g^{-1}$ on $\G$ through $\Id$ (see Fig.~\ref{fig:Adjoint}). 

The adjoint representation ($\Ad_g =d \Psi_g (\Id) $) maps any tangent vector $v$ in $\fg=T_{\Id}\G$
 to another tangent vector $Ad_g v=gvg^{-1}$ in $T_{\Id} \G$ while  $L_g$ or $R_g$
 maps tangent vectors in $T_{\Id} \G$  to tangent vectors in $T_{g} \G$ (see Fig.~\ref{fig:Adjoint}).

\subsubsection{Lie Derivatives on a Function}
Let $X \in \fg$, the Lie algebra of the Lie group $\G$, and let $f: \G \rightarrow \Real$ be analytic. 
\paragraph*{Left-Lie derivative}
$\forall g \in \G$, the left Lie derivative of  $f(g)$ with respect to   $X$, is defined by \cite{chirikjian2011stochastic} as
\[
\begin{split}
 \mathcal{L}_X^l f(g)&= \tilde X^l f (g)\\
&:=\lim_{t \rightarrow 0} \frac{f( \exp(-tX) g)   -f(g)}{t}\\
 &=\frac{d}{dt}  f(\exp(tX)   g) \bigg |_{t=0}.
 \  \end{split}
 \]  
\paragraph*{Right-Lie derivative}
 Similarly, 
 $\forall g \in \G$, the right  Lie derivative of  $f(g)$ with respect to   $X$, is defined by \cite{chirikjian2011stochastic} as
\[
\begin{split}
 \mathcal{L}_X^r f(g)&=\tilde X^r f (g)\\
 &:=\lim_{t \rightarrow 0} \frac{f(g \exp(tX)) -f(g)}{t}\\
 &=\frac{d}{dt}    f(g  \exp(tX)) \bigg |_{t=0}.
 \  \end{split}
 \]  

\subsubsection{Left-Regular Representation} \label{sec:left_regular_representation}
A useful way to let a group $\G$ act on functions is through left-regular representations. In this case, a function is transformed by transforming the domain $X$ by the action of the group $\G$ on $X$.
The left-regular representation of $g \in G$ acting on $f(x)$ is defined by
\begin{equation}\label{eq:left}
L_g(f)(x) = g \circoo  f(x)= f(g^{-1} \circoo x)
\end{equation}
where $\circoo$ denotes the action of the group $\G$ on the appropriate domain or codomain.
$f\in \mathbb{L}^2(\mathbb{R}^2)$ is a square-integrable function and $g^{-1}$ is the inverse of the group element $g$.

% \JS{Need to be reviewed from here}
% The left-regular representation of a Lie group G can be represented using pushforward notation in the view of smooth manifolds.
% Let $G$ be a Lie group, and let $L: G\rightarrow Diff(G)$ be the left-regular representation of $G$ given by
% \[L_g(h) = g \cdot h, \forall g, h \in G\]
% with $\cdot$ being the group operation in G.
% The pushforward notation for the left-regular representation is given by:
% \[L_*: T_e G \rightarrow X(G)\]
% where $T_eG$ is the tangent space to G at the identity element $e$, and $X(G)$ is the space of smooth vector fields on $G$.
% The pushforward $L_*$ is defined by:
% \[L_*(v)_g =  \left (\frac{d}{dt} \right ) \bigg |_0 L_g(\exp(tv))\]
% where $v$ is a tangent vector at the identity element e, and $\exp(tv)$ is the one-parameter subgroup of $G$ generated by $v$. The pushforward $L_*$ assigns to each tangent vector $v$ at the identity element e a vector field $L_*(v)$ on $G$, which is a left-invariant vector field.
%
% Therefore, the left-regular representation of a Lie group G can be represented as a pushforward notation using the pushforward map $L_*$.
%
% In other words, the left-regular representation of SE(2) acts on functions by transforming their arguments in the opposite direction of the group element $g$. This means that if we apply a transformation $g$ to the domain of a function $f$, we can obtain the transformed function $L_g(f)$ by applying the left-regular representation of $SE(2)$ to $f$.
% \JS{To here}

For example, the left-regular representation of SE(2) is an important tool in the study of group representations and equivariant neural networks, as it allows us to generalize the convolution operation of CNNs to equivariant group CNNs by replacing the usual convolution kernels with group-equivariant kernels that transform according to the left-regular representation of the group, which will be discussed in the next section. 

\subsection{Special Euclidean Group SE(3)}
In this subsection, we focus on the Special Euclidean Group $SE(3)$ as it is widely utilized in robotics applications. Although there are many other well-written robotics references, such as \cite{lynch2017modern}, we will follow the notations of \cite{murray1994mathematical} for unity in notations. Note also that the reference of this subsection is \cite{murray1994mathematical}.

\subsubsection{Lie Group Properties of $SE(3)$}
\paragraph*{Rigid Body Motions in $SE(3)$}
Let us consider the position and orientation of a coordinate frame B attached to the rigid body relative to an
inertial frame A (see Fig.~\ref{fig:SE(3)}).

The configuration space of the system is denoted by the special Euclidean group, i.e.,  $SE(3)$  that consists of the pair $(p_{ab} \in \Real^3, R_{ab} \in SO(3))$, which is  the product space of $\Real^3$ and  $SO(3)$.
\[
\begin{split}
SE(3) &= \{( p, R) : p\in \Real^3, R\in SO(3) \}\\
 &= \Real^3 \times SO(3). 
\end{split}
\]
An element $(p, R)\in SE(3)$ informs  
both a specification of the configuration of a rigid body and a transformation taking the coordinates of a point from one frame to another.

For example, $g_{ab} = (p_{ab}, R_{ab})\in SE(3)$ is the specification of the configuration of
the B frame relative to the A frame. We may also write
$g(q)$ to denote the action of a rigid transformation on a point,
$g(q) = p + R_q,$ so that $q_a = g_{ab}(q_b).$

Given $q_b$, we can find $q_a$ by a transformation of
coordinates such that
\[q_a = p_{ab} + R_{ab}q_b,\]
where $q_a$ and $q_b$ are   the coordinates of a point $q$ relative to frames
A and B, respectively. 

\begin{figure}[!t]
\centering
\resizebox{\columnwidth}{!}{
\input{Figures/Coordinate_frame.tex}}
\caption{Coordinate frames $\{A\}$ and $\{B\}$ for specifying rigid motions.}
\label{fig:SE(3)}
\end{figure}

\paragraph*{Homogeneous Matrix Representation in 
$SE(3)$.}
The $4 \times 4$ matrix $\bar g_{ab}$ is referred to as  the homogeneous representation of $g_{ab} \in
SE(3)$
\[
\bar q_a:= \left[
\begin{array}{c}
 q_{a}   \\
     1 
\end{array}
\right]
 =
\left[
\begin{array}{cc}
  R_{ab}    &  p_{ab}  \\
 0 & 1   
\end{array}
\right]
 \left[
\begin{array}{ccc}
 q_{b}   \\
     1 
\end{array}
\right]
=:\bar g_{ab} \bar q_b.
\]
%
The coordinate of  $q$ with respect to frame B can be represented with respect to  frame A by
\[
\bar q_a = \bar g_{ab} \bar q_b.
\]
Without subscripts, if $g = (p, R)\in SE(3)$, we have  its homogeneous representation 
\[
\bar g=\left[
\begin{array}{ccc}
  R    &  p  \\
 0 & 1   
\end{array}
\right]  \in
SE(3).
\]

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.70\columnwidth]{./Figures/coordinate_transformation.png} 
\vskip -0.5pc
\caption{Rigid body motion generated by rotation about a fixed axis.
}\label{fig:Motion}
\end{center}
\vskip -1.5pc
\end{figure}

Consider the rotational motion of a rigid body about a line in the $z$-direction through $(0, l_1, 0) \in \Real^3$, as shown in Fig.~\ref{fig:Motion}.
The orientation of the coordinate frame B relative to frame A  is given by
\[
R_{ab}=
\left[
\begin{array}{ccc}
 \cos \theta &  -\sin \theta  &  0  \\
 \sin \theta &  \cos \theta  &  0 \\
 0 &  0  &   1
\end{array}
\right]
\]
The coordinates of the origin of frame B relative to frame A are given by
\[
p_{ab}=\left[
\begin{array}{c}
0  \\
 l_1   \\
 0  
\end{array}
\right].
\] 
The homogeneous representation of the configuration of the rigid body is then given by
\[
\bar{g}_{ab}=\left[
\begin{array}{cc}
  R_{ab}    &  p_{ab}  \\
 0 & 1   
\end{array}
\right]
=
\left[
\begin{array}{cccc}
 \cos \theta &  -\sin \theta  &  0 & 0 \\
 \sin \theta &  \cos \theta  &  0 & l_1 \\
 0 &  0  &   1 & 0\\
  0 &  0  &   0 & 1
\end{array}
\right].
\]
Rigid body transformations may be composed to form a new rigid body
transformations. Let $g_{bc} \in SE(3)$ be the configuration of a frame C
relative to a frame B, and $g_{ab}$ the configuration of frame B relative to
another frame A. Using the following composition rule, the configuration of C
relative to frame A is given by
\[
\bar g_{ac}=\bar g_{ab} \bar g_{bc}
= \left[
\begin{array}{ccc}
  R_{ab} R_{bc}   &  R_{ab} p_{bc}+ p_{ab}  \\
 0 & 1   
\end{array}
\right]
\]
since $\bar q_a=\bar g_{ab} ( \bar   q_b =\bar g_{bc} \bar   q_c)$  gives 
 \[\bar q_a=\bar g_{ab}  \bar g_{bc}   \bar q_c= \bar g_{ac} \bar q_c.\]

As can be seen from the example above, rigid body transformations may be composed iteratively  such that
 \[\bar q_a=\bar g_{ab}  \bar g_{bc}   \cdots \bar g_{op}  \bar q_p= \bar g_{ap} \bar q_p.\]

For the rest of the paper, we will now denote the homogeneous matrix representation of $\SE$ $\bar g$ as $g$. 

Using the homogeneous
representation,  the set of rigid transformations is shown to be 
a group.
\begin{itemize}
\item If $g_1, g_2\in SE(3)$, then $g_1g_2\in SE(3)$.
\item The  identity  $ \Id \in  SE(3)$.
\item If $g\in SE(3)$, then the inverse of $g$ is determined by the 
matrix inversion:
\[
g^{-1}= 
 \left[
\begin{array}{ccc}
 R^T  & -R^T p  \\
    0 & 1 
\end{array}
\right] \in SE(3),
\]
where $g^{-1} = (-R^Tp, R^T)$.
\item The composition rule for rigid body transformations is associative.
\end{itemize}

\subsubsection{Lie Algebra Properties of $\SE$}
\paragraph*{Hat- and Vee-maps in $SE(3)$.}
 The Lie algebra of $SO(3)$, denoted by  $\fso$, defines skew-symmetric matrices.
 The hat-map for $\fso$ is defined by 
$\widehat{(\cdot)}\, (\text{or} \, (\cdot )^{\wedge} ): \Real^3 \rightarrow \fso,$ which maps an angular velocity vector $\omega \in \Real^3$ to its skew-symmetric cross product matrix, i.e.,  
\[\hat \omega=- \hat \omega^T
=
  \left[
\begin{array}{ccc}
0  & -\omega_3 & \omega_2   \\
 \omega_3 & 0 & -\omega_1 \\
  -\omega_2  & \omega_1 & 0
\end{array}
\right]  \in \Real^{3 \times 3}
\] 


for $\omega \in \Real^3.$
 Hence, for $v \in \Real^3$, $\hat \omega v = \omega \times v.$
The inverse of the hat map is the   vee-map    
 $
 (\cdot )^\vee: \fso : \rightarrow \Real^3.
 $
Similarly, the hat-map for $\fse$ is defined as  $\widehat{(\cdot)}: \Real^6 \rightarrow \fse.$
The inverse of the hat map is the   vee-map    
 $
 (\cdot )^\vee: \fse : \rightarrow \Real^6.
 $
Thus, we have
\[
 \fse \ni \hat \xi = 
 \left[
\begin{array}{ccc}
 \hat \omega  & v  \\
    0 & 0 
\end{array}
\right] \in \Real^{4 \times 4},
\forall  \xi = 
 \left[
\begin{array}{ccc}
  v  \\
    \omega
     \end{array}
\right] \in \Real^6,
\]
where $v, \omega \in \Real^3, \hat \omega \in \fso.$

\paragraph*{Twists}
An element of $\fse$ is referred to as a twist or a (infinitesimal) generator
of the Euclidean group.  Recall that the adjoint action  of $g \in SE(3)$ on $\xi \in \fse$, $\Ad: SE(3) \times \fse \rightarrow \fse$, is then defined by
\[
Ad_g \xi = g \xi g^{-1}.
\]

\paragraph*{Spatial and Body Velocities (twists in $SE(3)$)}
Consider a pure rotation. 
Let $R_{ab}(t) \in SO(3)$ be a curve representing a trajectory of an object frame B  relative to a fixed (inertial) coordinate frame A.
Any point $q$ attached to the rigid body follows a trajectory in spatial coordinates:
\[
q_a(t) =R_{ab}(t) q_b.
\]
The velocity of $q$ in spatial coordinates is
\[
\begin{split}
v_{q_a}(t)  = \frac{d}{dt} q_a(t)&=\dot R_{ab}(t) q_b\\
&=\underbrace{\dot R_{ab}(t) R_{ab}^{-1}(t)}_{=:\widehat \omega_{ab}^s (t)} R_{ab}(t) q_b\\
&=\widehat \omega_{ab}^s(t) R_{ab} (t) q_b \\
&=\omega_{ab}^s (t) \times  R_{ab} (t)q_b\\
&=\omega_{ab}^s (t) \times  q_a (t)\\
\end{split}
\]
where $\omega_{ab}^s$ is the instantaneous spatial angular velocity, i.e.,
\[
\widehat \omega_{ab}^s:=\dot R_{ab} R_{ab}^{-1}.
\]

We also define the angular velocity as viewed from
the instantaneous body  coordinate frame B as  the instantaneous body angular velocity:
\[
\widehat \omega_{ab}^b:= R_{ab}^{-1}\dot R_{ab}.
\]

Relationships between two angular velocities are
\[
\widehat \omega_{ab}^b=R^{-1}_{ab} \widehat \omega_{ab}^s R_{ab},   \quad \text{or} \quad \omega_{ab}^b=R_{ab}^{-1} \omega_{ab}^s.
\]
From this, we can describe the velocity of $q$ relative to body frame B:
\[
v_{q_b} (t):= R_{ab}^T(t) v_{q_a}(t)= \omega_{ab}^b(t) \times q_b.
\]

Consider now a   curve parameterized by time,  representing a trajectory of
a rigid body such that
\[
g_{ab}(t)= \left[
\begin{array}{cc}
     R_{ab}(t) & p_{ab}(t)  \\
      0 &   1
\end{array}
\right]
\]

The coordinates of $q$ attached to the body frame B in spatial coordinates are given by
\[
q_a(t)= g_{ab} (t) q_b.
\]
The velocity of $q$ in spatial coordinates is
\[
\begin{split}
v_{q_a}=\frac{d}{dt} q_a &=\dot g_{ab} q_b= \dot g_{ab} g_{ab}^{-1} q_a\\
&=\widehat V_{ab}^s q_a= \omega_{ab}^s \times q_a + v_{ab}^s.
\end{split}
\]
Here  we  define the spatial velocity $\widehat{V}_{ab}^s$ of a rigid motion $g_{ab} \in SE(3)$
\[
\widehat{V}_{ab}^s:= \dot g_{ab} g_{ab}^{-1}=
\left[
\begin{array}{cc}
\dot R_{ab}   R_{ab}^T &  -\dot R_{ab}   R_{ab}^T p_{ab} +  \dot  p_{ab} \\
  0 & 0
  \end{array}
\right],
\] 
\[
{V}_{ab}^s=\left[
\begin{array}{c}
 v_{ab}^s \\
   \omega_{ab}^s  
\end{array}
\right]
=
\left[
\begin{array}{c}
  -\dot R_{ab}   R_{ab}^T p_{ab} +  \dot  p_{ab} \\
      ( \dot R_{ab} R_{ab}^T)^\vee
\end{array}
\right]
\] 
We also define the body (or generalized) velocity of a rigid motion $g_{ab} \in SE(3)$
\[
\begin{split}
\widehat{V}_{ab}^b:= g_{ab}^{-1} \dot g_{ab} &=
\left[
\begin{array}{cc}
 R_{ab}^T  \dot R_{ab} &   R_{ab}^T    \dot p_{ab}  \\
  0 & 0
  \end{array}
\right]\\
&=
\left[
\begin{array}{cc}
\widehat \omega_{ab} &   v_{ab}  \\
  0 & 0
  \end{array}
\right],
\end{split}
\] 
where $\widehat \omega_{ab}^b =R_{ab}^T  \dot R_{ab} $ and $v_{ab}^b=R_{ab}^T    \dot p_{ab}$.
\[
{V}_{ab}^b=\left[
\begin{array}{c}
 v_{ab}^b \\
   \omega_{ab}^b  
\end{array}
\right]
=
\left[
\begin{array}{c}
  R_{ab}^T    \dot  p_{ab} \\
      (  R_{ab}^T \dot R_{ab})^\vee
\end{array}
\right]
\] 

Body velocity can be transformed into the spatial velocity by the adjoint transformation $Ad_g$, i.e.,
\[
{V}_{ab}^s=
\left[
\begin{array}{c}
 v_{ab}^s\\
   \omega_{ab}^s  
\end{array}
\right]
=
\underbrace{
\left[
\begin{array}{cc}
 R_{ab} & \widehat{p}_{ab} R_{ab}\\
    0 & R_{ab}
    \end{array}
\right]}_{=\Ad_{g_{ab}}}
\left [ V_{ab}^b=
\left[
\begin{array}{c}
 v_{ab}^b \\
   \omega_{ab}^b  
\end{array}
\right]
\right ] \] 
\[
i.e., \,
 {V}_{ab}^s=\Ad_{g_{ab}}{V}_{ab}^b, 
\]

Given  $g \in SE(3)$, the adjoint transformation $\Ad_g : \Real^6 \rightarrow \Real^6$ maps one coordinate to another 
\[
\Ad_g =\left[
\begin{array}{cc}
R & \widehat{p} R\\
    0 & R
    \end{array}
\right]
\]
$\Ad_g$ is invertible and its inverse is given by
\[
\Ad_g^{-1}=\left[
\begin{array}{cc}
R^T & -R^T\widehat{p} \\
    0 & R^T
    \end{array}
\right]
=\Ad_{g^{-1}}
\]

The body and spatial velocities are related by the (large) adjoint transformation.
\[
V^s=\Ad_g V^b, \quad  V^b=\Ad_{g}^{-1} V^s=\Ad_{g^{-1}} V^s.
\]

As mentioned previously, the large adjoint map used herein is a linear operator version. 

Consider the motion of three frames A, B, and C. The configuration of frame C with respect to A is given by
\[
g_{ac}=g_{ab}g_{bc}.
\]
We then represent $\widehat V_{ac}^s$ using $\Ad_{g_{ab}}$ via the chain rule.
\[
\begin{split}
\widehat V_{ac}^s&=\dot g_{ac} g_{ac}^{-1}\\
&=(\dot g_{ab} g_{bc} + g_{ab} \dot g_{bc}) (g_{bc}^{-1}g_{ab}^{-1})\\
&=\dot g_{ab}g_{ab}^{-1} + g_{ab} (\dot g_{bc} g_{bc}^{-1}) g_{ab}^{-1}\\
&=\widehat V_{ab}^s+ g_{ab} \widehat V_{bc}^s g_{ab}^{-1}\\
\end{split}
\]
In twist coordinates, we have
\[
 V_{ac}^s=V_{ab}^s+ \Ad_{g_{ab}}   V_{bc}^s.
\]
Similarly $\widehat V_{ac}^b$  can be shown that
\[
  V_{ac}^b=\Ad_{g_{bc}^{-1}}  V_{ab}^b+ V_{bc}^b.
\]

 When frames B and C  are attached to  a rigid body and A  is the inertial frame, as shown in Fig.~\ref{fig:Wrench}, we have $V_{bc}^b=0$ such that
$V_{ac}^b=\Ad_{g_{bc}^{-1}}  V_{ab}^b$, which implies 
\[
V_{ab}^b= \Ad_{g_{bc}}V_{ac}^b=\Ad_{g_{cb}^{-1}}V_{ac}^b,
\]
 where $g_{bc} \in SE(3): \{ B\} \rightarrow \{C\},$ i.e.,  the configuration of frame C relative to frame B.    
This adjoint action of $SE(3)$ on $\fse$ clearly shows  the effect of a change
of body frame on the body velocity.

\begin{figure}[!t]
\centering
\resizebox{\columnwidth}{!}{
\input{Figures/wrench}}
\caption{Transformation of wrench $F$ between coordinate frames.}
\label{fig:Wrench}
\end{figure}

\paragraph*{Translated twists}
For a twist $\xi$ that  is the motion of a screw and we want to move it by applying  a constant  rigid motion $g$ with  $\dot g=0$. We then have new $\xi'$
\[
\xi'=\Ad_g \xi, \quad \hat \xi'=g \hat \xi g^{-1}.\]
We can interpret $\xi'$ such that 
if $\widehat \xi \in \fse$ is a twist with the coordinate $\xi \in \Real^6$, $\forall g \in SE(3)$, 
$g \widehat\xi g^{-1}$ is a twist with the coordinate $\Ad_g \xi \in \Real^6$.

\paragraph*{Dual of the Lie algebra}
The co-adjoint    action of $g$ (or sometimes used with $g^{-1}$) on  $\xi^* \in \fse^*$ which is the dual of $\xi$,  $\Ad_{g^{-1}}^* : G \times  \fse^* \rightarrow \fse^*$, is defined by a matrix in $\Real^{6 \times 6}$ such as
\[
Ad_{g^{-1}}^* =Ad_{g^{-1}}^T.
\]

In general, the co-adjoint action of $g$ on $\fg^*$, the dual of the Lie algebra $\fg$ of $g$, can be defined.
Let $Ad_g^*: \fg^* \rightarrow \fg^*$ be the dual of $Ad_g$ defined by
\[
\langle Ad_{g^{-1}}^* (\alpha), \xi \rangle= \langle \alpha, Ad_{g} (\xi) \rangle 
\] 
for $\alpha \in \fg^*$ and $\xi \in \fg$. The co-adjoint action of $g$ on $\fg^*$ is then given by the map $\Phi^*: G \times \fg^* \rightarrow \fg^* $
\[
\Phi^* (g, \alpha) =Ad_{g^{-1}}^* \alpha.
\]

\paragraph*{Wrenches}
A pair of a force and a moment acting on a rigid body 
is referred to as a wrench, i.e., 
a generalized force.
\[
F= 
\left[
\begin{array}{c}
  f  \\
  \tau    
\end{array}
\right],
\]
 where $f \in \Real^3$ and $\tau \in \Real^4$ are linear and rotational force components, respectively.

 Consider the motion of a rigid body by $g_{ab}(t)$ with respect to an inertial frame A and a body frame B.
Let $V_{ab}^b \in \Real^6$ and $F_b\in \Real^6$ be the instantaneous body velocity and an applied wrench.
The infinitesimal work is obtained by the inner product of $V_{ab}^b \in \Real^6$ and $F_b$.
\[
\delta W=   \langle V_{ab}^b,   F_b \rangle=(v^T f+ \omega^T \tau).
\]
The net work generated by applying $F_b$ through  a twist $V_{ab}^b$ during the  interval $[t_1, \, t_2]$ is given by
\[
W=\int_{t_1}^{t_2}  \langle V_{ab}^b, F_b  \rangle dt.
\]

Let $g_{bc} =(p_{bc},R_{bc})$ be the configuration of frame C relative to B.
To find an equivalent wrench $F_c$ applied at C, we equate two instantaneous work quantities by $F_c$ and $F_b$.
\[
\begin{split}
  \langle V_{ac}, F_c \rangle&=\langle  V_{ab}, F_b \rangle\\
  &= (Ad_{g_{bc}}V_{ac})^T F_b = \langle V_{ac} , \Ad_{g_{bc}}^T F_b \rangle,
\end{split}
\]
where we use the relationship between body velocities, i.e., $V_{ab}=\Ad_{g_{bc}} V_{ac}.$

The coordinate transformation between wrenches $F_c$ and $F_b$  (see Fig.~\ref{fig:Wrench}) can be represented by different ways.
\[
\begin{split}
F_c &= \Ad_{g_{bc}}^T F_b=\Ad_{g_{ba}g_{ac}}^T F_b\\
&=(\Ad_{g_{ba}}\Ad_{g_{ac}} )^T F_b=\Ad_{g_{ac}}^T\Ad_{g_{ba}}^T F_b\\
    &=\Ad_{g_{cb}^{-1}}^T F_b=\Ad_{(g_{ca}g_{ab})^{-1}}^T F_b =\Ad_{ g_{ab}^{-1} g_{ca}^{-1} }^T F_b\\
    &= (\Ad_{ g_{ab}^{-1}} \Ad_{g_{ca}^{-1} } )^T F_b=  \Ad_{g_{ca}^{-1} }^T  \Ad_{ g_{ab}^{-1}}^T F_b,
\end{split}
\]
where the adjoint composition  rule in \eqref{eq:Adchain} was used.    

 

\paragraph*{Exponential map from $\fse$ to $SE(3)$.}
Given $\hat \xi \in \fse$ and $\theta \in \Real$, the exponential of $\hat \xi \theta$ is in $SE(3)$, i.e., 
\[
\begin{split}
    \exp{(\hat \xi \theta)} &= \exp{   \left (\left[
\begin{array}{ccc}
 \hat \omega  & v  \\
    0 & 0 
\end{array}
\right]   \theta  \right ) }\in SE(3)\\
&=I+ {    \left[
\begin{array}{ccc}
 \hat \omega  & v  \\
    0 & 0 
\end{array}
\right]   \theta    } + { \frac{1}{2!}   \left[
\begin{array}{ccc}
 \hat \omega^2  & \hat \omega v  \\
    0 & 0 
\end{array}
\right]   \theta^2    } \\ &+ { \frac{1}{3!}   \left[
\begin{array}{ccc}
 \hat \omega^3  & \hat \omega^2 v  \\
    0 & 0 
\end{array}
\right]   \theta^3    }+ \cdots
\end{split}
\] 
This shows that the exponential map from $\fse$ to $SE(3)$ is the matrix exponential on a linear combination of the
generators.
We interpret the transformation $g=\exp(\hat \xi \theta)$ 
as a mapping  from an initial coordinate, $p(0)\in \Real^3$, to its
coordinate $p(\theta)$ after the rigid motion is applied such that
\[
p(\theta)= \exp{(\hat \xi \theta)} p(0).
\]
Let $g_{ab}(0)$ represent the initial configuration of a rigid body relative to a frame A, then the final configuration,
 with respect to A, is given by
\[
g_{ab}(\theta)= \exp{(\hat \xi \theta)} g_{ab}(0).
\]
The exponential map for a twist gives the relative motion of a rigid
body.

\subsubsection{Forward Kinematics}
The forward kinematics of the manipulator is given by the product of the exponentials formula, i.e., a map $g: Q \rightarrow SE(3):$
\[
g(\F)=e^{(\hat \xi_1 \theta_1)}e^{(\hat \xi_2 \theta_2)} \cdots e^{(\hat \xi_n \theta_n)} g(0),
\]
where $e^{(\cdot)}=\exp(\cdot)$ and $g(\theta)$ is the homogeneous representation of the end-effector in the spatial frame, $\xi_i \in \Real^6$ and $\theta_i \in \Real$ are a twist represented in the spatial frame and a joint angle of the $i$-th joint, respectively, for $i=1, 2, \cdots n$, starting from the base. See more details in \cite{murray1994mathematical}.

==> Old/Section4_EquivariantDeepLearning.tex <==
\subsection{Regular Group Convolutional Neural Networks}
\subsubsection{Standard Convolutional Neural Networks: Cross-correlation Kernels and Weight-sharing}
Before introducing the equivariant group CNNs (G-CNNs),  let us first consider the standard CNNs, which use cross-correlation (or convolution) kernels to extract features from images. 
\paragraph*{Cross-correlation Kernels} The cross-correlation (or convolution) operation between an input image $f(x)$ and a correlation kernel $\W(x)$ (or a convolution kernel $\hat \W(x)$, respectively) at   $x$ can be written as:
\begin{equation}\label{eq:conv}
\begin{split}
y(x) &= (\W \star f )(x) = \int_{\mathbb{R}^n} f( \tilde  x)\W(\tilde x-x)d \tilde  x\\
&= (\hat \W \ast f) (x) =  \int_{\mathbb{R}^n} f( \tilde  x) \hat \W(x- \tilde x)d \tilde  x,
\end{split} 
\end{equation}
where $\W(x)=\hat \W(-x)$.
As can be seen in Fig.~\ref{fig:Alex}, many redundant rotated edge filters in different angles are generated in the standard CNNs (by training under image augmentation via rotation). These are convolutional filters in the first layer of AlexNet \cite{krizhevsky2012imagenet} trained on ImageNet \cite{deng2009imagenet}. Note that interpreting standard CNNs as cross-correlation kernels allows us a straightforward extension to the group equivariant CNNs.

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/Alexnet_1st_layer.png}
    \caption{Convolutional filters in the first layer of AlexNet\cite{krizhevsky2012imagenet} trained on ImageNet \cite{deng2009imagenet}. Many rotated edge filters with similar shapes can be spotted. This standard CNN is not efficient without weight sharing in the rotational angle. This figure is generated using pre-trained AlexNet provided by PyTorch \cite{PytorchAlexNet}.}
    \label{fig:Alex}
\end{figure}

\paragraph*{Weight-sharing}\label{weightsharing}
 Recall 
 the left-regular representation of $g \in G$ acting on $f(x)$ is defined by
\begin{equation}\label{eq:left2}
    L_g(f)(x) = g \circ  f(x)= f(g^{-1} \circ x)
\end{equation}
where $\circ$ denotes the
action of the group $G$ on the domain of $X$.
 $f\in \mathbb{L}^2(\mathbb{R}^2)$ is a square-integrable function and $g^{-1}$ is the inverse of the group element $g$.
 We also notice that
\begin{equation}\label{eq:g1g2}
\begin{split}
L_{g_1g_2}(f)(x) &= g_1g_2 \circ  f(x)=L_{g_1}L_{g_2}(f)(x)\\
&= f((g_1g_2)^{-1} \circ x)=f(g_2^{-1}g_1^{-1} \circ x).
\end{split}
\end{equation}

Once we use the left-regular representation in the translation group as in \eqref{eq:left2} as 
\[ \T_x(\W) (\tilde x):= L_x(\W)(\tilde x) = \W(\tilde x-x),\] 
\eqref{eq:conv} can then be represented as an inner product. 
\[
\begin{split}
y(x) = (\W \star f )(x) &= \int_{\mathbb{R}^n} f(\tilde x)\W(\tilde x-x)d \tilde x\\
&=\langle \T_x (\W), f\rangle_{\mathbb{L}_2 (\mathbb{R}^n)}.
\end{split}
\]
From the inner product form, the convolution using learned kernels in standard CNNs is now considered template matching in order 
to extract features over different locations in $x$.  This leads to efficient learning via sharing kernel weights across various locations in the data. 
Standard  CNNs are effective for data that exhibits translation symmetry. However, they may not efficiently learn features such as an edge shape with different angles without weight sharing in rotational angles. To address this limitation, data augmentation techniques such as rotating images with different angles are used to generate a larger number of kernels (or filters) with various orientations, as in  Fig.~\ref{fig:Alex}.


 We now consider a transformation operator in $SE(2)$ $L_g$ with the roto-translation parameter $g=(x,\theta)$, where $x$ and $\theta$ are the translation vector and the rotation angle, respectively.
 
 Due to \eqref{eq:g1g2} with $g_1=(x)$ and $g_2=(\theta)$, $L_g=L_{(x,\theta)}$ can be obtained as follows.
  \[
  \begin{split}
[ L_{g_1g_2} \W ](\tilde x)&=[ L_{(x,\theta)} \W ](\tilde x) =[L_x L_\theta \W ](\tilde x)\\ &=\W (g_2^{-1} g_1^{-1} \tilde x)) = \W (R^{-1}_\theta (\tilde x - x)).
 \end{split}
 \]

 One can also obtain the same result by using a homogeneous matrix representation as follows:
\begin{equation*}
    \begin{split}
        &g = \begin{bmatrix}
            R_\theta & x \\
            0 & 1
        \end{bmatrix}, \quad g^{-1} = \begin{bmatrix}
            R^{-1}_\theta & -R^{-1}_\theta x \\
            0 & 1
        \end{bmatrix}\\
        &g^{-1} \begin{bmatrix}
            \tilde{x} \\ 1
        \end{bmatrix}  = \begin{bmatrix}
            -R^{-1}_\theta (x - \tilde{x}) \\ 1 
        \end{bmatrix} = \begin{bmatrix}
            R^{-1}_\theta (\tilde{x} - x) \\ 1
        \end{bmatrix} \\
        &\implies g^{-1} \circ \tilde{x} = R^{-1}_\theta (\tilde{x} - x).
    \end{split} 
\end{equation*}

\subsubsection{$SE(2)$-Group Convolutional Neural Networks}
\paragraph*{$SE(2)$ Lifting Correlations.}  We can then define the roto-translation lifting correlation from $\Real^2$ to the space of $SE(2)$ such as 
 \begin{equation}\label{eq:LiftingCov}
 \begin{split}
y(g)&=y(x, \theta)=(\W \star_{SE(2)}  f )  (x, \theta)\\
 &=  \langle L_{(x, \theta)}\W, f \rangle_{\mathbb{L}_2 (\Real^2)} =\langle L_{x} L_\theta \W, f \rangle_{\mathbb{L}_2 (\Real^2)} \\
&=\int_{\Real^2} \W (R^{-1}_{\theta} (\tilde x-x)) f(\tilde x) d \tilde x.
 \end{split}
\end{equation}

\paragraph*{ $SE(2)$ Group Convolutions} $SE(2)$ group convolution are roto-translation equivariant. 
Following the initial roto-translation lifting correlation on a 2D image, a feature map is generated on   $SE(2)$. The feature layers resulting from the lifting operation are then parameterized by patterns of position-orientation localized features, which can be transformed by the action of the group element $L_{(x, \theta)}$. This transformation enables the use of $SE(2)$-equivariant convolutional neural networks (G-CNNs) that operate on $SE(2)$ kernels, thereby allowing for the efficient extraction of features that are invariant to both translation and rotation.
After the $SE(2)$ lifting convolution, the $SE(2)$  group convolution can be performed in the lifted higher dimensional feature maps of $SE(2)$.
\begin{equation}\label{eq:SEfilter}
    \begin{split}
    y(g) &= 
     \int_{SE(2)} \W (g^{-1} \circoo \tilde g) f(\tilde g) d \tilde g\\
    &= \int_{\Real^2} \int_{S^1} \W(R^{-1}_\theta (\tilde x- x),  \tilde \theta -\theta) f(\tilde x, \tilde \theta) d \tilde x d \tilde \theta.
    \end{split}
\end{equation}

\subsubsection{Equivariant maps} Suppose $\G$ is a Lie group, and $M$ and
$N$ are both smooth manifolds with smooth left or right $\G$-actions. A map (e.g., a neural network)
$\Phi : M \rightarrow N$ is said to be equivariant with respect to   $\G$-actions   if for each
$g \in \G$, 
\[
\Phi(g \cdot p)=g \cdot \Phi(p),\quad \text{for left actions},\]
and 
\[
\Phi(p \cdot g)= \Phi(p) \cdot g, \quad  \text{for right actions \cite{leesmooth}.} \] 
Equivariance implies that no information is lost by input transformations, i.e., 
the output will be shifted to different locations in the output domain. It also allows for weight sharing over the transformations in the
group (e.g., SE(2) or SE(3) including rotation), which reduces a significant number of learnable parameters as compared to the standard CNNs (e.g., see Fig.~\ref{fig:Alex}). 
For example, $SE(2)$ equivariant CNNs (i.e., G-CNNs) for 2D images can be built using lifting and group convolutions from \eqref{eq:LiftingCov} and \eqref{eq:SEfilter}, respectively. Although G-CNNs are more efficient due to weight sharing compared to the standard CNNs,  the  filtered  outputs in discretized $\theta$
need to be computed and stored for the higher dimensional feature space in $SE(2)$. Steerable filters can be used to mitigate these computational and memory burdens.

\subsection{Steerable Group Convolutional Neural Networks}
More efficient equivariant convolutional neural networks (i.e., steerable G-CNNs) can be constructed using 
steerable feature vectors, which will remove the discretization in rotation as in G-CNNs with the $SE(2)$ regular group convolutions.
Steerability of a vector (say $h$) implies that for a transformation group $g$, the vector $h$ transforms via matrix-vector multiplication $D(g)h$. 
Steerable methods avoid discretization of $SO(n)$ in regular G-CNNs by exploiting irreducible representations, which allows for Fourier theory on Lie groups. Steerable methods build on the following concepts: steerable feature vectors, spherical harmonics, Wigner-D matrices, and the Clebsch-Gordan tensor product. 
In particular, as the spherical harmonics (SH) play a crucial role in the formulation of steerable group convolutional neural networks, we will first introduce the details of the SH. 
% In particular, we will first cover the formulation of the SH.

\subsubsection{Spherical Harmonics (SH)}
Spherical harmonics (SH) provide a theoretical foundation for the steerable functions as they serve as a basis function for $\SO$ transformation. SH is a class of functions on the sphere $S^2$ and can be used as a Fourier basis on the sphere. As will be mentioned later, they are steered by Wigner-D matrices and allow the interpretation of steerable vectors as functions on $S^2$. Moreover, spherical harmonics allow the embedding of 3D displacement vectors into arbitrarily large steerable vectors, i.e., allows lifting. 
Although the theory of SH is well established among physics/chemistry fields, those with engineering backgrounds might be unfamiliar with this concept. Therefore, we present the motivations and formulation of SH for readers to understand easily. 
Spherical harmonics are motivated by the Laplace equation in the spherical coordinates. We will first build the SH in the complex domain, but general applications of SH are built in the real domain, and the interchange between the two domains is possible. Note also that the derivation is from \cite{SH_wiki}.

Consider a function $f:\mathbb{R}^3 \to \mathbb{C}$. For the function without any sink or source, the following Laplace's equation holds:
\begin{equation} \label{eq:Laplaces}
    \nabla \cdot \nabla f(x,y,z) = \nabla ^2 f(x,y,z) = 0
\end{equation}
SH naturally arises as we try to solve the \eqref{eq:Laplaces} in spherical coordinate systems, i.e., using the change of coordinates (See Fig.~\ref{fig:change_of_coordinates}):
\begin{equation}
    x = r \sin{\theta}\cos{\phi}, \;\; y = r \sin{\theta}\sin{\phi}, \;\; z = r \cos{\theta}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width = 0.6\linewidth]{Figures/Spherical_coordinate.png}
    \caption{Change of coordinates; from Cartesian $(x,y,z)$ to the spherical coordinates $(r,\theta,\phi)$.}
    \label{fig:change_of_coordinates}
\end{figure}

Then, after some algebra, we have
\begin{equation} \label{eq:Laplace_spherical}
    \begin{split}
        \nabla^2f &= \underbrace{\dfrac{1}{r^2}\dfrac{\partial}{\partial r} \left(r^2 \dfrac{\partial f}{\partial r} \right)}_{\triangleq\lambda} \\
        &+ \underbrace{\dfrac{1}{r^2 \sin\theta} \dfrac{\partial}{\partial \theta} \left(\sin{\theta} \dfrac{\partial f}{\partial \theta}\right) + \dfrac{1}{r^2 \sin^2\theta} \dfrac{\partial^2 f}{\partial \phi ^2}}_{\triangleq-\lambda} = 0.
    \end{split}    
\end{equation}
To solve the partial differential equation (PDE) \eqref{eq:Laplace_spherical}, we first use the separation of variables as follows:
\begin{equation*}
    f(r,\theta,\phi) = R(r) Y(\theta,\phi)
\end{equation*}
By dividing \eqref{eq:Laplace_spherical} into two terms and with more algebra, we have
\begin{align}
     & \dfrac{1}{R}\dfrac{d}{dr}\left(r^2 \dfrac{dR}{dr}\right) = \lambda 
    \label{eq:radius_part}
    \\
    & \dfrac{1}{Y\sin\theta} \dfrac{\partial}{\partial \theta}\left(\sin{\theta}\dfrac{\partial Y}{\partial \theta}\right) + \dfrac{1}{Y\sin^2\theta} \dfrac{\partial^2 Y}{\partial \phi^2} = - \lambda. \label{eq:angle_part}
\end{align}
The angular terms \eqref{eq:angle_part} can be evaluated by using separation of variable again, i.e., $Y(\theta,\phi) = \Theta(\theta)\Phi(\phi)$, which leads to
\begin{align}
    &\dfrac{1}{\Phi} \dfrac{d^2 \Phi}{d\phi^2} = - m^2 \label{eq:phi_part} \\
    &\lambda \sin^2\theta + \dfrac{\sin{\theta}}{\Theta} \dfrac{d}{d\theta} \left(\sin\theta \dfrac{d \Theta}{d \theta}\right) = m^2.  \label{eq:theta_part}
\end{align}
with some number $m$. \eqref{eq:phi_part} is classic harmonic oscillator equation with respect to $\phi$. Therefore, $\Phi$ must be a period function whose period evenly divides $2\pi$, forming a boundary condition for \eqref{eq:phi_part}. Then, $m$ is necessarily an integer, and $\Phi$ is a linear combination of the complex exponentials $e^{\pm im\phi}$. 

Another fact that poses boundary conditions on \eqref{eq:theta_part} is that at the sphere's poles, i.e., $\theta = 0, \pi$, the function is regular: analytic and single-valued. Therefore, by imposing this regularity into the solution of $\Theta$ at the boundary points of the domains, we have the Strum-Liouville problem. As a result, the parameter $\lambda$ must have the form of $ \lambda = l(l+1)$ for some non-negative integer with $l \geq |m|$.

In what follows, after applying a change of variables $t = \cos{\theta}$ transforms the equation \eqref{eq:theta_part} into the Legendre equation, and the solution is given by a multiple of the associated Legendre polynomial $P^l_m$ \JS{$l$ upper and $m$ lower} \cite{associated_Legendre_polynomial}. Additionally, the solution of \eqref{eq:radius_part} has the solution of the form 
\begin{equation*}
    R(r) = Ar^l + Br^{-l-1},
\end{equation*}
but by applying the solution to be regular over $\mathbb{R}^3$ makes $B = 0$, i.e., when $r \to 0$.

Combining these results altogether, for a given value of $l$, there are $2l+1$ independent solutions of the form, $Y(\theta,\phi) = \Theta(\theta)\Phi(\phi)$, one for each integer $m$ with $-l \leq m \leq l$. We denote these independent solutions associated with the integer $m$ and $l$ as $Y_m^l$, $Y_m^l:S^2 \to \mathbb{C}$, and they are the product of complex exponentials and associated Legendre polynomials as follows:
\begin{equation} \label{eq:sol_Y}
    Y_m^l(\theta,\phi) = N e^{im\phi} P_m^l(\cos{\theta}).
\end{equation}
Here, $Y_m^l:S^2 \to \mathbb{C}$ is referred to as a spherical harmonic function of degree $l$ and order $m$.
Finally, a solution $f:\mathbb{R}^3 \to \mathbb{C}$ to Laplace's equation \eqref{eq:Laplaces} in a spherical coordinates system is a linear combination of the spherical harmonic functions multiplied by the appropriate scale factor $r^l$:
\begin{equation}\label{eq:spherical_harmonics_expansion}
    f(r,\theta,\phi) = \sum_{l=0}^\infty \sum_{m=-l}^l f_m^l r^l Y_m^l(\theta,\phi),
\end{equation}
where $f_m^l \in \mathbb{C}$ are constants. 

Based on these motivation, spherical harmonics are functions $Y_m^l$ with $l \geq 0$ and $-l \leq m \leq l$ spanning the sub-representation of $V_l$ vector spaces:
\begin{equation}
    \begin{split}
        V_0 &= \text{Span}\{Y_0^0(n)\}\\
        V_1 &= \text{Span}\{Y_{-1}^{1}(n), Y_0^1(n), Y_1^{1}(n)\} \\
        &\vdots \\
        V_k &= \text{Span}\{Y_{-k}^{k}(n), Y^k_{-k+1}(n), \cdots , Y^k_0(n), \cdots, Y^k_k(n)\},
    \end{split}
\end{equation}
where $n$ is a unit vector on a unit sphere and is one-to-one correspondence to $(\theta,\phi)$ representation. We call $V_l$ vector space as type-$l$ vector field and an arbitrary vector $h \in V_l$ as type-$l$ vector. 
A critical property of the SH is that it is transformed by a 3-dim rotation matrix $R \in \SO$. Consider $2l+1$-dimensional vector field, i.e., type-$l$ vector field:
\begin{equation}
    \mathbf{Y}^l = \left(Y_{-l}^{l}, Y_{-l+1}^l, \cdots, Y^l_{l-1}, Y^l_l\right)^T
\end{equation}
Then, $\mathbf{Y}^l$ is transformed by $R$ s.t.
\begin{equation}
    \mathbf{Y}^l\left(R \frac{x}{\|x\|}\right) = D^l(R) \mathbf{Y}^l\left(\frac{x}{\|x\|}\right).
\end{equation}
where $D^l(R)$ is a left-regular representation of $R\in SO(3)$ with order $l$. $D^l(R)$ is a Wigner-D matrix.

\subsubsection{Steerable function and vectors}
\paragraph*{Steerable Function}
A function is steerable under a transformation group $\G$ if any transformation $g \in \G$ on $f$ can be represented as a linear combination of a fixed, finite set of basis functions $\{ \phi_i\}$.
\[
{L}_g f= \sum_{i=1}^n \alpha_i (g) \phi_i = \alpha^T(g) \Phi,
\]
where ${L}_g f$ is the left-regular representation of the group $G$ that transforms    $f$.
The concept of steerability was first coined in the computer vision community \cite{freeman1991design}.
Steerable neural networks work with feature vectors consisting of these steerable feature vectors. 

\paragraph*{Steerable Feature Vectors}
Steerable feature vectors are vectors that transform via Wigner-D matrices \cite{aubert2013alternative, se3t, thomas2018tensor}, which are representations of $SO(3)$ and $SU(2)$. Wigner-D matrices are used to define any representation and are irreducible. A type-$l$ steerable vector space $V_l$ is a $(2l+1)$-dimensional vector space that is acted upon by a Wigner-D matrix of order $l$. For example, if $h$ is a type-$3$ vector in $V_3$, then it is transformed by $g \in SO(3)$ via  $h \rightarrow D_3(g)h$.
As mentioned above, SH is used to formulate a type-$l$ vector and is steerable via the Wigner-D matrix. 

Any vector $x \in \Real^3$ can be converted into a type-$l$ vector by the evaluation of spherical harmonics $Y_m^{l}: S^2 \rightarrow \Real$ at $n = \frac{x}{ \| x\|}$. In particular, for any $x \in \Real^3$, $\mathbf{Y}^l$ is a type-$l$ steerable vector. 
\begin{equation*}
    \mathbf{Y}^l = \left(Y_m^l\left(\frac{x}{\|x\|}\right) \right)^T_{m = -l, -l+1, \dots, l}
\end{equation*}

Consider a function in terms of spherical bases, with {\it coordinates} $a^l = [a_0^l, \cdots, a_l^l]^T$:
\begin{equation*}
    f_a = \sum_{l=0}^\infty \sum_{m=-l}^l a_m^l Y_m^l = \sum_{l=0}^\infty (\mathbf{a}^l)^T \mathbf{Y}^l,
\end{equation*}
where $\mathbf{a}^l = (a_{-l}^l, a_{-l+1}^l, \cdots, a_{l-1}^l, a_l^l)^T$.
It is steerable since we can show that   \cite{brandstetter2021geometric}
\begin{equation}\label{eq:Lgf}
\begin{split}
    L_g f_a(n) &=  f_{D(g)a} (n) \\&=\sum_{i=1}^n \alpha_i (g) \phi_i = \alpha^T(g) \Phi=(D(g) a)^T \Phi,
\end{split}
\end{equation}
 where $\alpha(g)=D(g) a$ and $\Phi= (Y_0^{0}, Y_{-1}^{1}, Y_0^{1}, \cdots)^T$. Alternatively,
\begin{equation}
    \begin{split}
        L_g f_a(n) &= f_a(g^{-1} \circ n) \\
        &= \sum_{l=0}^\infty (\mathbf{a}^l )^T D^l(g^{-1})\mathbf{Y}^l = \sum_{l=0}^\infty (\mathbf{a}^l )^T D^l(g)^T\mathbf{Y}^l\\
        &= \sum_{l=0}^\infty (D^l(g) \mathbf{a}^l)^T \mathbf{Y}^l
    \end{split}
\end{equation}
where the definition of left-regular representation is used, and property of the Wigner-D matrix, i.e., $D^l(g^{-1}) = D^l(g)^T$, for $g\in \SO$ is utilized \cite{lee2018real}. The $D(g)$ in \eqref{eq:Lgf} can be understood as block diagonal stack of $D^l(g)$, i.e., $D(g) = \text{blkdiag}(D^0(g), D^1(g), D^2(g) \cdots)$.

\subsubsection{Wigner-D Matrices}
 $D^{(l)}_{mn} : SO(3) \rightarrow \Real$ form complete orthogonal basis for functions on $SO(3)$.
Therefore, any function on $SO(3)$ can be represented in terms of an $SO(3)$ Fourier series. 
\[ 
\begin{split}
f(R) &=\sum_{l}^\infty  \sum_{m=-l}^{l} \sum_{n=-l}^{n=l} \hat f_{mn}^{(l)}D_{mn}^{l} (R) 
= \sum_l^\infty \tr \left( \hat f^{(l)} (D^{l} (R))^T\right)\\
&=\sum_l^\infty \tr \left ( \hat f^{(l)} D^{l} (R^{-1})\right )
\end{split}
\]
where $R \in \SO$, and the equation above can be considered as the inverse Fourier transform. Note that $D^l(R^{-1}) = (D^l(R))^T$ is utilized again.
The Fourier transform of a function $f(R)$ on $SO(3)$ can be then obtained by the inner product using the basis as follows:
\[
\hat f^{(l)}_{mn}=\langle D_{mn}^l(R), f(R) \rangle.
\]

\subsubsection{Steerable Group Convolution}
 Consider an input feature map $f: \Real^3 \rightarrow \Real$.
In many applications, we want to perform template matching for arbitrary translations and rotations. We can then    define the roto-translation lifting correlation from $\Real^3$ (i.e., the original  feature map input space) to the space of $SE(3)$ with $g=(x,R)$ such as 
 \[
 \begin{split}
y(g)&=(\W \star_{SE(3)}  f )  (g) = \langle L_{g}\W, f \rangle_{\mathbb{L}_2 (\Real^3)}\\ &=  \langle L_{(x, R)}\W, f \rangle_{\mathbb{L}_2 (\Real^3)}= \langle L_{x} L_R \W, f \rangle_{\mathbb{L}_2 (\Real^3)} \\
&=\int_{\Real^3} \W(g^{-1} \circoo  \tilde x)f(\tilde x) d \tilde x =\int_{\Real^3} \W(R^{-1} (\tilde x-x)) f(\tilde x) d \tilde x.
 \end{split}
 \]

The subsequent group convolution is then performed in the lifted higher dimensional feature maps of $SE(3)$.
\[
\begin{split}
y(g) 
 &= \langle L_{g}\W, f \rangle_{\mathbb{L}_2 (SE(3))}\\
&= 
 \int_{SE(3)} \W (g^{-1} \circoo \tilde g) f(\tilde g) d \tilde g.
%&= \int_{\Real^3} \int_{S^2} \W(R^{-1} (\tilde x- x),  \tilde \theta -\theta) f(\tilde x, \tilde \theta) d \tilde x d \tilde \theta.
 \end{split}
  \]

Consider now a 3D convolution kernel that is expanded in a spherical
harmonic basis (up to degree $l$):  
\[
\W(x)=\W_{c (\| x\|)} (x):= \sum_{\ell=0}^L \sum_{m=-\ell}^{\ell} c_m^{(\ell)} (\| x\|) Y_m^{\ell} \left ( \frac{x}{\|x\|}\right ),
\]
where $c= (c_0^{(0)}, c_{-1}^{(1)}, c_0^{(1)}, \cdots)^T$ is the collection of basis coefficients that depends on $\|x\|.$
Due to \eqref{eq:Lgf}, we conclude that the kernel is steerable via the transformation of $c$ by its $SO(3)$ representation $D(R)$
\[
L_g  \W(x)=\W(g^{-1}x)=\W_c(R^{-1}x)=\W_{D(R)c(\| x\|)} (x).
\]
Using this steerable kernel, we perform $SE(3)$ lifting convolution, i.e., $g = (x,R) \in \SE$ such as
\[
\begin{split}
y(g) &=y(x,R)
= \langle L_{g}\W, f \rangle_{\mathbb{L}_2 (\Real^3)}\\
&=\int_{\Real^3} L_g \W(\tilde x) f(\tilde x) d \tilde x\\
&=\int_{\Real^3} \W( R^{-1}  (\tilde x-x)) f(\tilde x) d \tilde x\\
&=\int_{\Real^3} \W_{D(R)c} (\tilde x-x)  f(\tilde x) d \tilde x\\
&=\int_{\Real^3} ({D(R)c})^T \Phi (\tilde x- x)  f(\tilde x) d \tilde x\\
&=({D(R)c})^T \int_{\Real^3}  \Phi (\tilde x- x)  f(\tilde x) d \tilde x\\
&=({D(R)c})^T \hat f^{\Phi} (x)
\end{split}
\]

Here, any transformation $g \in G$ on $\W$ can be represented as a linear combination of a set of basis $\Phi$. Hence, $({D(R)c})^T $ can be pulled out of the convolutional integral. Therefore, $y(g)$ is a function of $g$ without further convolution since the feature vector is already convoluted with a collection of basis, which does not require discretization in $R$ as in (non-steerable) group convolution in \eqref{eq:LiftingCov}.

\subsubsection{Clebsch-Gordan Tensor Product}
Clebsch-Gordan (CG) tensor product is used in steerable linear layers, which map between steerable input and output vector spaces. Similar to regular neural networks, where matrix-vector multiplication is used to map between input and output vector spaces, the CG tensor product is used to map between steerable input and output vector spaces. The learnable CG tensor product is the key component of steerable neural networks, similar to the learnable weight matrix-feature multiplication in regular neural networks.

For any two steerable vectors $h_1 \in  V_{\ell_1}$ and $h_2 \in  V_{\ell_2}$,   the CG tensor product’s output is
again steerable with a $SO(3)$ representation $D(g)$ as follows. \JS{We will use superscript $l$ for $D^l(g)$ or $D^l_{mn}(g)$}
\[
D(g) (h_1 \otimes h_2)= (D^{l_1} (g) h_1 ) \otimes (D^{l_2} (g) h_2 ),
\]
where $h_1 \otimes h_2 = h_1 h_2^T$.

The output resulting vector $\text{vec} (h_1 h_2^T)$ is steered by a representation $D(g) = D^{l_2}(g) \otimes D^{l_1}(g)$.
\[
\begin{split}
\text{vec} \left ( (D^{l_1} (g) h_1) (D^{l_2} (g) h_2)^T   \right ) &=\text{vec} \left ( (D^{l_1} (g) h_1) h_2^T D^{l_2} (g)^T   \right )\\
&=(D^{l_2} (g) ) \otimes (D^{l_1} (g)   )\text{vec} (h_1 h_2^T)\\
&=D(g)  \text{vec} (h_1 h_2^T),
\end{split}
\]
where $\text{vec}(AXB) = (B^T \otimes A) \text{vec}(X)$ was used in the second line, with $A \otimes B$ is the Kronecker product of the two matrices.
%
% Note also that the tensor product to the matrix $A \otimes B$ is the Kronecker product of the two matrices, e.g.,
% \begin{equation*}
%     \begin{split}
%         A &= \begin{bmatrix}
%             a_{11} & a_{12}\\
%             a_{21} & a_{22}
%         \end{bmatrix}, \quad B = \begin{bmatrix}
%             b_{11} & b_{12} \\ 
%             b_{21} & b_{22}
%         \end{bmatrix}, \\
%         A \otimes B &= \begin{bmatrix}
%             a_{11} \begin{bmatrix} b_{11} & b_{12} \\ b_{21} & b_{22} \end{bmatrix} & a_{12} \begin{bmatrix} b_{11} & b_{12} \\ b_{21} & b_{22} \end{bmatrix} \\
%             a_{21} \begin{bmatrix} b_{11} & b_{12} \\ b_{21} & b_{22} \end{bmatrix} & a_{22} \begin{bmatrix} b_{11} & b_{12} \\ b_{21} & b_{22} \end{bmatrix}
%         \end{bmatrix} \\&= \begin{bmatrix}
%             a_{11} b_{11} & a_{11} b_{12} & a_{12} b_{11} & a_{12} b_{12} \\
%             a_{11} b_{21} & a_{11} b_{22} & a_{12} b_{21} & a_{12} b_{22} \\
%             a_{21} b_{11} & a_{21} b_{12} & a_{22} b_{11} & a_{22} b_{12} \\
%             a_{21} b_{21} & a_{21} b_{22} & a_{22} b_{21} & a_{22} b_{22} 
%         \end{bmatrix}
%     \end{split}
% \end{equation*}
where $\text{vec}(\cdot)$ is a vectorize operator, which vectorizes the matrix by stacking its columns.
\subsection{Representation theory of the Lie Group} \JS{Is this supposed to be here?}
 A \textit{representation} $ {D}$ of a group $G$ is a map from $G$ to the space of linear operators acting on a vector space $\mathcal{V}$ that has the following property:
 \begin{equation}
     \label{eqn:homomorphism}
      {D}(g) {D}(h)= {D}(gh) \quad\forall g,h\in G
 \end{equation}
 Two different representations $ {D}$ and $ {D}'$ are said to be of \textit{equi\underline{valen}ce} (not   \textit{equi\underline{varian}ce})
 if there exists a non-degenerate change of basis $ {U}$ such that
 \begin{equation}
      {D}'(g)= {U} {D}(g) {U}^{-1}\qquad\forall g\in G
 \end{equation}
 A representation is said to be \textit{reducible} if there exists a change of basis such that the representation can be decomposed (block-diagonalized) into smaller subspaces. An \textit{irreducible representation} is a representation that cannot be reduced anymore. 

 For the $SO(3)$ group, any representation $ {D}( {R})$ for $ {R}\in SO(3)$ can be reduced into a direct sum of $(2l+1)\times(2l+1)$ dimensional irreducible representations $ {D}_{l}( {R})$ of \textit{degree} $l\in\{0,1,2,\cdots\}$ such that
 \begin{equation}
      {D}( {R})= {U}\left[\bigoplus_{n=1}^{N}{ {D}_{l_n}( {R})}\right] {U}^{-1}\qquad \forall  {R}\in SO(3)
 \end{equation}
 where $\bigoplus$ denotes a direct sum\footnote{Direct sum can be intuitively understood as a concatenation/block-concatenation for vectors/matrices.}.
 Although there are infinitely many equivalent representations for such $ {D}_l$, a particularly preferred choice is one with a \textit{real basis}\footnote{Another commonly used choice of basis is the \textit{spherical basis} whose representations are unitary}. In this basis, all the representations $ {D}_l$ are orthogonal matrices. These matrices are called the \textit{(real) Wigner D-matrices} \cite{aubert2013alternative, se3t, thomas2018tensor}.
 The $(2l+1)$ dimensional vectors that are transformed by $ {D}^l( {R})$ are called \textit{type-$l$} (or \textit{spin-$l$}) vectors. Type-$l$ vectors are identical to themselves when they are rotated by $\theta = 2\pi/l$. Type-$0$ vectors, or \textit{scalars} are invariant to rotations ($\theta=\infty$). Type-$1$ vectors are the familiar 3-dimensional space vectors ($\theta=2\pi$). 
 
 Let $\mathcal{V}$ be a (steerable) vector space and $\mathcal{X}$ and $\mathcal{Y}$ be (point-cloud data) sets with a group action $\circoo$ such that $g\circoo (h\circoo \dX)=(gh)\circoo \dX$ and $g\circoo (h\circoo \dY)=(gh)\circoo \dY\ \ \forall g,h\in G, \dX\in\mathcal{X}, \dY\in\mathcal{Y}$.
 A map $ {f}(\dX|\dY):\mathcal{X}\times\mathcal{Y}\rightarrow\mathcal{V}$ is said to be $G$-\textit{equivariant} if
 \begin{equation}
      {D}_{\mathcal{V}}(g) {f}(\dX|\dY)= {f}(g\circoo \dX|g\circoo \dY),
 \end{equation}
 $\forall g\in G, \dX\in\mathcal{X}, \dY\in\mathcal{Y}$, 
 where $ {D}_{\mathcal{V}}$ is a representation of $G$ acting on $\mathcal{V}$. In the special case where $ {D}_{\mathcal{V}}= {I}$, the map $ {f}(X|Y)$ is said to be \textit{$G$-invariant}.

 A translation invariant and $SO(3)$-equivariant type-$l$ vector field, or simply an \textit{$SE(3)$-equivariant type-$l$ vector field}, $ {f}( {x}|\dX):\mathbb{R}^3\times\mathcal{X}\rightarrow\mathbb{R}^{2l+1}$ is a special case of $SE(3)$-equivariant map such that
 \begin{equation}
      {D}^l( {R}) {f}( {x}|\dX)= {f}( {R} {x}+ {p}|g\circoo \dX)\quad \forall g=(  {p}, R)\in SE(3)
 \end{equation}
 where  $ {p}\in\mathbb{R}^3$, $ {R}\in SO(3)$ and $g\circoo {x}= {R} {x}+ {p}$.
 From now on, we simply denote the action of $g\in SE(3)$ on $ {x}\in\mathbb{R}^3$ as $g {x}$ instead of $g\circoo  {x}$ for brevity. 
A detailed recipe for constructing such $SE(3)$-equivariant vector fields when $\dX\in \mathcal{X}$ is given as a graph is described in the following subsection.

\subsection{SE(3)-equivariant graph neural networks}
\label{appendix_equiv_gnn}
Graph neural networks are often used to model point cloud data \cite{wang2019dynamic, te2018rgcnn, shi2020point}. 
$SE(3)$-equivariant graph neural networks \cite{thomas2018tensor, se3t, liao2022equiformer,brandstetter2021geometric} exploit the roto-translation symmetry of graphs with spatial structures.
We briefly introduce  Tensor Field Networks (TFNs) \cite{thomas2018tensor} and the SE(3)-transformers \cite{se3t} as the backbone networks for equivariant deep learning models. 

\subsubsection{Tensor Product and Spherical Harmonics}
Given two vectors $ {u}$ and $ {v}$ of type-$l_1$ and -$l_2$, the tensor product $ {u}\otimes  {v}$ transforms according to a rotation $ {R}\in SO(3)$ as
\begin{equation}
     {u}\otimes  {v}\rightarrow ( {D}^{l_1}( {R}) {u})\otimes ( {D}^{l_2}( {R}) {v})
\end{equation}
Tensor products are important because they can be used to construct new vectors of different types.
By a change of basis, the tensor product $ {u}\otimes  {v}$ can be decomposed into the direct sum of type-$l$ vectors using the \textit{Clebsch-Gordan coefficients} \cite{thomas2018tensor, zee, griffiths2018introduction}. Let this type-$l$ vector be $( {u}\otimes  {v})^{(l)}$. The $m$'th components of this vector is calculated as:
\begin{equation}
    ( {u}\otimes  {v})^{(l)}_m=\sum_{m_1=-l_1}^{l_1}\sum_{m_2=-l_2}^{l_2} C^{(l,m)}_{(l_1,m_1)(l_2,m_2)}u_{m_1}v_{m_2}
\end{equation}
where  $C^{(l,m)}_{(l_1,m_1)(l_2,m_2)}$ is the Clebsch-Gordan coefficients in real basis, which can be nonzero only for ${|l_1-l_2|\leq l \leq l_1+l_2}$.

The \textit{(real) spherical harmonics} $Y_m^{(l)}( {x}/\| {x}\|)$ are orthonormal functions that form the complete basis of the Hilbert space on the sphere $S^2$. $l\in\{0,1,2,\cdots\}$ is called the \textit{degree} and $m\in\{-l,\cdots,l\}$ is called the \textit{order} of the spherical harmonic function. Spherical harmonic bases with a few different orders and degrees are shown in Fig.~\ref{SH}. \JS{Check}

Consider the following $(2l+1)$-dimensional vector field 
\[ {Y}^{(l)}=(Y^{l}_{m=-l},\cdots,Y^{l}_{m=l}).\]

By a 3-dimensional rotation $ {R}\in SO(3)$, $ {Y}^{(l)}$ transforms like a type-$l$ vector field such that
\begin{equation}
     {Y}^{(l)}( {R}( {x}/\| {x}\|))= {D}^l( {R}) {Y}^{(l)}( {x}/\| {x}\|)
\end{equation}

\subsubsection{Tensor Field Networks} Tensor field networks (TFNs) \cite{thomas2018tensor} are $SE(3)$-equivariant models for generating representation-theoretic vector fields from a point cloud input. TFNs construct equivariant output feature vectors from equivariant input feature vectors and spherical harmonics. Spatial convolutions and tensor products are used for the equivariance.

Consider a featured point cloud input with $M$ points given by 
\[\dX=\{( {x}_1, {f}_1),\cdots,( {x}_M, {f}_M)\}\] where $ {x}_i\in\mathbb{R}^3$ is the position and $ {f}_i$ is the equivariant feature vector of the $i$-th point.
Let $ {f}_i$ be decomposed into $N$ vectors such that $ {f}_i=\bigoplus_{n=1}^{N} {f}_i^{(n)}$, where $ {f}_i^{(n)}$ is a type-$l_n$ vector, which is $(2l_n+1)$ dimensional.
Therefore, we define the action of $g=( p, {R})\in SE(3)$ on $\dX$ as
\begin{equation*}
   g\circoo \dX=\{(g{x}_1, {D}( {R}) {f}_1),\cdots,(g {x}_M, {D}( {R}) {f}_M)\}
\end{equation*}
where ${p}\in\mathbb{R}^3$, ${R}\in SO(3)$,  and $ {D}( {R})=\bigoplus_{n=1}^{N} {D}_{l_n}( {R})$.

Consider the following input feature field $ {f}_{(in)}( {x}|X)$ generated by the point cloud input $X$ as
\begin{equation}
     {f}_{(in)}( {x}|X)=\sum_{j=1}^{M} {f}_{j}\delta^{(3)}( {x}- {x}_j)
\end{equation}
where $\delta^{(3)}( {x}- {y})=\prod_{\mu=1}^3\delta(x_\mu-y_{\mu})$ is the three-dimensional Dirac delta function centered at $ {x}_j$. 
Note that this input feature field is an $SE(3)$-equivariant field, that is:
\begin{equation*}
      {f}_{(in)}(g {x}|g\circoo \dX) =  {D}( {R}) {f}_{(in)}( {x}|\dX)\quad\forall\ g=(p,  {R})\in SE(3)
\end{equation*}

Now consider the following output feature field by a convolution
\begin{equation}
\label{eqn:tfn}
    \begin{split}
     {f}_{(out)}&( {x}|\dX)=\bigoplus_{n'=1}^{N'} {f}_{(out)}^{(n')}( {x}| \dX)\\
    &=\int{d^3 {y}} {W}( {x}- {y}) {f}_{(in)}( {y}|\dX)=\sum_{j} {W}( {x}- {x}_j) {f}_{j}
    \end{split}
\end{equation}
with the convolution kernel $ {W}( {x}- {y})\in \mathbb{R}^{dim( {f}_{(out)})\times dim( {f}_{(in)})}$
 whose $(n',n)$-th block $ {W}^{(n',n)}( {x}- {y})\in\mathbb{R}^{(2l_{n'}+1)\times(2l_n+1)}$ is defined as follows:
\begin{equation}
    \label{eqn:tfn_kernel_const}
    \begin{split}
        \left[ {W}^{(n',n)}( {x})\right]^{m'}_{\phantom{m'}m}\!=\!\sum_{J=|l_{n'}-l_n|}^{l_{n'}+l_n}\phi^{(n',n)}_{J}(\| {x}\|)\sum_{k=-J}^{J}C^{(l_{n'},m')}_{(l_n,m)(J,k)}Y^{(J)}_{k}\left( {x}/\| {x}\|\right)
    \end{split}
\end{equation}
Here, $\phi^{(n',n)}_{J}(\| {x}\|):\mathbb{R}\rightarrow\mathbb{R}$ is some learnable radial function. 
The output feature field $ {f}_{(out)}( {x}|X)$ in \eqref{eqn:tfn} is proven to be $SE(3)$-equivariant \cite{thomas2018tensor, se3t}. 

\subsubsection{SE(3)-Transformers} The $SE(3)$-Transformers \cite{se3t} are variants of TFNs with self-attention. Consider the case in which the output field is also a featured sum of Dirac deltas
\begin{equation}
     {f}_{(out)}( {x}|X)=\sum_{j=1}^{M} {f}_{(out),j}\delta^{(3)}( {x}- {x}_j)
\end{equation}
where $ {x}_i$ is the same point as that of the point cloud input $X$. The SE(3)-Transformers apply type-0 (scalar) self-attention $\alpha_{ij}$ to \eqref{eqn:tfn}:
\begin{equation}
\begin{split}
     {f}_{(out),i}=\sum_{j\neq i}\alpha_{ij} {W}( {x}- {x}_j) {f}_{j}+\bigoplus_{n'}^{N'}\sum_{n=1}^{N} {W}_{(S)}^{(n',n)} {f}_{j}^{(n)}
\end{split}
\end{equation}
where the $ {W}_{(S)}^{(n',n)}$\ \ term is called the \textit{self-interaction} \cite{thomas2018tensor}. $ {W}_{(S)}^{(n',n)}$ is nonzero only when $l_n'=l_n$. The self-interaction occurs where $i=j$ such that $ {W}(x_i-x_j)=W(0)$. The self-interaction term is needed because $ {W}$ is a linear combination of the spherical harmonics,  which are not well defined in $ {x}=0$. Details about the calculation of the self-attention $\alpha_{ij}$ can be found in \cite{se3t}.
% \section{PAPER SIZE AND FORMAT}


\subsubsection{Equivariant Spherical Channel Network}
Equivariant Spherical Channel Network (eSCN)~\cite{passaro2023reducing} introduces a mathematically equivalent alternative to the original tensor product operation in TFNs with improved efficiency. eSCN reduces the computational complexity of tensor product from $O(L^6)$ to $O(L^3)$ where $L$ is the highest feature type. This unlocks the utilization of much higher frequency features, which has been reported to improve the accuracy in robotic manipulation tasks \cite{gao2024riemann, hu2024orbitgrasp}.

Specifically, eSCN exploits the sparsity of Clebsch-Gordon coefficients when the reference frame is aligned to the message-passing direction such that $x/\|x\|$ in \eqref{eqn:tfn_kernel_const} becomes $\hat{e}_y=(0,1,0)$. In this reference frame, the spherical harmonics component becomes sparse:
\begin{equation}
    \label{eqn:sparse_sh}
    Y^{(J)}_m(\hat{e}_y)=\delta_{m0}=\begin{cases}
        1 & \text{if } \ m=0
        \\
        0 & \text{else}
    \end{cases}
\end{equation}
To exploit this sparsity, \cite{passaro2023reducing} proposes to 1) rotate the reference frame where the message passing direction is aligned to $y$-axis, 2) apply tensor product, 3) and revert the transformation:
\begin{equation}
    \begin{split}
        f_{(out)}(x)&=\sum_{i}D(R_y^{-1}) W(\|x-x_j\|\hat{e}_y)D(R_y)f_j
        \\
        R_y(x-x_j)&=\|x-x_j\|\hat{e}_y
    \end{split}
\end{equation}
Note that $W(x)=D(R^{-1}) W(Rx)D(R)$ for all $x,R$ due to the kernel equivariance constraint.

By substituting \eqref{eqn:sparse_sh} into \eqref{eqn:tfn_kernel_const}, the convolution kernel becomes
\begin{equation}
    \label{eqn:escn-kernel}
    \begin{split}
        {W}^{(n',n)}( \hat{e}_y)\ &=\sum_{J=|l_{n'}-l_n|}^{l_{n'}+l_n}
        \phi^{(n',n)}_{J}(\| {x}\|)
        \bar{C}^{(l_n'\leftarrow l_n)}_{J}
        \\
        \left[\bar{C}^{(l_n'\leftarrow l_n)}_{J}\right]^{m'}_{\phantom{m'}m}&=C^{(l_{n'},m')}_{(l_n,m)(J,0)}
    \end{split}
\end{equation}
As pointed out by \cite{passaro2023reducing}, this tensor product can be understood as an $SO(2)$ convolution in the spectral domain. 
To show this, let us first drop the superscript $(l_n'\leftarrow l_n)$ for brevity. 
From Proposition~3.1 in \cite{passaro2023reducing}, one can show that $\bar{C}_{J}=\bar{S}_{J}+\bar{A}_{J}$ where  $\bar{S}_J$ is a symmetric diagonal matrix and $\bar{A}_J$ is an antisymmetric antidiagonal matrix. Additionally, $\bar{S}_J$ is symmetric to the row inversion.
\begin{equation}
    \label{eqn:escn-symmetry}
    \begin{split}
        \left[\bar{S}_J\right]^{m}_{\phantom{m}m}=\left[\bar{S}_J\right]^{-m}_{\phantom{-m}-m} 
        \ \ \forall\ m,\quad 
        \left[\bar{S}_J\right]^{m'}_{\phantom{m'}m}&=0\ \  \text{if}\ \ m'\neq m
        \\
        \left[\bar{A}_J\right]^{m}_{\phantom{m}-m}=-\left[\bar{A}_J\right]^{-m}_{\phantom{-m}m} 
        \ \ \forall\ m,\quad 
        \left[\bar{A}_J\right]^{m'}_{\phantom{m'}m}&=0\ \  \text{if}\ \ m'\neq -m
    \end{split}
\end{equation}
Hence, the convolution kernel ${W}^{(n',n)}( \hat{e}_y)$ in \eqref{eqn:escn-kernel} can also be decomposed into symmetric and antisymmetric parts that follows the same condition in \eqref{eqn:escn-symmetry}. 
This is because ${W}^{(n',n)}(\hat{e}_y)$ in \eqref{eqn:escn-kernel} is a linear combination of $\mathbf{C}_J^{(l_n'\leftarrow l_n)}$ whose coefficients are $\phi^{(n',n)}_{J}$.
\begin{equation}
    \begin{split}
        {W}^{(n',n)}(\hat{e}_y)&=S^{(n',n)}+A^{(n',n)}
        \\
        S^{(n',n)}&=\sum_{J=|l_{n'}-l_n|}^{l_{n'}+l_n}\phi^{(n',n)}_{J}(\| {x}\|)\bar{S}_J^{(l_n'\leftarrow l_n)}
        \\
        A^{(n',n)}&=\sum_{J=|l_{n'}-l_n|}^{l_{n'}+l_n}\phi^{(n',n)}_{J}(\| {x}\|)\bar{A}_J^{(l_n'\leftarrow l_n)}
    \end{split}
\end{equation}
Therefore, the convolution kernel ${W}^{(n',n)}(\hat{e}_y)$ is fully characterized by $2l_n+1$-dimensional vector $h^{(n',n)}$ defined as
\begin{equation*}
    h^{(n',n)}_m =
    \begin{cases}
        \left[S^{(n',n)}\right]^{m}_{\phantom{m}m} & m\geq 0
        \\
        \left[A^{(n',n)}\right]^{m}_{\phantom{m}-m} & m < 0
    \end{cases}
\end{equation*}

To show the connection with Fourier analysis, let us denote the complexification map from  $\mathbb{R}^{2l+1}$ to $\mathbb{C}^{l+1}$ as
\begin{equation}
    \tilde{f}_m
    =\begin{cases}
            \left[f\right]_{m}+i\left[f\right]_{-m} & m=1,2\cdots,l
            \\
            \left[f\right]_{0} & m =0
    \end{cases}
\end{equation}
The output tensor could be computed as the complex multiplication of these two vectors, which is similar to the $SO(2)$ convolution, which is simply a pointwise multiplication in Fourier space.
\begin{equation}
    \label{eqn:escn-fourier}
    \widetilde{(Wf)}^{(n')}_m
    =\begin{cases}
        \tilde{h}_m^{(n',n)}\tilde{f}_m^{(n)} & 0\leq m \leq l_n
        \\
        0 & m>l_n
    \end{cases}
\end{equation}
Indeed, $\tilde{h}_m^{(n',n)}$ is related to the Fourier coefficient\footnote{Note the Fourier coefficients of real functions are fully determined by non-negative frequencies because $\tilde{f}_{-m}=\tilde{f}_m^*$.} of the convolution kernel with frequency $m$ \cite{passaro2023reducing}. 
Furthermore, there exist a linear bijection from $\phi^{(n',n)}_{J}$ to $h^{(n',n)}$ \cite{passaro2023reducing}, and hence a bijection to $\tilde{h}^{(n',n)}$. Consequently, for any TFN-like $SO(3)$ tensor product (parameterized by $SO(3)$-invariant coefficients $\phi^{(n',n)}_{J}$), there exist a unique eSCN-like $SO(2)$ convolution (parameterized by the kernel's Fourier coefficients $\tilde{h}^{(n',n)}$) that is mathematically identical but much cheaper in terms of computation.





% \begin{equation}
%     \begin{split}
%     \left[\mathbf{S_0}\right]_{m'm}&=\begin{cases}
%         \left[\mathbf{S_0}\right]_{-m-m} & \text{if }\ m'=m
%         \\
%         0 & \text{else}
%     \end{cases}
%     \\
%     \left[\mathbf{A_0}\right]_{m'm}&=\begin{cases}
%         -\left[\mathbf{A_0}\right]_{m'm} & \text{if }\ m'=-m
%         \\
%         0 & \text{else}
%     \end{cases}
%     \end{split}
% \end{equation}


\subsubsection{Gaunt Tensor Product}
\HR{TODO: This section will review recently proposed Gaunt Tensor Product framework that reduces the complexity of C-G tensor product from $O(L^6)$ to $O(L^3)$}

\subsection{Wigner-Eckart Theorem of G-steerable Kernels}
\HR{TODO: This section will review the general theory and recipe for building equivariant neural networks for arbitrary Lie groups.}

\subsubsection{Peter-Weyl theorem}
\HR{TODO: Theoretical background for steerable functions on a compact Lie group and their homogeneous spaces.}

==> Old/Section5_GeometricImpedanceControl.tex <==
We introduce geometric impedance control (GIC) \cite{seo2023geometric, seo2024comparison} here and show that it serves as a SE(3) group equivariant control law. In this note, 
Furthermore, under the framework of variable impedance control, GIC can be considered as an SE(3) group equivariant force-based policy. The main contents of this section are already published in \cite{seo2024comparison}. Readers can consider this section as the more detailed explanation version of \cite{seo2024comparison}.

\paragraph*{Necessity of geometric formulation}
As can be seen in \eqref{eq:manipulator_dynamics}, the underlying coordinate of the manipulator is described in the joint space. However, as suggested in \cite{khatib1987unified}, the manipulator will execute a task on the workspace, i.e., end-effector space. Therefore, the task can be described more intuitively in the end-effector space. The pose of the end-effector can be calculated via forward kinematics (Sec~\ref{sec:Prelim}), and thereby, it can be well described by utilizing a group structure of SE(3). 

Conventional impedance control designs do not consider the full geometric structure of SE(3). For instance, the papers from the early stage of robot control \cite{hogan1985impedance, khatib1987unified} could be considered. In \cite{hogan1985impedance}, the end-effector coordinate $x \in \mathbb{R}^6$ is just utilized without explicitly mentioning its definition. To correctly define the rotational errors, many representations are studied in \cite{caccavale1999six}, including Euler-angle representation, axis-angle representation of SO(3), and quaternion representation. Similarly, in \cite{khatib1987unified}, the translational and rotational parts of the $x$ vector were separately considered. 

In this regard, by incorporating a full geometric structure of SE(3) into the control design, one can expect a further increase in performance. Moreover, as we are going to describe in the later part of this Section, the intuition for the equivariant force, velocity-based policy structures can be obtained. 

\subsection{Manipulator Dynamics}
\subsubsection{Manipulator Dynamics in joint space}
The manipulator dynamics in the joint space is written as follows.
\begin{equation} \label{eq:manipulator_dynamics}
    M(q)\ddot{q} + C(q,\dot{q})\dot{q} + G(q) = \tau + \tau_e,
\end{equation}
where $q\in\mathbb{R}^n$ is a joint coordinate in position, $\dot{q} \in \mathbb{R}^n$ is joint velocity, $\ddot{q}\in\mathbb{R}^n$ is joint acceleration, $M(q)\in\mathbb{R}^{n\times n}$ is inertia matrix, $C(q,\dot{q})\in\mathbb{R}^{n\times n}$ is Coriolis matrix, $G(q) \in \mathbb{R}^n$ is gravity force vector in joint space, $\tau \in \mathbb{R}^n$ is joint torque as a control input, and $\tau_e \in \mathbb{R}^n$ is external disturbance acting in the form of joint torque. 

\subsubsection{Manipulator Dynamics in Workspace on SE(3)}
As the task that the manipulator performs is done by the end-effector, it is often preferable to define the task in the workspace, not in the joint space. Thus, we are now interested in the framework that regards the operational space as $\SE$. 
Employing the operational space formula from \cite{khatib1987unified}, the manipulator dynamics using the body-frame velocity $V^b$ is given by:
\begin{align} \label{eq:robot_dynamics_eef}
    &\tilde{M}(q)\dot{V}^b + \tilde{C}(q,\dot{q})V^b + \tilde{G}(q) = \tilde{T} + \tilde{T}_e, \text{ where}\\
   & \tilde{M}(q)= J_b(q)^{-T} M(q) J_b(q)^{-1}, \nonumber\\
    &\tilde{C}(q,\dot{q})=J_b(q)^{-T}(C(q,\dot{q}) \!-\! M(q) J_b(q)^{-1}\dot{J})J_b(q)^{-1}, \nonumber\\
   & \tilde{G}(q)= J_b(q)^{-T} G(q),\; \tilde{T}= J_b(q)^{-T} T,\; \tilde{T}_e= J_b(q)^{-T} T_e.\nonumber,
\end{align}
where $J_b$ is a body-frame Jacobian matrix which relates body velocity and joint velocity by $V^b = J_b \dot{q}$. See \cite{seo2023geometric, seo2024comparison} for more details. 

\subsection{Error Functions: Distance-like metrics on SE(3)}
Lyapunov stability theory provides a foundation for describing the stability property of the given autonomous or control system. 
The key idea behind the Lyapunov stability theory is to represent the dynamics of a high-dimensional nonlinear ordinary differential equation (ODE) without solving it. Instead, the scalar function (Lyapunov function), which gets the state of the ODE as input, is defined, and the convergence property of the Lyapunov function is analyzed to describe the property of the original system. For the mechanical control system, total mechanical energy (potential energy + kinetic energy) is traditionally considered as the Lyapunov candidate \cite{koditschek1989application}. Here, the kinetic energy is composed of the velocity parts of the states, while the potential energy is composed of the position parts. It is quite straightforward to find out that the potential energy is closely related to the distance of two points, as the potential function and the distance metrics are both defined from the \emph{difference} of two points. 

Defining the difference between two points in Euclidean space is straightforward. Consider $x_1, x_2 \in \mathbb{R}^n$ in Euclidean space. Then, a \emph{vector} to describe the difference between two points can be considered as $v = x_1 - x_2$, and the Euclidean norm can be utilized to describe the distance, i.e., $d = \|v\|_2$.

On the other hand, the difference between the two points on the manifold (Lie group) is more subtle. Before we introduce the notion of difference in $\SE$, we need to respect the fact that the unit of the two elements $\SO$, $\mathbb{R}^3$ are not the same. Therefore, we have no choice but to use the notion of the \emph{error function}, $\Psi: \SE \times \SE \to \mathbb{R}$, instead of using the terminology of distance. For this reason, we will now use the word ``\textbf{error function}'' to describe the scalar variable between two elements on $\SE$ that works as the distance between two points.
There are two major ways to represent such error function on $\SE$ \cite{seo2024comparison}.
\begin{enumerate}
    \item SE(3) as a matrix group
    \item Property of Lie algebra (being a local chart of the manifold)
\end{enumerate}
Two different perspectives of error function lead to different perspectives of potential functions, resulting in different control laws. The former aspect leads to the definition of distance and potential function on the Lie group \cite{seo2023geometric, bullo1999tracking, lee2010geometric}, and the latter one leads to the potential function on the Lie algebra \cite{teng2022lie, bullo1995proportional}. Here, we will refer to the squared distance-like metric as an error function.

\subsubsection{Configuration Error}
Before we define the error function, we need to first have a notation to define the difference between two configurations. The transformation matrix between the desired $g_d = (p_d,R_d)$ and current configuration $g = (p, R)$ is defined as
\[
    g_{de} = g_d^{-1}g.
\]
We will call $g_{de}$ as the \emph{configuration error} and is utilized to define the error in the configuration in many of the geometric control literature, e.g., \cite{seo2023geometric, bullo1995proportional, lee2010geometric,bullo1999tracking,teng2022lie,lee2012exponential}.

\subsubsection{Error function from matrix group perspective}
One can just focus on the fact that a homogeneous matrix representation is nothing but a matrix. This concept was first proposed in \cite{koditschek1989application}, further developed in \cite{bullo1999tracking}, revisited in \cite{lee2010geometric}, and widely utilized thereafter, especially on SO(3), i.e., UAV field. In SO(3), a error function on this perspective $\Psi(R,R_d)$ is given by
\[
    \Psi(R,R_d) = \text{tr}(I - R_d^T R)
\]
However, what is overlooked from the error function $\Psi(R,R_d)$ is that it originates from the Frobenius norm. In the SO(3) case, the following equality holds \cite{huynh2009metrics}:
\begin{equation*}
    \Psi(R,R_d) = \text{tr}(I - R_d^T R) = \dfrac{1}{2}\text{tr} \left((I - R_d^T R)^T(I - R_d^T R)\right) 
\end{equation*}
The definition of the Frobenius norm, i.e., $\|A\|_F^2 = \text{tr}(A^T A)$, can be used to derive
\begin{equation} \label{eq:Frob_norm_SO3}
    \Psi(R,R_d) = \dfrac{1}{2}\|I - R_d^T R\|_F^2.
\end{equation}

Let us chew on \eqref{eq:Frob_norm_SO3}. When $R = R_d$, then $R_d^TR = I$; $\Psi(R,R_d) = \|0\|_F = 0$. Thus, what it means is that we first see the difference between two points in SO(3), compare the difference rotation matrix with the identity matrix, and quantify its discrepancy from the identity as the Frobenius norm. Recalling that the transpose operator in $\SO$ is the same as the inverse operator, one could extend \eqref{eq:Frob_norm_SO3} defined on $\SO$ to the $\SE$ as the following formula, which is also based on the Frobenius norm. 
\begin{align} \label{eq:Frob_norm_SE3}
        &\Psi_1(g,g_d) = \dfrac{1}{2}\|I - g_d^T g\|_F^2 \\
        &= \tfrac{1}{2} \tr\left((I - g_d^{-1}g)^T(I - g_d^{-1}g)^T \right) = \tfrac{1}{2} \tr (X^T X) \nonumber,
\end{align}
with $X$ is defined as
\begin{equation*}
    X = X(g,g_d) = \begin{bmatrix}
    (I - R_d^TR) & -R_d^T(p - p_d) \\
    0 & 0 
    \end{bmatrix} \nonumber
\end{equation*}
By further unraveling the equation, one can show that
\begin{equation} \label{eq:error_function_SE3}
    \Psi_1(g,g_d) = \tr(I - R_d^TR) + \tfrac{1}{2}(p - p_d)^T(p - p_d)
\end{equation}
Therefore, we can see that the error function in SE(3) is composed of SO(3) and $\mathbb{R}^3$ similar to the first perspective. 

\subsubsection{Error function from Lie algebra perspective}
The main intuition here is that the Lie algebra can be considered as the vector space of the SE(3) manifold. Note that Lie algebra is defined as the element on the tangent space of the identity. Thus, Lie algebra is vector space but not (necessarily) attached to the tangent space of the current configuration.  As we can see from the Euclidean space example, the first intuitive way to define distance is by using a vector.
In \cite{teng2022lie}, the Lyapunov candidate was proposed using this concept. The implication is that the proposed Lyapunov candidate function is actually a potential function (for the first-order system case), and if we remove the \emph{weights} in the potential, then it can be considered as the distance metric (squared). The vector representation $\xi_{de} \in \mathbb{R}^6$ of a difference between two configurations is defined as
\begin{equation}
    \xi_{de} = \log{(g_{de})}^\vee = 
    \begin{bmatrix}
        \hat{\psi}_{de} & b_{de} \\
        0 & 0
    \end{bmatrix}^\vee = \begin{bmatrix}
        b_{de} \\ \psi_{de}
    \end{bmatrix}
\end{equation}
where (See pp. 413-414 of \cite{murray1994mathematical})
\begin{align*}
    &\hat{\psi}_{de} = \log(R_d^TR), \quad b_{de} = A^{-1}(\psi_{de}) R_d^T(p - p_d)\\
    &A^{\text{-}1}(\psi) \!=\! I \!-\! \dfrac{1}{2}\hat{\psi} + \dfrac{2\sin\|\psi\| - \|\psi\|(1 + \cos\|\psi\|)}{2 \|\psi\|^2 \sin \|\psi\|} \hat{\psi}^2,
\end{align*}
when $\psi \neq 0$.
Note that the logarithm of the matrix is not unique \cite{Matrix_log_wiki}, and there are many alternative definitions, e.g., \cite{seo2024comparison, bullo1995proportional}
\begin{align*}
    A^{-1}(\psi) &= I - \dfrac{1}{2}\hat{\psi} + \left(1 - \alpha(\|\psi\|)\right) \dfrac{\hat{\psi}^2}{\|\psi\|^2},\\ &\text{with} \; \alpha(y) = (y/2)\cot{(y/2)}.
\end{align*}

As mentioned in \cite{bullo1995proportional}, the inner product on $\so$ is well defined and has desirable properties of positive definite and bi-invariant. The inner product of two elements $\hat{\psi}_1, \hat{\psi}_2 \in \so$ is defined using the Killing form, a bilinear operator defined by $\langle \cdot, \cdot \rangle _K: \so \times \so \to \mathbb{R}$, as \cite{park1995distance}
\begin{equation*}
    \begin{split}
        \langle\hat{\psi}_1, \hat{\psi}_2\rangle_{\so} &\triangleq -\tfrac{1}{4} \langle\hat{\psi}_1, \hat{\psi}_2\rangle_K, \;
        \langle\hat{\psi}_1, \hat{\psi}_2\rangle_K \triangleq \tr( \ad_{\psi_1} \ad_{\psi_2} ).
    \end{split}    
\end{equation*}
where $\ad$ is an adjoint (small adjoint) operator, where if $\psi \in \so$, $\ad_{\psi}= \hat{\psi}$.

In contrast, there is a negative result on $\se$: there is no symmetric bilinear form on $\se$ that is both positive definite and bi-invariant \cite{bullo1995proportional, park1995distance}.
Still, one can define a left-invariant inner product on $\se$ by exploiting the fact that $\se$ is isomorphic to $\mathbb{R}^6$. We will denote the inner product by $\langle \hat{\xi}_1, \hat{\xi}_2\rangle_{(P,I)}$, as follows \cite{park1995distance, teng2022lie, vzefran1996choice, belta2002euclidean}:
\begin{equation}
\label{eq:inner_product_se(3)}
    \langle \hat{\xi}_1, \hat{\xi}_2 \rangle_{(P,I)} = \xi_1^T P \xi_2
\end{equation}
where $\hat{\xi}_1, \hat{\xi}_2 \in \se$, and $P \in \mathbb{R}^{6\times 6}$ is symmetric positive definite matrix. 
The subscript $P$ in definition \eqref{eq:inner_product_se(3)} indicates that the inner product is equipped with the Riemannian metric $P$, while the subscript $I$ represents the fact that the Lie algebra $\se$ is a vector space tangent at the identity element of $\SE$. As can be clarified later, the introduction of these subscriptions is to fill the discrepancies between the definition of the inner product of Lie algebra and Riemannian metric; the inner product of the Lie algebra is defined literally on the Lie algebra, but the Riemannian metric is defined on the tangent space attached to each point on the manifold. 

Then, one can define the Riemannian metric on $\SE$ on the point $g \in G$,
using the inner product on $\se$ $\langle \cdot, \cdot \rangle_{(P,g)} : T_gG\times T_gG \to \mathbb{R}$, as follows. Consider two tangent \emph{vectors} (perturbation on the configuration manifold) on the tangent space at point g, $\delta g_i \in T_gG$, such that $\delta g_i = g \hat{\xi}_i$ with $\hat{\xi}_i = (\hat{\psi}_i, b_i)$ for $i = \{1,2\}$.
The Riemannian metric is then defined as \cite{park1995distance, vzefran1996choice, belta2002euclidean}
\begin{equation} \label{eq:Riemannian_metric}
    \langle \delta g_1, \delta g_2 \rangle_{(P,g)} \!=\! \langle g^{-1} \delta g_1, g^{-1} \delta g_2 \rangle_{(P,I)} = \langle \hat{\xi}_1, \hat{\xi}_2 \rangle_{(P,I)}
\end{equation}
The Riemannian metric defined in \eqref{eq:Riemannian_metric} is often referred to as a left-invariant Riemannian metric since $g^{-1} \delta g_i = \hat{\xi}_i$ is left invariant, i.e., for any arbitrary left transformation matrix $g_l$, $(g_l g)^{-1} (g_l g) \hat{\xi}_i = \hat{\xi}_i$. 

Finally, we can define an error function on $\SE$ from Lie-algebra perspective by letting $P = \tfrac{1}{2}I_{6\times6}$ as follows:
\begin{equation} \label{eq:error_function_SE3_algebra}
    \Psi_2(g,g_d) = \langle g_{de}\hat{\xi}_{de}, g_{de}\hat{\xi}_{de} \rangle_{\left(0.5I, g_{de}\right)} = \tfrac{1}{2} \|\psi_{de}\|^2 + \tfrac{1}{2}\|b_{de}\|^2
\end{equation}
where $\hat{\xi}_{de} = \log(g_{de}) = (\hat{\psi}_{de}, b_{de})$. 
\eqref{eq:error_function_SE3_algebra} can also be obtained by considering  $\SE$ as a general affine group, as done in \cite{belta2002euclidean}  and \cite{liu2013finite}. 

\subsection{Error Vectors on SE(3)}
\subsubsection{Positional Error Vectors on SE(3)}
\paragraph*{Geometrically Consistent Error Vector (GCEV)} GCEV was proposed in \cite{seo2023geometric} and serves as a positional error vector in SE(3). Note that this error vector formulation is derived from the Lie group-based error function. The error vector derivation on SO(3) was first proposed in \cite{lee2010geometric}. We first perturb a configuration $g \in SE(3)$ with a right translation in the direction of an arbitrary vector $\eta$, as was done in \cite{lee2010geometric} for $SO(3)$.
\begin{equation*}\begin{aligned}
    g_{\hat{\eta}}= g e^{\hat{\eta}\epsilon}\!, \quad \eta=\begin{bmatrix}\eta_1\\ \eta_2\end{bmatrix}\!\in\!\mathbb{R}^6 \implies \hat{\eta}\!\in\!se(3), \;\epsilon\!\in\!\mathbb{R},
\end{aligned}\end{equation*}
where $\eta_1, \eta_2\!\in\!\mathbb{R}^3$ refer to translational and rotational components, respectively. The perturbed configuration matrix $\delta g$ can be found by
\begin{equation*}
    \begin{split}
        \delta g &= \left.\dfrac{d}{d\epsilon}(g e^{\hat{\eta}\epsilon})\right|_{\epsilon=0} = \left. g \hat{\eta}  e^{\hat{\eta}\epsilon}\right|_{\epsilon = 0} = g \hat{\eta} \in T_gSE(3), \\
        &\implies \begin{bmatrix}
        \delta R & \delta p \\
        0 & 0 
        \end{bmatrix}  = \begin{bmatrix}
        R\hat{\eta}_2 & R \eta_1 \\ 0 & 0 
        \end{bmatrix}.
    \end{split}    
\end{equation*}
The perturbed error function $\delta \Psi(g,g_d)$ can be obtained and evaluated by
\begin{equation*} \label{eq:perturbation_of_error_metric}
    \begin{split}
    \delta \Psi(g,g_d)&=\dfrac{1}{2}\tr\begin{bmatrix}\!
    -\delta R^T R_d-R_d^T \delta R & \ast \nonumber
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(p-p_d)^T \delta p
    \end{bmatrix} \nonumber \\
    &=\!\dfrac{1}{2}\tr\begin{bmatrix}
    -\hat{\eta}_2^T R^TR_d-R_d^T R \hat{\eta}_2 & \ast
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(p-p_d)^T R \eta_1 
    \end{bmatrix}\nonumber \\
    &= -\tr(R_d^T R \hat{\eta}_2) + (p-p_d)^T R \eta_1 \nonumber \\
    &= (R_d^T R - R^T R_d)^\vee \cdot \eta_2 + (p - p_d)^T R \eta_1,
    \end{split}
\end{equation*}
where $\cdot$ is an inner product between two vectors.

We now define the \emph{position} error vector or Geometrically Consistent Error Vector (GCEV) $\eg$
as
\begin{equation}\begin{aligned}\label{eq:eg}
    \eg = \begin{bmatrix}
    e_p \\ e_R
    \end{bmatrix} = \begin{bmatrix}
    R^T(p - p_d) \\
    (R_d^T R - R^T R_d)^\vee 
    \end{bmatrix} \in \mathbb{R}^6,
\end{aligned}\end{equation}
so that $\delta \Psi(g,g_d) = \eg ^T \eta$ and
\begin{equation*}\begin{aligned}
    \hat{e}_g = \begin{bmatrix}
    R_d^T R - R^T R_d & R^T (p - p_d) \\
    0 & 0 
    \end{bmatrix} \in se(3).
\end{aligned}\end{equation*}

\paragraph*{Lie algebra-based Error Vector}
Similar to the way that the GCEV is derived from its Lie group-based error function, we can also derive the positional error vector from the Lie algebra-based error function. To put a conclusion, such a positional error vector is a log map of the configuration error $g_{de}$, \cite{teng2022lie}.

\subsubsection{Velocity Error Vector}
Velocity error vector should be defined properly on the SE(3) manifold, as the two tangent vectors $\dot{g} = g \hat{V}^b$ and $\dot{g}_d = g_d \hat{V}^b_d$ do not lie on the same tangent spaces. Specifically, for the Frobenius-norm-based error function, the desired velocity vector $V_d^b$ is translated using the following formula (See Ch 2.4 of \cite{murray1994mathematical} for the details of these steps, and \cite{seo2023geometric, lee2010geometric}): 
\begin{equation*}\begin{aligned}
    \hat{V}_d^* = g_{ed} \hat{V}_d^b g_{ed}^{-1}, \text{ where } g_{ed} = g^{-1}g_d.
\end{aligned}\end{equation*}
Then, it is straightforward to have in the vector form:
\begin{equation}\begin{aligned}\label{eq:Ad_velo}
    V_d^* = \text{Ad}_{g_{ed}}V_d^b, \text{ with } \text{Ad}_{g_{ed}} = \begin{bmatrix}
   R_{ed} & \hat{p}_{ed} R_{ed} \\ 0 & R_{ed}
    \end{bmatrix},
\end{aligned}\end{equation}
where $\text{Ad}_{g_{ed}}: \mathbb{R}^6 \to \mathbb{R}^6$ is an Adjoint map, $R_{ed} = R^T R_d$, and $p_{ed} =-R^T(p - p_d)$. 

Based on this, we define the \emph{velocity} error vector $\ev$ as 
\begin{equation}\begin{aligned} \label{eq:ev}
    \ev = \underbrace{\begin{bmatrix}
    v^b \\ w^b \end{bmatrix}}_{V^b} - \underbrace{\begin{bmatrix}
     R^TR_d v_d + R^T R_d \hat{\omega}_d R_d^T (p - p_d)\\
     R^T R_d \omega_d \end{bmatrix}}_{V_d^*} = \begin{bmatrix}
    e_v \\ e_\Omega \end{bmatrix}.
\end{aligned}\end{equation}

The interpretation of this Lie group-based derivation is as follows. First, the two tangent vectors $\dot{g} \in T_g\SE$ and $\dot{g}_d \in T_{g_d}\SE$ cannot be directly compared since they are lying on the different tangent spaces. Therefore, to compare the tangent vectors on the tangent space $T_g\SE$, $\dot{g}_d$ is first translated via right multiplication $g_d^{-1}g$. Note that this right multiplication action can be considered as pushforward mapping since the action is translating a tangent vector from one tangent space to another tangent space. 

On the other hand, the configuration error $g_{de}$ is directly interpreted as an element on the manifold $\SE$, and the time-derivative of $g_{de} = g_d^{-1}g$ is dealt with in \cite{teng2022lie} in the following way.
\begin{align*}
    \dfrac{d}{dt}(g_d^{-1}g) &=  g_d^{-1}\dot{g} + \dot{g}_d^{-1} g = g_d^{-1}\dot{g} -  g_d^{-1}\dot{g}_d g_d^{-1} g \nonumber \\
    &= g_d^{-1}g \hat{V}^b - g_d^{-1}g_d\hat{V}_d^b g_d^{-1}g \\
    &= g_d^{-1}g \left(\hat{V}^b - (g_d^{-1}g)^{-1}\hat{V}_d^b (g_d^{-1}g)\right) \triangleq g_d^{-1}g (\hat{e}_V) \nonumber\\
    \implies \dot{g}_{de} &= g_{de} \hat{e}_V \in T_{g_{de}}\SE\nonumber
\end{align*}
Notice that $g_{de} = g_d^{-1}g$, $g_{de}^{-1} = g_{ed}$, and $(g \hat{\xi} g^{-1})^\vee = \Ad_g\xi$, for $g \in \SE$ and $\xi \in \se$.

On the other hand, in Lie algebra-based formulation, the configuration error $g_{de} = g_d^{-1}g$ is directly interpreted as a component on $G \subset \SE$. The tangent vector is then directly derived on the tangent space $\dot{g}_{de} \in T_{g_{de}}\SE$, and it turns out that $\dot{g}_{de} = g_{de} \hat{e}_V$, leading to same velocity error formulation. 

Therefore, we conclude that although both approaches have different rationales, they share the same structure of velocity error vector, which leads to the same Kinetic energy function and the same impedance control law. We refer to the description from \cite{seo2024comparison} for the details of the velocity error vector.

\subsection{Energy Functions on SE(3)}
We consider two energy functions for our control design: potential energy function and kinetic energy function.

\subsubsection{Potential energy function} 
We interpret the potential energy function as a weighted distance metric. This concept is motivated by the potential energy of the spring in the Euclidean space. Consider a linear spring with one end attached to the origin $x_0 = 0 \in \mathbb{R}^3$ and the other end attached to $x \in \mathbb{R}^3$. Then, the potential energy stored in the spring can be written by 
\begin{equation*}
    P = \frac{1}{2} x^T K x = \frac{1}{2}\|x\|_K^2
\end{equation*}
where $K \in \mathbb{R}^3$ is a symmetric positive definite stiffness matrix, and the potential energy can be interpreted as the weighted 2-norm or weighted squared Euclidean distance. Recalling that we have derived the distance metric in $SE(3)$ in two different ways, we will define the potential functions on $SE(3)$ accordingly. 

\paragraph*{Potential Energy Function from Matrix Group Perspective} We weight the distance metric in \eqref{eq:Frob_norm_SE3} by first introducing a weighted matrix $X_K$ given by:
\begin{equation}
    X_K = \begin{bmatrix}
        \sqrt{K_R}(I - R_d^TR) & -\sqrt{K_p}R_d^T(p - p_d)\\
        0 & 0
    \end{bmatrix}
\end{equation}
where $K_p, K_R \in \mathbb{R}^{3\times3}$ are symmetric positive definite stiffness matrices for translational and rotational parts, respectively, and the square root of the matrix can be defined from the singular value decomposition. Note that the square root of the matrix is utilized to recover the original matrix in the potential energy form.
Then, the potential function $P_1(g,g_d)$ on Lie group SE(3) is defined in the following way:
\begin{equation} \label{eq:potential_lie_group}
    \begin{split}
        & P_1(g,g_d) = \tfrac{1}{2}\tr(X_K^T X_K) \\
        &\;\;= \tr(K_R(I - R_d^T R)) + \tfrac{1}{2}(p - p_d)^T R_d K_p R_d^T (p - p_d) 
    \end{split}
\end{equation}

\paragraph*{Potential Energy Function from Lie algebra perspective}
Given the inner product on $\se$ and the error function defined previously, the potential function from the Lie algebra perspective can be given as \cite{teng2022lie, seo2024comparison}:
\begin{equation} \label{eq:potential_lie_algebra}
    P_2(g,g_d) = \langle \hat{\xi}_{de}, \hat{\xi}_{de}\rangle_{(0.5K_\xi, I)} = \tfrac{1}{2}\xi_{de}^T K_{\xi} \xi_{de},
\end{equation}
where $P=\tfrac{1}{2}K_{\xi}$ and $K_\xi \in \mathbb{R}^{6\times6}$ is symmetric positive definite. Henceforth, we interpret $K_\xi$ as a stiffness matrix. We emphasize that $P_1(g,g_d)$ and $P_2(g,g_d)$ are left-invariant, positive definite, and quadratic. Left-invariance of these potential functions will be utilized later in this Section to prove the $\SE$-Equivariance. 

\subsubsection{Kinetic Energy on SE(3)}
The kinetic energy function on $\SE$ for the impedance control design can be formulated by using a velocity error vector $\ev$ and inertia matrix in the following form:
\begin{equation} \label{eq:kinetic_energy}
    K(t,q,\dot{q}) = \tfrac{1}{2}e_V^T \tilde{M} e_V,
\end{equation}

\subsection{Geometric Impedance Control}
We now introduce a geometric impedance control law (GIC) based on the potential and kinetic energy functions. The main idea behind the GIC is that the total mechanical energy function (potential + kinetic energy) should be dissipated over time. 

\subsubsection{Impedance Control as a Dissipative Control Law}
The total mechanical energy function, our Lyapunov function is defined as
\begin{equation} \label{eq:lyapunov}
    V_i(t,q,\dot{q}) = K(t,q,\dot{q}) + P_i(t,q), \quad i \in \{1,2\}
\end{equation}
where $K$ and $P_i$ are the kinetic and potential energy components of the Lyapunov function. Note that $P_1$ is given in \eqref{eq:potential_lie_group} and $P_2$ is in \eqref{eq:potential_lie_algebra}. The desired property of the impedance control to be dissipative control law \cite{kronander2016stability} is defined as
\begin{equation} \label{eq:dissipative}
    \dot{V}_i = -e_V^T K_d e_V
\end{equation}
where $K_d \in \mathbb{R}^6$ is symmetric positive definite damping matrix. 
To satisfy \eqref{eq:dissipative}, the impedance control laws for each potential function are
\begin{equation} \label{eq:control_law}
        \tilde{T}_i \!=\! \tilde{M}\dot{V}^*_{d} \!+\! \tilde{C}{V}^*_{d} + \tilde{G} \!-\! f_{_{G,i}} \!-\! K_d e_V, \;\text{for}\; i \in \{1,2\}
\end{equation}
where $f_{_{G,i}} \in \mathbb{R}^6$, $\hat{f}_{_{G,i}}\in \se^*$, are given respectively by
\begin{equation}
    \begin{split}
        f_{_{G,1}} &= \begin{bmatrix}
        f_p \\ f_R
        \end{bmatrix} = \begin{bmatrix}
            R^T R_d K_p R_d^T (p - p_d)\\
            (K_R R_d^T R - R^T R_d K_R)^\vee
        \end{bmatrix} \\ 
        f_{_{G,2}} &= K_\xi \xi_{de}.
    \end{split}    
\end{equation}
The derivation process of $f_{_{G,1}}$ is shown in \cite{seo2023geometric} and $f_{_{G,2}}$ in \cite{seo2024comparison}.
We can show that both control laws satisfy almost global asymptotic stability. We refer to \cite{seo2023geometric, seo2024comparison} for the details of such properties.

\subsubsection{Geometric Impedance Control is SE(3)-Equivariant Control}
One of the crucial advantages of the GICs is that the control law is $\SE$ equivariant if it is described on the spatial frame. In \cite{seo2023contact}, the GIC law with learning gain scheduling policy is proved to be equivariant if the gain scheduling policy is left-invariant. Without any gain scheduling law, i.e., fixed impedance gains, similar analysis is also possible. Take $f_{_{G,1}} : \SE \times \SE \to se^*(3)$ for example, the left-invariance of $f_{_{G,1}}(g,g_d)$ can be shown as follows:
\begin{align}
    &f_{_{G,1}}(g_lg,g_lg_d) \nonumber\\&= \begin{bmatrix}
        (R_l R)^T R_l R_d K_p (R_l R_d)^T (R_l p + p_l - R_l p_d - p_l)\\
        (K_R(R_l R_d)^TR_lR - (R_l R)^T R_l R_d K_R)^\vee
    \end{bmatrix} \nonumber \\
    &= \begin{bmatrix}
        R^T R_d K_p R_d(p - p_d)\\
        (K_R R_d R - R^T R_d K_R)^\vee
    \end{bmatrix} = f_{_{G,1}}(g,g_d),
\end{align}
Note that the elastic force $f_{_{G,1}}$ is described on the body-frame coordinate. Similarly for $f_{_{G,2}}$,
\begin{equation}
    \begin{split}
        f_{_{G,2}}(g_lg, g_lg_d) &= K_\xi \log{(g_l g_d)^{-1} (g_l g_e))} \\
    &= K_{\xi} \log{(g_d^{-1} g_e)} = K_{\xi}\xi_{de}.
    \end{split}
\end{equation}

Then, the feedback terms of the GIC law are $\SE$ equivariant if they are described in the spatial frame, as can be shown from Proposition 2 of \cite{seo2023contact}. We will skip the proof in this note, as it has already been proved in the paper. 
However, it is worth mentioning that a generalized recipe for the velocity and force-based policy to be $\SE$-equivariant can be obtained. According to \cite{seo2023contact}, such a general recipe is given by:
\begin{enumerate}
    \item The policy is left-invariant.
    \item The policy is described on the body-frame coordinate.
\end{enumerate}
Although in \cite{seo2023contact} only mentioned velocity and force-based policy, it can be trivially extended to displacement $\Delta g$ within a sampling period. 

==> Old/Section6_FutureWorks.tex <==
\subsection{Towards vision-to-force SE(3)-Equivariance}
\JS{TBD}
\subsection{Symmetry breaking in robotics and control systems}
\JS{TBD}

==> Old/Section7_Conclusions.tex <==
\JS{TBD}


==> Old_2024_1130/Section2_Preliminaries.tex <==
\subsection{Groups}

A group is defined by a set $\G$ along with a group product (a binary operator) $``\cdot"$  
that satisfies  the axioms:
\begin{itemize}
\item $\forall h, g \in \G$ we have $h \cdot g \in \G$ (Closure);
\item  $\exists \Id \in \G$  such that $\Id \cdot g = g \cdot \Id =  g$ (Identity); 
\item 
$\forall g \in \G$, $\exists$  $g^{-1} \in \G$ such that
$g^{-1} \cdot g = g\cdot g^{-1}= \Id$ (Inverse);
\item  $\forall g, h, f\in \G$ we have $(g \cdot h) \cdot  f = g\cdot (h\cdot f)$ (Associativity).
\end{itemize}

The translation group consists of the set of translation vectors in $\mathbb{R}^n$ equipped with the group product and inverse given by $g_1 \cdot g_2 = x_1 + x_2$ and $g^{-1}=(-x)$, for group elements $g_1=(x_1)$, and $g_2=(x_2)$.
The general linear group over $\Real$, denoted by  $GL(n, \mathbb{R})$ consists of the set of $n \times n$ matrices with real entries that can be inverted  $GL(n,\mathbb{R}):= \{ A \in \mathbb{R}^{n \times n} |\det (A) \neq 0\},$
together with the operation of matrix multiplication. With a stronger restriction that the determinant be positive real numbers, we have  $GL^+(n, \mathbb{R}):= \{ A \in \mathbb{R}^{n \times n} |\det (A) >0\}$, which is a subgroup of $GL(n, \mathbb R)$. A subgroup is a subset of a group $(H \subseteq G)$, which is itself a group that is closed under
the group operation of $G$.
 The unitary group is a  subset of $GL(n,\mathbb{C})$ that consists of  unitary matrices    
$U(n):=\{A \in \mathbb{C}^{n \times n} | AA^* = {\Id}\} \subset GL (n,\mathbb C),$
together with the matrix multiplication. The orthogonal group consists of  real matrices    
$O(n):=\{A \in \mathbb{R}^{n \times n} | AA^T = {\Id}\}$.
% With an additional constraint $\det (R)=+1$, the orthogonal group forms the rotation group, i.e., a special orthogonal group denoted by $G=SO(n)$. 
With an additional constraint $\det (R)=+1$, the special orthogonal group, denoted by $G=SO(n)$, can be produced. It is a Lie group\footnote{A Lie group is a continuous group that is also a
differentiable manifold.} that consists of the set of rotation matrices 
$\{ R \in \mathbb{R}^{n \times n} | R^TR=RR^T={\Id}, \det (R)=+1 \},$
  together with the group
product and inverse are given respectively by the matrix product and inverse 
  $g_1 \cdot g_2 := (R_1 R_2)$,  $g^{-1}:= (R^{-1})$ for $g_1=(R_1)$ and $g_2 = (R_2)$.
We now introduce the rotation-translation group, i.e., a special Euclidean motion group denoted by 
$SE(n)$. It consists of the set  $\mathbb{R}^n \times SO(n)$ of translation vectors in  $\mathbb{R}^n$ and rotations in $SO(n)$, together with the group product and inverse given respectively by
$g_1 \cdot g_2 = (R_1x_2 + x_1, R_1R_2)$ and  $g^{-1}=(-R^{-1}x, R^{-1}),$
where $g_1=(x_1,R_1)$ and $g_2=(x_2, R_2)$. \HA{I believe that the $SE(3)$ group is more accurately represented as a semi-direct product of $R^3$ and $SO(3)$, rather than a direct product.}

\subsection{Smooth Manifolds}
The concept of smooth manifolds is the foundation of differential geometry and resulting geometric algorithms. 
% Although reviewing all of the smooth manifold concepts is beyond the tutorial paper's scope, we have included a review of the smooth manifolds in Appendix~\ref{sec:appendix_smooth} for the completeness of contents and for the readers who hope to understand the details from the base.
Although an in-depth review of smooth manifold theory is beyond this paper's scope, we have included a brief introduction in Appendix~\ref{sec:appendix_smooth} for completeness of the paper and to aid readers in understanding the fundamentals.
% \JS{For the details of the smooth manifolds, please refer to the Appendix} \JS{We need to select which to survive}
% {\color{red}AK: Slightly awkward sentence, perhaps rephrase: Although an in-depth review of smooth manifold theory is beyond this paper's scope, we have included a review in Appendix~\ref{sec:appendix_smooth} for completeness and to aid readers in understanding the fundamentals}
\subsection{Lie Groups and Algebras}
\subsubsection{Lie Groups}
%Lie groups appear as symmetry groups of physical systems, and their Lie algebras, i.e., tangent vectors near the identity $\Id$,   can be viewed as infinitesimal symmetry motions.  
A Lie group is a continuous group that is also a differentiable manifold. It is a group equipped with a smooth structure that allows continuous transformations and compositions, preserving both the algebraic and geometric properties.  Lie groups play a fundamental role in various areas of mathematics and physics, serving as a framework to study symmetries and transformations in a continuous manner.

{\color{red}AK: Feels a little unclear; removing the first or second half might improve clarity}
Examples of Lie groups include the group of translations in $n$-dimensional space, the group of invertible $n \times n$ matrices with real entries, i.e., general linear group $GL(n,\Real)$, the group of rotations in $n$-dimensional space, i.e., $SO(n)$ and the special Euclidean motion group in $n$-dimensional space, i.e., $SE(n)$.

Lie groups emerge from symmetry groups governing physical systems, with their corresponding Lie algebras representing infinitesimal symmetry motions as tangent vectors in the vicinity of the identity element $\Id$.
% {\color{red} AK: Paragraph structure for the rest of this can be improved a little. Perhaps start with "For instance, the rigid body motion of links in a robotic arm can be modeled by a Lie group $SE(3)$ that captures its essential symmetries and the group's corresponding Lie Algebras which represent infinitesmal motions about the robots joints." rejected}
{\color{red} Reframe this paragraph from the beginning in the context of robotics; maybe start out with: "In robotics, Lie groups of rigid body motion, i.e, $SE(3)$, represent the symmetries in motion of various points on a robot while their Lie algebras, twists, capture the incremental movements of a system via its joints...."}
For instance, Lie groups concerning the rigid body motion, i.e., $SE(3)$, represent symmetries in such systems, while their Lie algebras, such as twists, capture infinitesimal motions. In robotics, twists, comprising linear and angular velocity components, represent small incremental movements of a system via robotic arm's joints. This elegant mathematical framework connects Lie groups, Lie algebras, and physical motions, offering a powerful tool to model symmetries and transformations in various robotic applications, which will be further explored in the following subsection.

{\color{red} Choi: It would be good to connect how these Lie groups and algebras connect our topics and pinpoint specific ones  and the corresponding sections in the paper.}

\subsubsection{Lie Algebra}

{\color{red} Choi: Let's make sure the notations here are compatible with ones in our paper. For examples, $Z$, $t$, $I_n$. We should make them all consistent by merging them with other existing notations and symbols or eliminating them if necessary. }

\JS{I guess we can still use $\Id$ here, as it notates identity on the Lie group, and the Lie group does not necessarily have a matrix representation. We can use identity matrix notation $I_n$ on the $\SE$ group though, with homogeneous matrix representation. I changed $Z$ with $X$, but a little bit reluctant with changing $\varepsilon$ to $t$, as $t$ strongly gives the notion of time, while $\varepsilon$ feels more like some small positive constant. }



{\color{red} Horowitz: I think that this entire definition using so called generators is coming from nowhere. For example $g(\epsilon,X) = \Id + \epsilon X$, not just $g(\epsilon)$. Maybe it should be $g(\epsilon X) = \Id + \epsilon X$. (Also, I think that $X$ must be left-invariant, i.e. $X \in T_{g(\epsilon X)} \G$a.) Can someone let me know where this came from? }

An element $g \in \G$  (Lie group) close to the identity $\Id$ can be denoted as $g(\epsilon) = \Id +\epsilon X$, where $\epsilon \in \Real$ is a small number and $X$ is called a generator.  The generator $X \in \fg$, where $\fg = T_{\Id} \G$ (i.e the tangent space of $\G$ at its identity element $\Id$). %is the Lie algebra of $\G$.  
$\fg$ can be viewed as the set of all infinitesimal transformations that are  generated by the Lie group, starting from $\Id$.
% These  infinitesimal transformations change the object only slightly.  
 To obtain a finite transformation, we repeat the infinitesimal transformation infinitely often, which can be represented as the limit of the product of  infinitesimal transformations 
\[g(t) = \lim_{N\rightarrow \infty}  \left ({\Id}  + \frac{t}{N}X \right )^N = \exp(tX).\] 

\JS{Where this derivations come from: JC: I could not find the original document but I found a similar derivations at (36)-(37) in \url{https://arxiv.org/pdf/2012.00834}. I also found (5-55) in \url{https://chaosbook.org/library/Chen5-2.pdf}. Both of them are like textbooks, and we  explain it in a similar fashion.}
%where  
%$Z$ is the generator that generates the finite transformation $g$. The generator is an element of the Lie algebra of the Lie group. The Lie algebra is the tangent space of the Lie group at $\Id$, 
 
% For example, the general linear  matrix Lie group $(GL(n), \cdot)$ is a Lie group for which the set $GL(n)$ is an analytic manifold (embedded in a higher $n^2$-dimensional Euclidian space)
% where  each $g \in GL(n)$ is an $n \times n$ nonsingular matrix. The group operation $\cdot$  is matrix multiplication,
% and the mappings $g_1 \cdot g_2$ and $g^{-1}$ are both analytic.
For example, for the general linear matrix Lie group  $GL(n, R)$, the set  of invertible real $n \times n$ matrices, 
%and is an analytic manifold  (embedded in a higher $n^2$-dimensional Euclidian space), 
elements sufficiently close to the identity, $\Id = I_n$ can be written utilizing the matrix exponential function 
\begin{equation}\label{eq:exp}
% g(t) =  \exp_m(tX)=\sum_{k=0}^{\infty} \frac{(tX)^k}{ k!},
g(t) =  \exp(tX)=\sum_{k=0}^{\infty} \frac{(tX)^k}{ k!},
\end{equation}
for $X \in \fgl$, where  $\fgl = T_{I_n} GL(n)$ is the Lie algebra of $GL(n)$. 
%Therefore, one can define
For
any real $n \times n$  matrix  $X \in \fgl(n)$, its matrix exponential $\exp(X)$ is   defined by  the series in \eqref{eq:exp}.
The exponential   maps $X \in \fgl(n)$ into $\exp(X) \in GL(n)$.
The matrix
Lie algebra $\fg$  is  the set of all matrices $X$   such that the exponential of each $tX$ results in an element of $GL(n)$, i.e., 
\[
\fg= \{ X \in \fgl (n) | \exp(tX) \in GL(n), \forall t \in \Real \}.
\]

Let 
${\G}$ be a Lie group (i.e., a smooth manifold) and let 
$q \in  {\G}$. Let 
${\displaystyle T_{q}{\G}}$ be the tangent space at 
$q$. {\color{red} SML: Explain dual space?} \JS{Defined at the Appendix, add the reference Appendix} The cotangent space at $q$ is then defined as the dual space of 
${\displaystyle T_{q}{\G}}$:
${\displaystyle T_{q}^{*}\!{\G}=(T_{q}{\G})^{*}}$. Thus,
 $\fg=T_{\Id} \G$ and $\fg^*=T_{\Id}^*\G$ denote the Lie algebra (i.e., the tangent space of the  Lie group $\G$ at  $q=\Id$) and its dual, respectively (see Fig.~\ref{TG}). {\color{red} SML: I find this section hard to grasp and read. Similar notations and terms appear frequently, which make it hard to distinguish.}

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{./Figures/TG} 
\vskip -0.5pc
\caption{Illustration of   a Lie group $G$ and its tangent spaces.
The Lie algebra $\fg = T_{\Id}G$ is the tangent space at the identity $\Id$.
}\label{TG}
\end{center}
%\vskip -1.5pc
\end{figure}

\subsubsection{Lie Bracket}
 A Lie algebra $\fg$ is a vector space equipped with a Lie bracket operation
$[ \cdot, \cdot ] : \fg \times \fg \rightarrow \fg$ which is bilinear, anti-symmetric, $[a, b] = -[b, a]$, and satisfies the
Jacobi identity
$[a, [b, c]] + [b, [c, a]] + [c, [a, b]]=0.$ 

Let $\mathfrak{X}$ represent the set of smooth vector fields on $\G$. For any smooth function $f :\G\rightarrow \Real$,   the Lie bracket $[\cdot,\cdot]:\mathfrak{X} \times \mathfrak{X}\rightarrow \mathfrak{X}$ is then defined such that $[X,Y](f) := X(Y(f))-Y(X(f))$.

\subsubsection{Exponential Map and Logarithm Map}
\paragraph*{Exponential Map} The exponential map, $\exp: \fg \rightarrow \G$ is a local diffeomorphism defined by {\color{red} SML: diffeomorphism and isomorphism are mentioned before being defined. Define homeomorphism?} 
 \[
 \exp(X):=\gamma(1),
 \] 
 where $\gamma: \Real \rightarrow \G$ is a continuous group homomorphism with $\dot \gamma(0)=X$. 



{\color{red} Choi: Let's make sure the notations here are compatible with ones in our paper---check with hat map--how the way it is used.  }

 Define the isomorphism of the hat-map such as
 \[
 \widehat{(\cdot )}: \Real^n \rightarrow \fg,
 \]
 that maps a vector in $\Real$ to $T_{\Id} \G$. Its inverse map vee-map is defined as
 \[
 (\cdot )^\vee: \fg : \rightarrow \Real^n.
 \]
 For $X \in \fg$, the Lie exponential can be denoted by
map as
\[
\exp(\cdot): \Real^n \rightarrow \G, \quad \exp(X)=\exp_m(\widehat{X}),
\]
 where $\exp_m(\cdot)$ is the exponential of square matrices.
 The exponential map takes an element of the Lie algebra in $\fg =T_{\Id} \G$ and produces an element
of the Lie group $\G$ such as $\exp: \fgl(n) \rightarrow GL(n)$, i.e.,  $\exp(X=\log(g)) = g$.  
\paragraph*{Logarithm Map}
On the other hand, the  logarithm does the opposite $\log: GL(n)\rightarrow \fgl(n)$, i.e., 
$\log( g=\exp X) = X$ (see Fig.~\ref{TG}). 

In summary, we have
\[
\begin{split}
\exp(X)&=\exp_m (\widehat{X}) =g,\\
\log(g)&=\log_m(g)^\vee =X,
\end{split}
\]
where $\exp_m(\cdot)$ and $\log_m(\cdot)$ are the matrix exponential and logarithm, respectively. 

\subsubsection{Group Representations} \label{sec:group_representations}
Before introducing group representation, we first introduce special morphisms frequently utilized in Lie Group theory. 
\paragraph*{Diffeomorphisms}
Given two manifolds 
$M$ and $N$, a differentiable map ${ \phi \colon M\rightarrow N}$ is called a diffeomorphism if it is a bijection and its inverse 
${\phi^{-1}\colon N\rightarrow M}$ is differentiable as well.

{\color{lightgray} SML: 
\paragraph*{Homeomorphisms}
Given two topological spaces $X$ and $Y$, a continuous map ${ \phi \colon X\rightarrow Y}$ is called a homeomorphism if it is a bijection, continuous, and its inverse ${ \phi^{-1} \colon X\rightarrow Y}$ is also continuous. 
}

\paragraph*{Homomorphisms}
A homomorphism is a mapping from one group to a subset of another, $\phi: (G, \circ) \rightarrow (H, \hat \circ)$ such that
\[
\phi(g\circ h) = \phi(g) \, \hat \circ \,  \phi (h).
\]
With $h=\Id,$  we see that 
$\phi(g) = \phi(g\circ \Id) = \phi(g) \, \hat \circ \,  \phi(\Id),$ and
therefore,  $\phi(\Id)=\Id_H$ is  the identity in $H$.

\paragraph*{Isomorphisms}
A homomorphism is an isomorphism if and only if it is bijective. 

\paragraph*{Automorphism}
An automorphism is an isomorphism from a structure to itself.

\paragraph*{Group Representation}
If a linear map is a bijection then it is called a linear isomorphism.
Assume that $V$ is an $n$-dimensional vector space over $\Real$. We define 
\[GL(V ) = \{ A : V \rightarrow V\; |\; A \text{ is a linear isomorphism} \}  \]

Let $\G$ be a Lie group and $V \in \Real^n$ is a vector space. 
A representation of a Lie group is a map $D: \G \rightarrow  GL(V )$ of Lie groups. The representation $D$ acting on the vector space $V$ has the following property:
\begin{equation}
    D(g) D(h) = D(gh) \quad \forall g,h \in \G
\end{equation}
 Two different representations $ {D}$ and $ {D}'$ are said to be of \textit{equi\underline{valen}ce} (not   \textit{equi\underline{varian}ce})
 if there exists a non-degenerate change of basis $ {U}$ such that
 \begin{equation}
      {D}'(g)= {U} {D}(g) {U}^{-1}, \quad\forall g\in \G
 \end{equation}
Note also that a representation is said to be \textit{reducible} if there exists a change of basis such that the representation can be decomposed (block-diagonalized) into smaller subspaces. An \textit{irreducible representation} is a representation that cannot be reduced anymore. 

\paragraph*{Lie Group Left and Right Translations}
Note first that what we are referring to as translation in this section is different from a translational motion used in  rigid-body kinematics and dynamics.
Let $g, h \in \G$ be elements of a Lie group $\G$. We define the left translation of $\G$ by $g$ as the map
$L_g : \G \to \G,$ such that  $L_g(h) = gh$,  $\forall h \in \G$, and right translation as the map $R_g: \G \to \G$, such that $R_g(h) = hg$, $\forall h \in \G$. 

Notice that 
\[L_g^{-1} (h)=L_{g^{-1}}(h) \text{ and  } R_g^{-1} (h)=R_{g^{-1}}(h)\]
 since $L_g (L_g)^{-1} (h)=g (g^{-1})h=h$ and  $R_g (R_g)^{-1} (h)=h g (g^{-1})=h.$ 
Henceforth, both $L_g$ and $R_g$ are diffeomorphisms.  In addition, they commute with each other, i.e., $L_g R_h=R_h L_g$.

A left-invariant vector field $X \in T G$, where $TG$ is the tangent bundle of $G$ (See Appendix~\ref{sec:appendix_smooth}), satisfies 
\[
X(gh)=dL_g(h) X(h), 
\]
where $dL_g(h)$ is the differential (tangent map) of $L_g$  evaluated at $h$. If $h=\Id,$ the identity, then $X(g)=dL_g(\Id) \zeta,$ where $\zeta=X(\Id).$

\subsubsection{Adjoint Representations}
Due to smooth  multiplication and inverse maps,
 $L_g$ and $R_g$ are diffeomorphisms.
The inner automorphism $R_{g^{-1}} \circoo L_g= R_{g^{-1}}L_g$  is then given by  
$\Psi_g(h)=R_{g^{-1}}L_g(h)
 = ghg^{-1}.$

\paragraph*{Adjoint Representation of Lie group $\G$}
The derivative of $\Psi_g=R_{g^{-1}} L_g$ at the identify $\Id$ i.e.,   $d\Psi_g(\Id): \fg \to \fg$  is an isomorphism of Lie algebras, denoted by $\Ad_g: \G \times GL(\fg) \to GL(\fg)$.

Given an element $X \in \fg$ of the Lie algebra and $g \in \G$ of the Lie group, the large adjoint (Adjoint) operator is then obtained as
\[
\begin{split}
\Ad_g X &:= \frac{d}{dt} (g \cdot \exp(tX) \cdot g^{-1})|_{t=0}\\
&= \frac{d}{dt} \exp (t g Xg^{-1}) |_{t=0} \\
&=gXg^{-1}.
\end{split}
\]
The large adjoint representation of $\G$ gives a homomorphism from the group $\G$ into the set of all invertible linear transformations of $\fg$ onto itself.  
% For all $g \in \G$, and all $X \in \fg$ we have $\Ad_g X=gXg^{-1}.$
This  Lie
algebra isomorphism enables change of frames (see Fig~\ref{fig:Adjoint}).

Note that in the robotics community, a large adjoint representation is often interpreted as a linear operator in $\SE$, i.e., $\Ad_g: \SE \times \Real^6 \to \Real^6$, where $\Real^6$ is an isomorphic vector space of $\fg \in \se$ and $g \in \SE$. Although it might be confusing, as both adjoint representations are one-to-one, we will not distinguish their notations.

 \paragraph*{Adjoint Representation of Lie algebra  $\fg$}
 The derivative of $\Ad$ at the identity $\Id$, i.e.,  $d(\Ad_{\Id}): \fg \rightarrow \fgl(\fg)$  is the map of Lie algebras, denoted by
  $ad: \fg \rightarrow \fg(\fg)$ called the adjoint representation of $\fg$ with 
\[\ad_X Y=[X,Y].\]

The relationship between $\Ad$ and $\ad$ is given by
\[\Ad_{(\exp tX)}=\exp_m(t \cdot \ad_{(X)}).\]
(as we have $g=\exp (X)$.)

The summary of  Lie algebra and Lie group and their adjoints is illustrated in Fig.~\ref{fig:Summary}.

\begin{figure}[!t]
    \centering
    \centering
    \resizebox{0.9\columnwidth}{!}{
    \input{Figures/Summary.tex}}
    \caption{Summary of Lie algebra and Lie group and their adjoints that take an element of Lie algebra for $(\cdot)$.
    }\label{fig:Summary}    
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\columnwidth]{Figures/adjoint_2.png}
    \caption{An illustration of   a Lie group $\G$ and its Lie algebra  $\fg$ of the tangent space at $\Id$.
    The  Adjoint  of $g$ applied on an element of $\fg$, i.e.,  $v=\frac{d}{ds} \gamma(s)|_{s=0}$ is illustrated.    Note that $Ad_g v \in \fg.$
     $\Psi_g(\Id)=g\Id g^{-1}=\Id$
    implies  that any curve $\gamma(s)$ through $\Id$
     on $\G$
     is mapped by this homomorphism $\Psi_g$ to another  curve  $g \gamma(s) g^{-1}$ on  $\G$ through $\Id$.
     }
     \label{fig:Adjoint}
\end{figure}
The derivative of $L_{g^{-1}}$ at $g$ is a linear
map  from   $T_g \G$ to  $T_\Id \G=\fg$ because $L_{g^{-1}}g=g^{-1}g=\Id$.
Given a differentiable curve $g(t)$ on $\G$ with its velocity $\dot g(t):=\frac{d g(t)}{dt}$, the left differential of $L_{g^{-1}}$, i.e., $dL_{g^{-1}} : T_g \G \rightarrow \fg$ maps $\dot g$ to an element $\fg$ such as 
% {\color{red} SML: add or take out parenthesis to make them look aligned? 
% \[dL_{g^{-1}} (g)(\dot g)\] and 
% \[dR_{g^{-1}}(g) \dot g\]}
\[dL_{g^{-1}}(\dot g) =g^{-1} \dot g \in \fg.\]
Similarly, the right differential can be defined as 
\[dR_{g^{-1}}(\dot g)=\dot g g^{-1} \in \fg.\]

In the next section, we  show that for $g\in SE(3)$,  $g^{-1} \dot g$ and $\dot g g^{-1}$  represent body and spatial velocities, respectively.

\paragraph*{Inverse and Composition Rules}
Recall that $\Ad_g$ can be defined by the inner automorphism $\Psi_g(h) = R_{g^{-1}} L_g(h) = ghg^{-1}$. The adjoint representation is  linear and acts on the Lie algebra $\mathfrak{g}$ of $\G$ defined as:
\[
\Ad_g: \mathfrak{g} \rightarrow \mathfrak{g}, \quad \Ad_g(X) = d(\Psi_g)_\mathrm{\Id}(X),
\]
where $X$ is an element of the Lie algebra $\mathfrak{g}$. 

For $g, h \in \G$, we see that  $(\Psi_g)^{-1}$ shall satisfy  
\[
   \begin{split}
(\Psi_g) (\Psi_g)^{-1}h&=g [ (\Psi_g)^{-1}h] g^{-1}=h,\\
  (\Psi_g)^{-1} (\Psi_g) h&= (\Psi_g)^{-1}  g h g^{-1}=h.
  \end{split}
\]
Therefore, we have
\[
(\Psi_g)^{-1}= \Psi_{g^{-1}}.
\]

For $g, h, k \in \G$,  the composition rule  of inner automorphisms is given by 
\[\Psi_{gh (k)}=\Psi_{g}  \Psi_{h} (k),\]
which shows the homomorphism.{\color{red} } This can be shown as follows:
\[
    \begin{split}
    \Psi_{g}  \Psi_{h} (k) &=   
    \Psi_g( \Psi_h (k))\\
    &=R_{g^{-1}}L_g( \Psi_h (k))
     = g  \Psi_h (k) g^{-1}= g h k h^{-1}g^{-1}\\
     &=(gh)k (gh)^{-1}=
    \Psi_{gh}(k).
    \end{split}
\] 

For $X \in \fg,$ we see that $(\Ad_g)^{-1}$ needs to satisfy 
\[
    \begin{split}
(\Ad_g) (\Ad_g)^{-1}X&=g [ (\Ad_g)^{-1}X] g^{-1}=X,\\
  (\Ad_g)^{-1} (\Ad_g) X&=(\Ad_g)^{-1} g X g^{-1}=X.
    \end{split}
\]

As a result, similar to the previous case, we have
\[
(\Ad_g)^{-1}= \Ad_{g^{-1}}
\]

The Adjoint composition rule  can be given by
\begin{equation}\label{eq:Adchain}
 \Ad_{g} \Ad_{h}(X) = \Ad_{gh}(X)   
\end{equation}
 for arbitrary $X$ in the Lie algebra $\mathfrak{g}$.

This can be shown by
\[
\Ad_g \Ad_h(X) = g(hXh^{-1} )g^{-1} = (g h)X(gh)^{-1}= \Ad_{gh}X,
\]
which shows that $Ad_{(\cdot)}$ is a homomorphism.

\paragraph*{Adjoint Representations and Translations}
$\Psi_g(\Id)=g\Id g^{-1}=\Id$
implies that any curve $\gamma(s)$ through $\Id$
on $\G$
is mapped by this homomorphism $\Psi_g$ to another curve $g \gamma(s) g^{-1}$ on $\G$ through $\Id$ (see Fig.~\ref{fig:Adjoint}). 

The adjoint representation ($\Ad_g =d \Psi_g (\Id) $) maps any tangent vector $v$ in $\fg=T_{\Id}\G$
 to another tangent vector $Ad_g v=gvg^{-1}$ in $T_{\Id} \G$ while  $L_g$ or $R_g$
 maps tangent vectors in $T_{\Id} \G$  to tangent vectors in $T_{g} \G$ (see Fig.~\ref{fig:Adjoint}). 
 {\color{red} SML: Is this part "while  $L_g$ or $R_g$ maps tangent vectors in $T_{\Id} \G$  to tangent vectors in $T_{g} \G$" also shown in the figure?}

\subsubsection{Lie Derivatives on a Function}
Let $X \in \fg$, the Lie algebra of the Lie group $\G$, and let $f: \G \rightarrow \Real$ be analytic. 
We define the Lie derivative of a function $f(g)$ on the Lie group, i.e., $\forall g \in \G$, with respect to $X$ as follows:
\begin{equation} \label{eq:lie_deriv_group}
    \begin{split}
        \Lie_X f(g) &:= \lim_{t \rightarrow 0} \frac{f(g \exp(tX)) -f(g)}{t}\\
        &= \frac{d}{dt}    f(g  \exp(tX)) \bigg |_{t=0}.
    \end{split}
\end{equation}
Note that the definition of Lie derivative here is referred to as a right-Lie derivative from \cite{chirikjian2011stochastic}. It is also mentioned in \cite{chirikjian2011stochastic} that the right-Lie derivative is often mentioned as left-Lie derivative, as it is invariant to the translation acting on the left, i.e., left-invariant. As we are interested in the left-invariant Lie derivative, we will only consider the form \eqref{eq:lie_deriv_group} as our Lie derivative. 
% We define 
% \JS{DECIDE What to do}
% \paragraph*{Left-Lie derivative} \JS{Right-invariant}
% $\forall g \in \G$, the left Lie derivative of  $f(g)$ with respect to   $X$, is defined by \cite{chirikjian2011stochastic} as
% \[
% \begin{split}
%  \mathcal{L}_X^l f(g)&= \tilde X^l f (g)\\
% &:=\lim_{t \rightarrow 0} \frac{f( \exp(-tX) g)   -f(g)}{t}\\
%  &=\frac{d}{dt}  f(\exp(tX)   g) \bigg |_{t=0}.
%  \  \end{split}
%  \]  
% \paragraph*{Right-Lie derivative} \JS{Left-invariant}
%  Similarly, 
%  $\forall g \in \G$, the right  Lie derivative of  $f(g)$ with respect to   $X$, is defined by \cite{chirikjian2011stochastic} as
% \[
% \begin{split}
%  \mathcal{L}_X^r f(g)&=\tilde X^r f (g)\\
%  &:=\lim_{t \rightarrow 0} \frac{f(g \exp(tX)) -f(g)}{t}\\
%  &=\frac{d}{dt}    f(g  \exp(tX)) \bigg |_{t=0}.
%  \  \end{split}
%  \]  

% \subsubsection{Left-Regular Representation} \label{sec:left_regular_representation}

% \JS{This needs to be redefined or moved elsewhere
% JC: We can move it to where it is used later.
% }
% A useful way to let a group $\G$ act on functions is through left-regular representations. In this case, a function is transformed by transforming the domain $\mathcal{X}$ by the action of the group $\G$ on $\mathcal{X}$.
% The left-regular representation of $g \in \G$ acting on $f(x)$ with $x \in \mathcal{X}$ is defined by
% \begin{equation}\label{eq:left}
% L_g(f)(x) = g \circoo  f(x)= f(g^{-1} \circoo x)
% \end{equation}
% where $\circoo$ denotes the action of the group $\G$ on the appropriate domain or codomain.
% $f\in \mathbb{L}^2(\mathbb{R}^2)$ is a square-integrable function.

% \JS{Need to be reviewed from here}
% The left-regular representation of a Lie group G can be represented using pushforward notation in the view of smooth manifolds.
% Let $G$ be a Lie group, and let $L: G\rightarrow Diff(G)$ be the left-regular representation of $G$ given by
% \[L_g(h) = g \cdot h, \forall g, h \in G\]
% with $\cdot$ being the group operation in G.
% The pushforward notation for the left-regular representation is given by:
% \[L_*: T_e G \rightarrow X(G)\]
% where $T_eG$ is the tangent space to G at the identity element $e$, and $X(G)$ is the space of smooth vector fields on $G$.
% The pushforward $L_*$ is defined by:
% \[L_*(v)_g =  \left (\frac{d}{dt} \right ) \bigg |_0 L_g(\exp(tv))\]
% where $v$ is a tangent vector at the identity element e, and $\exp(tv)$ is the one-parameter subgroup of $G$ generated by $v$. The pushforward $L_*$ assigns to each tangent vector $v$ at the identity element e a vector field $L_*(v)$ on $G$, which is a left-invariant vector field.

% Therefore, the left-regular representation of a Lie group G can be represented as a pushforward notation using the pushforward map $L_*$.

% In other words, the left-regular representation of SE(2) acts on functions by transforming their arguments in the opposite direction of the group element $g$. This means that if we apply a transformation $g$ to the domain of a function $f$, we can obtain the transformed function $L_g(f)$ by applying the left-regular representation of $SE(2)$ to $f$.
% \JS{To here}

% For example, the left-regular representation of $SE(2)$ is an important tool in the study of group representations and equivariant neural networks, as it allows us to generalize the convolution operation of CNNs to equivariant group CNNs by replacing the usual convolution kernels with group-equivariant kernels that transform according to the left-regular representation of the group, which will be discussed in the next section. 

\subsection{Special Euclidean Group SE(3)}
In this subsection, we focus on the Special Euclidean Group $SE(3)$ as it is widely utilized in robotics applications. Although there are many other well-written robotics references, such as \cite{lynch2017modern}, we will follow the notations of \cite{murray1994mathematical} for unity in notations. Note also that the reference of this subsection is \cite{murray1994mathematical}.

\subsubsection{Lie Group Properties of $SE(3)$}
\paragraph*{Rigid Body Motions in $SE(3)$}
Let us consider the position and orientation of a coordinate frame B attached to the rigid body relative to an
inertial frame A (see Fig.~\ref{fig:SE(3)}).

\begin{figure}[!t]
\centering
\resizebox{\columnwidth}{!}{
\input{Figures/Coordinate_frame.tex}}
\caption{Coordinate frames $\{A\}$ and $\{B\}$ for specifying rigid motions.}
\label{fig:SE(3)}
\end{figure}

The configuration space of the system is denoted by the special Euclidean group, i.e.,  $SE(3)$  that consists of the pair $(p \in \Real^3, R \in SO(3))$, which is the product space of $\Real^3$ and  $SO(3)$. \HA{I believe that the $SE(3)$ group is more accurately represented as a semi-direct product of $R^3$ and $SO(3)$, rather than a direct product.} \JS{This is true, but then we need to define semi-direct product, do we want to do this?}
\HA{I think this is quite important. So, if there is enough blank space in the paper, I can write about it. (maybe near the section 2.1)}
\[
\begin{split}
SE(3) &= \{( p, R) : p\in \Real^3, R\in SO(3) \}\\
 &= \Real^3 \times SO(3). 
\end{split}
\]
An element $g = (p, R)\in SE(3)$ informs  
both a specification of the configuration of a rigid body and a transformation taking the coordinates of a point from one frame to another.
{\color{black}
For example, $g_{ab} = (p_{ab}, R_{ab})\in SE(3)$ is the specification of the configuration of
the B frame relative to the A frame. We may also write
$g(q)$ to denote the action of a rigid transformation on a point,
$g(q) = p + Rq,$ so that $q_a = g_{ab}(q_b).$

Given $q_b$, we can find $q_a$ by a transformation of
coordinates such that
\[q_a = p_{ab} + R_{ab}q_b,\]
where $q_a$ and $q_b$ are   the coordinates of a point $q$ relative to frames
A and B, respectively.}

\paragraph*{Homogeneous Matrix Representation in 
$SE(3)$.}
The $4 \times 4$ matrix $\bar g_{ab}$ is referred to as  the homogeneous representation of $g_{ab} \in
SE(3)$
\[
\bar q_a:= \left[
\begin{array}{c}
 q_{a}   \\
     1 
\end{array}
\right]
 =
\left[
\begin{array}{cc}
  R_{ab}    &  p_{ab}  \\
 0 & 1   
\end{array}
\right]
 \left[
\begin{array}{ccc}
 q_{b}   \\
     1 
\end{array}
\right]
=:\bar g_{ab} \bar q_b.
\]
%
The coordinate of  $q$ with respect to frame B can be represented with respect to  frame A by
\[
\bar q_a = \bar g_{ab} \bar q_b.
\]
Without subscripts, if $g = (p, R)\in SE(3)$, we have  its homogeneous representation 
\[
\bar g=\left[
\begin{array}{ccc}
  R    &  p  \\
 0 & 1   
\end{array}
\right]  \in
SE(3).
\]

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.70\columnwidth]{./Figures/coordinate_transformation.png} 
\vskip -0.5pc
\caption{Rigid body motion generated by rotation about a fixed axis.
}\label{fig:Motion}
\end{center}
\vskip -1.5pc
\end{figure}

{ \color{lightgray}
Consider the rotational motion of a rigid body about a line in the $z$-direction through $(0, l_1, 0) \in \Real^3$, as shown in Fig.~\ref{fig:Motion}.
The orientation of the coordinate frame B relative to frame A  is given by
\[
R_{ab}=
\left[
\begin{array}{ccc}
 \cos \theta &  -\sin \theta  &  0  \\
 \sin \theta &  \cos \theta  &  0 \\
 0 &  0  &   1
\end{array}
\right]
\]
The coordinates of the origin of frame B relative to frame A are given by
\[
p_{ab}=\left[
\begin{array}{c}
0  \\
 l_1   \\
 0  
\end{array}
\right].
\] 
The homogeneous representation of the configuration of the rigid body is then given by
\[
\bar{g}_{ab}=\left[
\begin{array}{cc}
  R_{ab}    &  p_{ab}  \\
 0 & 1   
\end{array}
\right]
=
\left[
\begin{array}{cccc}
 \cos \theta &  -\sin \theta  &  0 & 0 \\
 \sin \theta &  \cos \theta  &  0 & l_1 \\
 0 &  0  &   1 & 0\\
  0 &  0  &   0 & 1
\end{array}
\right].
\]
}
{\color{lightgray}
Rigid body transformations may be composed to form a new rigid body
transformations. Let $g_{bc} \in SE(3)$ be the configuration of a frame C
relative to a frame B, and $g_{ab}$ the configuration of frame B relative to
another frame A. Using the following composition rule, the configuration of C
relative to frame A is given by
\[
\bar g_{ac}=\bar g_{ab} \bar g_{bc}
= \left[
\begin{array}{ccc}
  R_{ab} R_{bc}   &  R_{ab} p_{bc}+ p_{ab}  \\
 0 & 1   
\end{array}
\right]
\]
since $\bar q_a=\bar g_{ab} ( \bar   q_b =\bar g_{bc} \bar   q_c)$  gives 
 \[\bar q_a=\bar g_{ab}  \bar g_{bc}   \bar q_c= \bar g_{ac} \bar q_c.\]

As can be seen from the example above, rigid body transformations may be composed iteratively  such that
 \[\bar q_a=\bar g_{ab}  \bar g_{bc}   \cdots \bar g_{op}  \bar q_p= \bar g_{ap} \bar q_p.\]}

For the rest of the paper, we will now denote the homogeneous matrix representation of $\SE$ $\bar g$ as $g$. Similarly, we will also denote the coordinate transformation of the point as $q_a = g_{ab} q_b$.

Using the homogeneous
representation,  the set of rigid transformations is shown to be 
a group.
\begin{itemize}
\item If $g_1, g_2\in SE(3)$, then $g_1g_2\in SE(3)$.
\item The  identity  $ I_4 \in  SE(3)$.
\item If $g\in SE(3)$, then the inverse of $g$ is determined by the 
matrix inversion:
\[
g^{-1}= 
 \left[
\begin{array}{ccc}
 R^T  & -R^T p  \\
    0 & 1 
\end{array}
\right] \in SE(3),
\]
where $g^{-1} = (-R^Tp, R^T)$.
\item The composition rule for rigid body transformations is associative.
\end{itemize}

\subsubsection{Lie Algebra Properties of $\SE$}
\paragraph*{Hat- and Vee-maps in $SE(3)$.}
 The Lie algebra of $SO(3)$, denoted by  $\fso$, defines skew-symmetric matrices.
 The hat-map for $\fso$ is defined by 
$\widehat{(\cdot)}\, (\text{or} \, (\cdot )^{\wedge} ): \Real^3 \rightarrow \fso,$ which maps an angular velocity vector $\omega \in \Real^3$ to its skew-symmetric cross product matrix, i.e.,  
\[\hat \omega=- \hat \omega^T
=
  \left[
\begin{array}{ccc}
0  & -\omega_3 & \omega_2   \\
 \omega_3 & 0 & -\omega_1 \\
  -\omega_2  & \omega_1 & 0
\end{array}
\right]  \in \Real^{3 \times 3}
\] 


for $\omega \in \Real^3.$
 Hence, for $v \in \Real^3$, $\hat \omega v = \omega \times v$ with {\color{red} (SML: with -> , where)} $\times$ represents the cross product of vectors.
The inverse of the hat map is the   vee-map    
 $
 (\cdot )^\vee: \fso : \rightarrow \Real^3.
 $
Similarly, the hat-map for $\fse$ is defined as  $\widehat{(\cdot)}: \Real^6 \rightarrow \fse.$
The inverse of the hat map is the   vee-map    
 $
 (\cdot )^\vee: \fse : \rightarrow \Real^6.
 $
Thus, we have
\[
 \hat \xi = 
\begin{bmatrix}
     \hat \omega  & v  \\
    0 & 0 
\end{bmatrix} \in \fse \subset \Real^{4 \times 4}, \;\;
\forall  \xi = 
\begin{bmatrix}
  v  \\
    \omega
\end{bmatrix} \in \Real^6,
\]
where $v, \omega \in \Real^3, \hat \omega \in \fso.$

\paragraph*{Twists}
An element of $\fse$ is referred to as a twist or a (infinitesimal) generator
of the Euclidean group.  Recall that the adjoint action  of $g \in \SE$ on $\hat{\xi} \in \fse$, $\Ad_g: SE(3) \times \fse \rightarrow \fse$, is then defined by
\[
Ad_g \hat{\xi} = g \hat{\xi} g^{-1}.
\]
Let $\hat{\xi}' = g \hat{\xi} g^{-1}$. $\hat{\xi}'$ is $\xi$ applied by a constant rigid motion $g$ with $\dot{g}=0$ {\color{red} (SML: with -> , where)}. With the previous notion of $\Ad_g:\SE \times \mathbb{R}^6 \to \mathbb{R}^6$ as an linear operator, we can write:
\[
    \hat{\xi}' = g\hat{\xi}g^{-1}, \quad \xi' = \Ad_g \xi.
\]
We can interpret $\hat{\xi}$ as a twist with the coordinate $\xi \in \mathbb{R}^6$, and $\hat{\xi}'$ a twist with the coordinate $\Ad_g \xi \in \mathbb{R}^6$, $\forall g \in \SE$.

\paragraph*{Spatial and Body Velocities (twists in $SE(3)$)} b
{\color{lightgray}
Consider a pure rotation. 
Let $R_{ab}(t) \in SO(3)$ be a curve representing a trajectory of an object frame B  relative to a fixed (inertial) coordinate frame A.
Any point $q$ attached to the rigid body follows a trajectory in spatial coordinates:
\[
q_a(t) =R_{ab}(t) q_b.
\]
The velocity of $q$ in spatial coordinates is
\[
\begin{split}
v_{q_a}(t)  = \frac{d}{dt} q_a(t)&=\dot R_{ab}(t) q_b\\
&=\underbrace{\dot R_{ab}(t) R_{ab}^{-1}(t)}_{=:\widehat \omega_{ab}^s (t)} R_{ab}(t) q_b\\
&=\widehat \omega_{ab}^s(t) R_{ab} (t) q_b \\
&=\omega_{ab}^s (t) \times  R_{ab} (t)q_b\\
&=\omega_{ab}^s (t) \times  q_a (t)\\
\end{split}
\]
where $\omega_{ab}^s$ is the instantaneous spatial angular velocity, i.e.,
\[
\widehat \omega_{ab}^s:=\dot R_{ab} R_{ab}^{-1}.
\]

We also define the angular velocity as viewed from
the instantaneous body  coordinate frame B as  the instantaneous body angular velocity:
\[
\widehat \omega_{ab}^b:= R_{ab}^{-1}\dot R_{ab}.
\]

Relationships between two angular velocities are
\[
\widehat \omega_{ab}^b=R^{-1}_{ab} \widehat \omega_{ab}^s R_{ab},   \quad \text{or} \quad \omega_{ab}^b=R_{ab}^{-1} \omega_{ab}^s.
\]
From this, we can describe the velocity of $q$ relative to body frame B:
\[
v_{q_b} (t):= R_{ab}^T(t) v_{q_a}(t)= \omega_{ab}^b(t) \times q_b.
\] 
}

Consider a curve parameterized by time,  representing a trajectory of
a rigid body such that
\[
g_{ab}(t)= \left[
\begin{array}{cc}
     R_{ab}(t) & p_{ab}(t)  \\
      0 &   1
\end{array}
\right]
\]
{ \color{lightgray}
The coordinates of $q$ attached to the body frame B in spatial coordinates are given by
\[
q_a(t)= g_{ab} (t) q_b.
\]
The velocity of $q$ in spatial coordinates is
\[
\begin{split}
v_{q_a}=\frac{d}{dt} q_a &=\dot g_{ab} q_b= \dot g_{ab} g_{ab}^{-1} q_a\\
&=\widehat V_{ab}^s q_a= \omega_{ab}^s \times q_a + v_{ab}^s.
\end{split}
\]
}
Now, we define the spatial velocity $\widehat{V}_{ab}^s$ of a rigid motion $g_{ab} \in SE(3)$
\[
\widehat{V}_{ab}^s:= \dot g_{ab} g_{ab}^{-1}=
\left[
\begin{array}{cc}
\dot R_{ab}   R_{ab}^T &  -\dot R_{ab}   R_{ab}^T p_{ab} +  \dot  p_{ab} \\
  0 & 0
  \end{array}
\right],
\] 
\[
{V}_{ab}^s=\left[
\begin{array}{c}
 v_{ab}^s \\
   \omega_{ab}^s  
\end{array}
\right]
=
\left[
\begin{array}{c}
  -\dot R_{ab}   R_{ab}^T p_{ab} +  \dot  p_{ab} \\
      ( \dot R_{ab} R_{ab}^T)^\vee
\end{array}
\right]
\] 
We also define the body (or generalized) velocity of a rigid motion $g_{ab} \in SE(3)$
\[
\begin{split}
\widehat{V}_{ab}^b:= g_{ab}^{-1} \dot g_{ab} &=
\left[
\begin{array}{cc}
 R_{ab}^T  \dot R_{ab} &   R_{ab}^T    \dot p_{ab}  \\
  0 & 0
  \end{array}
\right]\\
&=
\left[
\begin{array}{cc}
\widehat \omega_{ab} &   v_{ab}  \\
  0 & 0
  \end{array}
\right],
\end{split}
\] 
where $\widehat \omega_{ab}^b =R_{ab}^T  \dot R_{ab} $ and $v_{ab}^b=R_{ab}^T    \dot p_{ab}$.
\[
{V}_{ab}^b=\left[
\begin{array}{c}
 v_{ab}^b \\
   \omega_{ab}^b  
\end{array}
\right]
=
\left[
\begin{array}{c}
  R_{ab}^T    \dot  p_{ab} \\
      (  R_{ab}^T \dot R_{ab})^\vee
\end{array}
\right]
\] 

Body velocity can be transformed into the spatial velocity by the adjoint transformation $Ad_g$, i.e.,
\[
{V}_{ab}^s=
\left[
\begin{array}{c}
 v_{ab}^s\\
   \omega_{ab}^s  
\end{array}
\right]
=
\underbrace{
\left[
\begin{array}{cc}
 R_{ab} & \widehat{p}_{ab} R_{ab}\\
    0 & R_{ab}
    \end{array}
\right]}_{=\Ad_{g_{ab}}}
\left [ V_{ab}^b=
\left[
\begin{array}{c}
 v_{ab}^b \\
   \omega_{ab}^b  
\end{array}
\right]
\right ] \] 
\[
i.e., \,
 {V}_{ab}^s=\Ad_{g_{ab}}{V}_{ab}^b. 
\]

Given  $g \in SE(3)$, the (large) adjoint transformation $\Ad_g : \Real^6 \rightarrow \Real^6$ maps one coordinate to another {\color{red} SML: Is the equation the end of the sentence? AK: feels a little redudant to have the same equation basically from the previous one }
\[
\Ad_g = \begin{bmatrix}
R & \widehat{p} R\\
    0 & R
\end{bmatrix}   ,
\]
$\Ad_g$ is invertible, and its inverse is given by
\[
\Ad_g^{-1}=\left[
\begin{array}{cc}
R^T & -R^T\widehat{p} \\
    0 & R^T
    \end{array}
\right]
=\Ad_{g^{-1}}.
\]

The body and spatial velocities are related by the (large) adjoint transformation.
\[
V^s=\Ad_g V^b, \quad  V^b=\Ad_{g}^{-1} V^s=\Ad_{g^{-1}} V^s.
\]

As mentioned previously, the large adjoint map used herein is a linear operator version. 

{ \color{lightgray}
Consider the motion of three frames A, B, and C. The configuration of frame C with respect to A is given by
\[
g_{ac}=g_{ab}g_{bc}.
\]
We then represent $\widehat V_{ac}^s$ using $\Ad_{g_{ab}}$ via the chain rule.
\[
\begin{split}
\widehat V_{ac}^s&=\dot g_{ac} g_{ac}^{-1}\\
&=(\dot g_{ab} g_{bc} + g_{ab} \dot g_{bc}) (g_{bc}^{-1}g_{ab}^{-1})\\
&=\dot g_{ab}g_{ab}^{-1} + g_{ab} (\dot g_{bc} g_{bc}^{-1}) g_{ab}^{-1}\\
&=\widehat V_{ab}^s+ g_{ab} \widehat V_{bc}^s g_{ab}^{-1}\\
\end{split}
\]
In twist coordinates, we have
\[
 V_{ac}^s=V_{ab}^s+ \Ad_{g_{ab}}   V_{bc}^s.
\]
Similarly $\widehat V_{ac}^b$  can be shown that
\[
  V_{ac}^b=\Ad_{g_{bc}^{-1}}  V_{ab}^b+ V_{bc}^b.
\]

 When frames B and C  are attached to  a rigid body and A  is the inertial frame, as shown in Fig.~\ref{fig:Wrench}, we have $V_{bc}^b=0$ such that
$V_{ac}^b=\Ad_{g_{bc}^{-1}}  V_{ab}^b$, which implies 
\[
V_{ab}^b= \Ad_{g_{bc}}V_{ac}^b=\Ad_{g_{cb}^{-1}}V_{ac}^b,
\]
 where $g_{bc} \in SE(3): \{ B\} \rightarrow \{C\},$ i.e.,  the configuration of frame C relative to frame B.    
This adjoint action of $SE(3)$ on $\fse$ clearly shows  the effect of a change
of body frame on the body velocity.}

\begin{figure}[!t]
\centering
\resizebox{\columnwidth}{!}{
\input{Figures/wrench}}
\caption{Transformation of wrench $F$ between coordinate frames.}
\label{fig:Wrench}
\end{figure}

{ \color{lightgray}
\paragraph*{Translated twists}
For a twist $\xi$, that is the motion of a screw, and we want to move it by applying a constant rigid motion $g$ with  $\dot g=0$. We then have new $\xi'$
\[
\xi'=\Ad_g \xi, \quad \hat \xi'=g \hat \xi g^{-1}.\]
We can interpret $\xi'$ such that 
if $\widehat \xi \in \fse$ is a twist with the coordinate $\xi \in \Real^6$, $\forall g \in SE(3)$, 
$g \widehat\xi g^{-1}$ is a twist with the coordinate $\Ad_g \xi \in \Real^6$.
}

\paragraph*{Dual of the Lie algebra} 
The co-adjoint    action of $g$ (or sometimes used with $g^{-1}$) on  $\xi^* \in \fse^*$ which is the dual of $\xi$ is denoted as $\Ad_{g^{-1}}^* : \SE \times  \fse^* \rightarrow \fse^*$. {\color{red} SML: As mentioned before, should dual be defined? Also this sentence is pretty awkwardly phrased} Similar to the large adjoint operator of twist, we will not distinguish the linear operator version of $\Ad_{g}$, and is defined by a matrix in $\Real^{6 \times 6}$ such as
\[
Ad_{g^{-1}}^* =Ad_{g^{-1}}^T.
\]

In general, the co-adjoint action of $g$ on $\fg^*$, {\color{red} AK: remove this phrase; little redundant}the dual of the Lie algebra $\fg$ of $g$, can be defined.
Let $Ad_g^*: G \times \fg^* \rightarrow \fg^*$ be the dual of $Ad_g$ defined by
\[
\langle Ad_{g^{-1}}^* (\alpha), \xi \rangle= \langle \alpha, Ad_{g} (\xi) \rangle 
\] 
for $\alpha \in \fg^*$ and $\xi \in \fg$. The co-adjoint action of $g$ on $\fg^*$ is then given by the map $\Phi^*: G \times \fg^* \rightarrow \fg^* $
\[
\Phi^* (g, \alpha) =Ad_{g^{-1}}^* \alpha.
\]


\paragraph*{Wrenches}
A pair of a force and a moment acting on a rigid body 
is referred to as a wrench, i.e., 
a generalized force.
\[
F= 
\left[
\begin{array}{c}
  f  \\
  \tau    
\end{array}
\right] \in \mathbb{R}^6,
\]
 where $f \in \Real^3$ and $\tau \in \Real^3$ are linear and rotational force components, respectively.

Consider the motion of a rigid body by $g_{ab}(t)$ with respect to an inertial frame A and a body frame B.
Let $V_{ab}^b \in \Real^6$ and $F_b\in \Real^6$ be the instantaneous body velocity and an applied wrench.
The infinitesimal work is obtained by the inner product of $V_{ab}^b \in \Real^6$ and $F_b$.
\[
\delta W=   \langle V_{ab}^b,   F_b \rangle=({v_{ab}^b}^T f+ {\omega_{ab}^b} ^T \tau).
\]
The net work generated by applying $F_b$ through  a twist $V_{ab}^b$ during the  interval $[t_1, \, t_2]$ is given by
\[
W=\int_{t_1}^{t_2}  \langle V_{ab}^b, F_b  \rangle dt.
\]

Let $g_{bc} =(p_{bc},R_{bc})$ be the configuration of frame C relative to B.
To find an equivalent wrench $F_c$ applied at C, we equate two instantaneous work quantities by $F_c$ and $F_b$.
\[
\begin{split}
  \langle V_{ac}, F_c \rangle&=\langle  V_{ab}, F_b \rangle\\
  &= (Ad_{g_{bc}}V_{ac})^T F_b = \langle V_{ac} , \Ad_{g_{bc}}^T F_b \rangle,
\end{split}
\]
where we use the relationship between body velocities, i.e., $V_{ab}=\Ad_{g_{bc}} V_{ac}.$

The coordinate transformation between wrenches $F_c$ and $F_b$  (see Fig.~\ref{fig:Wrench}) can be represented by different ways.
\[
\begin{split}
F_c &= \Ad_{g_{bc}}^T F_b=\Ad_{g_{ba}g_{ac}}^T F_b\\
&=(\Ad_{g_{ba}}\Ad_{g_{ac}} )^T F_b=\Ad_{g_{ac}}^T\Ad_{g_{ba}}^T F_b\\
    &=\Ad_{g_{cb}^{-1}}^T F_b=\Ad_{(g_{ca}g_{ab})^{-1}}^T F_b =\Ad_{ g_{ab}^{-1} g_{ca}^{-1} }^T F_b\\
    &= (\Ad_{ g_{ab}^{-1}} \Ad_{g_{ca}^{-1} } )^T F_b=  \Ad_{g_{ca}^{-1} }^T  \Ad_{ g_{ab}^{-1}}^T F_b,
\end{split}
\]
where the adjoint composition  rule in \eqref{eq:Adchain} was used.

\paragraph*{Exponential Map from $\fse$ to $SE(3)$.}
Given $\hat \xi \in \fse$ and $\theta \in \Real$, the exponential of $\hat \xi \theta$ is in $SE(3)$, i.e., 
\[
\begin{split}
    \exp{(\hat \xi \theta)} &= \exp{   \left (\left[
\begin{array}{ccc}
 \hat \omega  & v  \\
    0 & 0 
\end{array}
\right]   \theta  \right ) }\in SE(3)\\
&=I+ {    \left[
\begin{array}{ccc}
 \hat \omega  & v  \\
    0 & 0 
\end{array}
\right]   \theta    } + { \frac{1}{2!}   \left[
\begin{array}{ccc}
 \hat \omega^2  & \hat \omega v  \\
    0 & 0 
\end{array}
\right]   \theta^2    } \\ &+ { \frac{1}{3!}   \left[
\begin{array}{ccc}
 \hat \omega^3  & \hat \omega^2 v  \\
    0 & 0 
\end{array}
\right]   \theta^3    }+ \cdots
\end{split}
\] 
This shows that the exponential map from $\fse$ to $SE(3)$ is the matrix exponential on a linear combination of the
generators.
We interpret the transformation $g=\exp(\hat \xi \theta)$ 
as a mapping  from an initial coordinate, $p(0)\in \Real^3$, to its
coordinate $p(\theta)$ after the rigid motion is applied such that
\[
p(\theta)= \exp{(\hat \xi \theta)} p(0).
\]
Let $g_{ab}(0)$ represent the initial configuration of a rigid body relative to a frame A, then the final configuration,
 with respect to A, is given by
\[
g_{ab}(\theta)= \exp{(\hat \xi \theta)} g_{ab}(0).
\]
The exponential map for a twist gives the relative motion of a rigid
body.

\subsubsection{Forward Kinematics}
The forward kinematics of the manipulator is given by the product of the exponentials formula, i.e., a map $g: Q \rightarrow SE(3):$
\[
g(\F)=e^{(\hat \xi_1 \theta_1)}e^{(\hat \xi_2 \theta_2)} \cdots e^{(\hat \xi_n \theta_n)} g(0),
\]
where $e^{(\cdot)}=\exp(\cdot)$ and $g(\theta)$ is the homogeneous representation of the end-effector in the spatial frame, $\xi_i \in \Real^6$ is a twist represented in the spatial frame and $\theta_i \in \Real$ a joint angle of the $i$-th joint, for $i=1, 2, \cdots n$, starting from the base. See more details in \cite{murray1994mathematical}.

% {\color{red}SML: where $e^{(\cdot)}=\exp(\cdot)$ and $g(\theta)$ is the homogeneous representation of the end-effector in the spatial frame. $\xi_i \in \Real^6$ is a twist represented in the spatial frame, and $\theta_i \in \Real$ is the joint angle of the $i$-th joint, starting from the base, for $i=1, 2, \cdots n$. See more details in \cite{murray1994mathematical}.}

==> Old_2024_1130/Section3_EquivariantDeepLearning.tex <==
% {\color{red} AK:Equivariant deep learning have been primarily employed to process visual inputs in form of 2D images or 3D pointclouds in robotic applications.}
Equivariant deep learning has been primarily employed to process visual inputs in the form of 2D images or 3D point clouds in robotic applications.
% Equivariant deep learning has been employed mainly to deal with vision inputs, e.g., 2D image and 3D point cloud, for robotics applications. 
In this chapter, we will introduce and review the concept of equivariance and equivariant neural network architectures to handle such vision inputs. We start with introducing the equivariant structure for the convolutional neural networks (CNN) to deal with image domain data, followed by the equivariant graph neural network (GNN) for point cloud data.
% \JS{(Brief outline) Equivariant deep learning to deal with vision inputs for robotics applications - for 2D image: GCNN is used, and for 3D pointcloud: Group equivariant graph neural networks. We will mention GCNN and Graph neural networks, but you know graph neural networks are also graph convolutions}
\subsection{Regular Group CNNs}
\subsubsection{Standard CNNs: Cross-correlation Kernels and Weight-sharing}
Before introducing the equivariant group CNNs (G-CNNs),  let us first consider the standard CNNs, which use cross-correlation (or convolution) kernels to extract features from images. 
\paragraph*{Cross-correlation Kernels} The cross-correlation (or convolution) operation between an input image $f(x)$ and a correlation kernel $\W(x)$ (or a convolution kernel $\hat \W(x)$, respectively) at   $x$ can be written as:
\begin{equation}\label{eq:conv}
\begin{split}
y(x) &= (\W \star f )(x) = \int_{\mathbb{R}^n} f( \tilde  x)\W(\tilde x-x)d \tilde  x\\
&= (\hat \W \ast f) (x) =  \int_{\mathbb{R}^n} f( \tilde  x) \hat \W(x- \tilde x)d \tilde  x,
\end{split} 
\end{equation}
where $\W(x)=\hat \W(-x)$, $\star$ denotes cross-correlation operator and $\ast$ denotes convolution operator.
As can be seen in Fig.~\ref{fig:Alex}, many redundant rotated edge filters in different angles are generated in the standard CNNs (by training under image augmentation via rotation). 
% {\color{red}AK: Remove following sentence}These are convolutional filters in the first layer of AlexNet \cite{krizhevsky2012imagenet} trained on ImageNet \cite{deng2009imagenet}.
Interpreting standard CNNs as cross-correlation kernels allows us a straightforward extension to the group equivariant CNNs.

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/Alexnet_1st_layer.png}
    \caption{Convolutional filters in the first layer of AlexNet\cite{krizhevsky2012imagenet} trained on ImageNet \cite{deng2009imagenet}. Many rotated edge filters with similar shapes can be spotted. This standard CNN is not efficient without weight sharing in the rotational angle. This figure is generated using pre-trained AlexNet provided by PyTorch \cite{PytorchAlexNet}.{\color{red} [Jun] Adding red boxes on the rotation-invariant filters, just as we did in NRF proposal, might be easy to understand}}
    \label{fig:Alex}
\end{figure}

\paragraph*{Left-regular Representation} 
Before we further investigate the cross-correlation kernels 
% {\color{red} [JC] is this typo? -> kernels} 
undergoing group action, one notable concept must be reviewed: left-regular representation. A left-regular representation is a useful way to let a group $\G$ act on functions. 
In this case, a function is transformed by transforming the domain $\mathcal{X}$ by the action of the group $\G$.
The left-regular representation of $g \in \G$ acting on $f(x)$ with $x \in \mathcal{X}$ is defined by
\begin{equation}\label{eq:left}
L_g(f)(x) = g \circ  f(x)= f(g^{-1} \circ x)
\end{equation}
where $\circ$ denotes the action of the group $\G$ on the appropriate domain or codomain. In the case of $\mathcal{X} = \mathbb{R}^2$, i.e., an image plane, $f \in \mathbb{L}^2(\mathbb{R}^2)$ 
% {\color{red}[JC] I think more common way to write image plane is $f: \mathbb{R}^2\rightarrow \mathbb{R}^c$, where $c$ is the channel dimension} 
is a square-integrable function.
We also notice that
\begin{equation}\label{eq:g1g2}
\begin{split}
L_{g_1g_2}(f)(x) &= g_1g_2 \circ  f(x)=L_{g_1}L_{g_2}(f)(x)\\
&= f((g_1g_2)^{-1} \circ x)=f(g_2^{-1}g_1^{-1} \circ x).
\end{split}
\end{equation}

\paragraph*{Weight-sharing}\label{weightsharing}
%  Recall 
%  the left-regular representation of $g \in G$ acting on $f(x)$ is defined by
% \begin{equation}\label{eq:left2}
%     L_g(f)(x) = g \circ  f(x)= f(g^{-1} \circ x)
% \end{equation}
% where $\circ$ denotes the
% action of the group $\G$ on the domain of $X$.
%  $f\in \mathbb{L}^2(\mathbb{R}^2)$ is a square-integrable function and $g^{-1}$ is the inverse of the group element $g$.
%  We also notice that
% \begin{equation}\label{eq:g1g2}
% \begin{split}
% L_{g_1g_2}(f)(x) &= g_1g_2 \circ  f(x)=L_{g_1}L_{g_2}(f)(x)\\
% &= f((g_1g_2)^{-1} \circ x)=f(g_2^{-1}g_1^{-1} \circ x).
% \end{split}
% \end{equation}

Once we use the left-regular representation in the translation group as in \eqref{eq:left} as 
\[ \T_x(\W) (\tilde x):= L_x(\W)(\tilde x) = \W(\tilde x-x),\] 
\eqref{eq:conv} can then be represented as an inner product. 
\[
\begin{split}
y(x) = (\W \star f )(x) &= \int_{\mathbb{R}^n} f(\tilde x)\W(\tilde x-x)d \tilde x\\
&=\langle \T_x (\W), f\rangle_{\mathbb{L}_2 (\mathbb{R}^n)}.
\end{split}
\]
From the inner product form above, it is clear that convolution can be considered template matching for feature extraction over different locations in $x$. This leads to efficient learning via sharing kernel weights across various locations in the data. 
Standard  CNNs are effective for data that exhibits translation symmetry. However, they may not efficiently learn features such as an edge shape with different angles without weight sharing in rotational angles. To address this limitation, data augmentation techniques such as rotating images with different angles are used to generate a larger number of kernels (or filters) with various orientations, as in  Fig.~\ref{fig:Alex}. 
The left-regular representation is an important tool for developing equivariant neural networks. For example, substituting the original CNN kernels with ones that transform according to left-regular group representation produces the group-equivariant CNNs, which will be discussed in the following sections.
% The left-regular representation and its application on CNNs is an important tool in the study of group representations and equivariant neural networks, as it allows us to generalize the convolution/cross-correlation operation of CNNs to equivariant group CNNs by replacing the usual convolution kernels with group-equivariant kernels that transform according to the left-regular representation of the group, which will be discussed in the followings.
% {\color{red}AK:Rephrase sentence as "The left-regular representation is an important tool for developing equivariant neural networks. For example, by substituting the original CNN kernels with ones that transform according to left-regular group representation, producing the group-equivariant CNNs discussed in the following sections}
%  One can also obtain the same result by using a homogeneous matrix representation as follows:
% \begin{equation*}
%     \begin{split}
%         &g = \begin{bmatrix}
%             R_\theta & x \\
%             0 & 1
%         \end{bmatrix}, \quad g^{-1} = \begin{bmatrix}
%             R^{-1}_\theta & -R^{-1}_\theta x \\
%             0 & 1
%         \end{bmatrix}\\
%         &g^{-1} \begin{bmatrix}
%             \tilde{x} \\ 1
%         \end{bmatrix}  = \begin{bmatrix}
%             -R^{-1}_\theta (x - \tilde{x}) \\ 1 
%         \end{bmatrix} = \begin{bmatrix}
%             R^{-1}_\theta (\tilde{x} - x) \\ 1
%         \end{bmatrix} \\
%         &\implies g^{-1} \circ \tilde{x} = R^{-1}_\theta (\tilde{x} - x).
%     \end{split} 
% \end{equation*}



\subsubsection{$SE(2)$-Group CNNs}
{\color{red} [Jun] As far as I understand, GCNN does not inherently leverage full SE(2)-equivariance; instead, they utilize finite subgroups of SO(2), such as cyclic groups to leverage $\mathbb{R}^2\rtimes C_N$. Using "SE(2)" in this context might lead to confusion. It could be more precise to refer to them simply as "Equivariant Group CNNs", "Lifting Convolution", and "Group convolution". Alternatively, if the purpose of this paragraph is to introduce the concept of lifting and group convolution, we might consider removing the term "G-CNN" altogether, since they are applied to both GCNNs and steerable CNNs.}

{\color{red} [Jun] I agree with Soomi, I think we should add a simple introduction for this section. Here is the suggested paragraph: To incorporate weight sharing under 2D rotations, G-CNNs \cite{cohen2016group} introduced the concept of convolution over the "roto-translation group $\mathbb{G}$". This approach involves two key steps: 1) Lifting convolution and 2) Group convolution. Lifting convolution maps the input image from the $\mathbb{R}^2$ domain to the group domain $\mathbb{G}$. Then, group convolution performs the convolution directly on the group domain. A similar framework is employed in Steerable CNNs \cite{cohen2016steerable}, utilizing representation theory and harmonic analysis. The following paragraphs provide a more detailed explanation of these processes.}

\paragraph*{$SE(2)$ Lifting Correlations} 
{\color{red}AK:Maybe add this sentence at the beginning, "For $SE(2)$, full equivariance can be accomplished by  }
We now consider a transformation operator in $SE(2)$, $L_g$ with the roto-translation parameter $g=(x,\theta)$, where $x$ and $\theta$ are the translation vector and the rotation angle, respectively. Due to \eqref{eq:g1g2} with $g_1=(x)$ and $g_2=(\theta)$, $L_g=L_{(x,\theta)}$ can be obtained as follows. {\color{red} SML: I think a short intuitive explanation and purpose of lifting in the beginning would facilitate understanding. }
\[
\begin{split}
[ L_{g_1g_2} \W ](\tilde x)&=[ L_{(x,\theta)} \W ](\tilde x) =[L_x L_\theta \W ](\tilde x)\\ &=\W (g_2^{-1} g_1^{-1} \tilde x)) = \W (R^{-1}_\theta (\tilde x - x)).
\end{split}
\]
Then, the roto-translation lifting correlation from $\Real^2$ to the space of $SE(2)$ is defined such as 
\begin{equation}\label{eq:LiftingCov}
\begin{split}
y(g)&=y(x, \theta)=(\W \star_{SE(2)}  f )  (x, \theta)\\
&=  \langle L_{(x, \theta)}\W, f \rangle_{\mathbb{L}_2 (\Real^2)} =\langle L_{x} L_\theta \W, f \rangle_{\mathbb{L}_2 (\Real^2)} \\
&=\int_{\Real^2} \W (R^{-1}_{\theta} (\tilde x-x)) f(\tilde x) d \tilde x.
\end{split}
\end{equation}

\paragraph*{ $SE(2)$ Group Convolutions} $SE(2)$ group convolution are roto-translation equivariant. 
Following the initial roto-translation lifting correlation on a 2D image, a feature map is generated on   $SE(2)$. The feature layers resulting from the lifting operation are then parameterized by patterns of position-orientation localized features, which can be transformed by the action of the group element $L_{(x, \theta)}$. This transformation enables the use of $SE(2)$-equivariant convolutional neural networks (G-CNNs) that operate on $SE(2)$ kernels, thereby allowing for the efficient extraction of features that are invariant to both translation and rotation.
After the $SE(2)$ lifting convolution, the $SE(2)$  group convolution can be performed in the lifted higher dimensional feature maps of $SE(2)$.
\begin{equation}\label{eq:SEfilter}
    \begin{split}
    y(g) &= 
     \int_{SE(2)} \W (g^{-1} \circ \tilde g) f(\tilde g) d \tilde g\\
    &= \int_{\Real^2} \int_{S^1} \W(R^{-1}_\theta (\tilde x- x),  \tilde \theta -\theta) f(\tilde x, \tilde \theta) d \tilde x d \tilde \theta.
    \end{split}
\end{equation}

\subsubsection{Equivariant maps} Suppose $\G$ is a Lie group, and $M$ and
$N$ are both smooth manifolds with smooth left or right $\G$-actions. A map (e.g., a neural network)
$\Phi : M \rightarrow N$ is said to be equivariant with respect to   $\G$-actions   if for each
$g \in \G$, 
\[
\Phi(g \cdot p)=g \cdot \Phi(p),\quad \text{for left actions},\]
and 
\[
\Phi(p \cdot g)= \Phi(p) \cdot g, \quad  \text{for right actions \cite{leesmooth}.} \] 
Equivariance implies that no information is lost by input transformations, i.e., 
the output will be shifted to different locations in the output domain. It also allows for weight sharing over the transformations in the
group (e.g., $SE(2)$ or $\SE$ including rotation), which reduces a significant number of learnable parameters as compared to the standard CNNs (e.g., see Fig.~\ref{fig:Alex}). 
For example, $SE(2)$ equivariant CNNs (i.e., G-CNNs) for 2D images can be built using lifting and group convolutions from \eqref{eq:LiftingCov} and \eqref{eq:SEfilter}, respectively. Although G-CNNs are more efficient due to weight sharing compared to the standard CNNs,  the  filtered  outputs in discretized $\theta$
need to be computed and stored for the higher dimensional feature space in $SE(2)$. Steerable filters can be used to mitigate these computational and memory burdens.

\subsection{Steerable Group CNNs}
{\color{red} [Jun] The convolutions in G-CNNs operate over the group elements, which increases computational cost and can lead to inefficiencies.} \JS{This is for the theoretical efficiency, but we can add some limitations of group equivariant neural networks in the final session as a caveat.} 
More efficient equivariant convolutional neural networks (i.e., steerable G-CNNs) can be constructed using 
steerable feature vectors, which will remove the discretization in rotation as in G-CNNs with the $SE(2)$ regular group convolutions. {\color{red} SML: Perhaps address limitations of discretization? }
Steerability of a vector (say $h$) implies that for a transformation group $g$, the vector $h$ transforms via matrix-vector multiplication $D(g)h$. 
Steerable methods avoid discretization of $SO(n)$ in regular G-CNNs by exploiting irreducible representations, which allows the use of Fourier theory on Lie groups. Steerable methods build on the following concepts: steerable feature vectors, spherical harmonics, Wigner-D matrices, and the Clebsch-Gordan tensor product. 
In particular, as the spherical harmonics (SH) play a crucial role in the formulation of steerable group convolutional neural networks, we will first introduce the details of the SH. 
{\color{red} SML: I think I'm getting lost in all the maths and explanations that it's hard to grasp the high level understanding of steerability. I think fully understanding it without digging into steerability is not so feasible, so instead, a clear high level explanation and purpose here would be likely to help the reader navigate through the rest of the paper. }
% In particular, we will first cover the formulation of the SH.

\subsubsection{Spherical Harmonics (SH)}
Spherical harmonics (SH) provide a theoretical foundation for the steerable functions as they serve as a basis function for $\SO$ transformation. SH is a class of functions on the sphere $S^2$ and can be used as a Fourier basis on the sphere. As will be mentioned later, they are steered by Wigner-D matrices and allow the interpretation of steerable vectors as functions on $S^2$. Moreover, spherical harmonics allow the embedding of 3D displacement vectors into arbitrarily large steerable vectors, i.e., allows lifting. 
Although the theory of SH is well established among physics/chemistry fields, those with engineering backgrounds might be unfamiliar with this concept. Therefore, we present the motivations and formulation of SH in the appendix for readers who want to investigate further. 

% Combining these results altogether, for a given value of $l$, there are $2l+1$ independent solutions of the form, $Y(\theta,\phi) = \Theta(\theta)\Phi(\phi)$, one for each integer $m$ with $-l \leq m \leq l$. We denote these independent solutions associated with the integer $m$ and $l$ as $Y_m^l$, $Y_m^l:S^2 \to \mathbb{C}$, and they are the product of complex exponentials and associated Legendre polynomials as follows:
In a nutshell, spherical harmonic function $Y_m^l : S^2 \to \mathbb{C}$ is given as follows:
\begin{equation} \label{eq:sol_Y}
    Y_m^l(\theta,\phi) = N e^{im\phi} P_m^l(\cos{\theta}),
\end{equation}
where $\theta$ and $\phi$ are azimuthal and longitudinal angles, respectively, and $P_m^l$ are associated Legendre polynomials. 
$l\in\{0,1,2,\cdots\}$ is called the \textit{degree} and $m\in\{-l,\cdots,l\}$ is called the \textit{order} of the spherical harmonic function. 
Although we have built the SH in the complex domain, general applications of SH are built in the real domain, and the interchange between the two domains is possible, e.g., \cite{lee2018real}.
Here, the \textit{(real) spherical harmonics} $Y_m^{l}(\theta, \phi)$ are orthonormal functions that form the complete basis of the Hilbert space on the sphere $S^2$. 

Spherical harmonic functions span the sub-representation of $V_l$ vector spaces:
\begin{equation}
    \begin{split}
        V_0 &= \text{Span}\{Y_0^0(n)\}\\
        V_1 &= \text{Span}\{Y_{-1}^{1}(n), Y_0^1(n), Y_1^{1}(n)\} \\
        &\vdots \\
        V_k &= \text{Span}\{Y_{-k}^{k}(n), Y^k_{-k+1}(n), \cdots , Y^k_0(n), \cdots, Y^k_k(n)\},
    \end{split}
\end{equation}
where $n$ is a unit vector on a unit sphere and is one-to-one correspondence to $(\theta,\phi)$ representation. We call $V_l$ vector space as \textit{type-$l$} (or \textit{spin-$l$}) vector field and an arbitrary vector $h \in V_l$ as type-$l$ vector. Type-$l$ vectors are identical to themselves when they are rotated by $\theta = 2\pi/l$. Type-$0$ vectors, or \textit{scalars} are invariant to rotations ($\theta=\infty$). Type-$1$ vectors are the familiar 3-dimensional space vectors ($\theta=2\pi$). 
A critical property of the SH is that it is transformed by a 3-dim rotation matrix $R \in \SO$. Consider $2l+1$-dimensional vector field, i.e., type-$l$ vector field:
\begin{equation}
    \mathbf{Y}^l = \left(Y_{-l}^{l}, Y_{-l+1}^l, \cdots, Y^l_{l-1}, Y^l_l\right)^T.
\end{equation}
Then, $\mathbf{Y}^l$ is transformed by $R$ s.t.
\begin{equation}
    \mathbf{Y}^l\left(R \frac{x}{\|x\|}\right) = D^l(R) \mathbf{Y}^l\left(\frac{x}{\|x\|}\right).
\end{equation}
where $D^l(R)$ is a left-regular representation of $R\in SO(3)$ with order $l$. $D^l(R)$ is a Wigner-D matrix.

\subsubsection{Wigner-D Matrices as Orthogonal Basis of SO(3)}
 $D^{l}_{mn} : SO(3) \rightarrow \Real$ form complete orthogonal basis for functions on $SO(3)$.
Therefore, any function on $SO(3)$ can be represented in terms of an $SO(3)$ Fourier series. 
\[ 
\begin{split}
f(R) &=\sum_{l}^\infty  \sum_{m=-l}^{l} \sum_{n=-l}^{n=l} \hat f_{mn}^{(l)}D_{mn}^{l} (R) 
= \sum_l^\infty \tr \left( \hat f^{(l)} (D^{l} (R))^T\right)\\
&=\sum_l^\infty \tr \left ( \hat f^{(l)} D^{l} (R^{-1})\right )
\end{split}
\]
where $R \in \SO$, and the equation above can be considered as the inverse Fourier transform. Note that $D^l(R^{-1}) = (D^l(R))^T$ is utilized.
The Fourier transform of a function $f(R)$ on $SO(3)$ can be then obtained by the inner product using the basis as follows:
\[
\hat f^{(l)}_{mn}=\langle D_{mn}^l(R), f(R) \rangle.
\]

\subsubsection{Wigner-D matrices as SO(3) Group Representation}
For the $SO(3)$ group, any representation $ {D}( {R})$ for $ {R}\in SO(3)$ can be reduced into a direct sum of $(2l+1)\times(2l+1)$ dimensional irreducible representations $ {D}^{l}( {R})$ of \textit{degree} $l\in\{0,1,2,\cdots\}$ such that
 \begin{equation}
      {D}( {R})= {U}\left[\bigoplus_{l=1}^{N}{ {D}^{l}( {R})}\right] {U}^{-1}\qquad \forall  {R}\in SO(3)
 \end{equation}
 where $\bigoplus$ denotes a direct sum\footnote{Direct sum can be intuitively understood as a concatenation/block-concatenation for vectors/matrices.}.
 Although there are infinitely many equivalent representations for such $ {D}^l$, a particularly preferred choice is one with a \textit{real basis}\footnote{Another commonly used choice of basis is the \textit{spherical basis} whose representations are unitary}. On this basis, all the representations $ {D}^l$ are orthogonal matrices. These matrices are called the \textit{(real) Wigner D-matrices} \cite{aubert2013alternative, se3t, thomas2018tensor}.

\subsubsection{Steerable Function and Vectors}
\paragraph*{Steerable Function}
A function is steerable under a transformation group $\G$ if any transformation $g \in \G$ on $f$ can be represented as a linear combination of a fixed, finite set of basis functions $\{ \phi_i\}$.
\[
{L}_g f= \sum_{i=1}^n \alpha_i (g) \phi_i = \alpha^T(g) \Phi,
\]
where ${L}_g f$ is the left-regular representation of the group $G$ that transforms    $f$.
The concept of steerability was first coined in the computer vision community \cite{freeman1991design}.
Steerable neural networks work with feature vectors consisting of these steerable feature vectors. 

% \JS{I should make a connection between Wigner-D and Spherical harmonics }
% AK:
% \paragraph*{Wigner D Matrices and Spherical Harmonics}
% The equivariant spherical harmonics-based representation can be derived for the case of equivariant convolutional networks \cite{weiler20183d}.
% \JS{Need to reduce and summarize more. We should not introduce more definitions here.}
% The transformation induced by a general correlation kernel $k$ on $\mathbb{R}^3$ can be represented by:
% \[
% (k \star f)(x) = \int_{\mathbb{R^3}}k(y-x)f(y)dy
% \]
% This kernel is equivariant to a $\SE$ transformation if it satisfies $k(gx) = \rho_2(R)k(x)\rho_1^{-1}(R)$ \cite{weiler20183d}, where $\rho_1(R)$ and $\rho_2(R)$ are representations of $\SO$ on the input domain and output domain, respectively, and with $g = (p,R) \in \SE$.
% % Since these cross-correlations layers are already translation invariant, it suffices to satisfy $k(Rx) = \rho_2(R)k(x)\rho_1^{-1}(R)$ for this kernel to be rotational equivariant. 
% \JS{The transition from general kernel space to steerable vector space is not smooth. To be smooth, we need first to define kernel to be $k:\mathbb{R}^3 \to \mathbb{R}^{K_{n+1} \times K_n} $, where $\mathbb{R}^{K_{n+1}}$ is vector space of $\mathcal{F}_{n+1}$ so on, by specifying $\mathbb{R}^{K_{n+1}}$ to be $\mathbb{R}^{2l+1}$}
% Here, the kernel is just redefined to take in a combined input $x$ for transformations on $\SO$. This can be expressed in terms of Wigner D matrices, which are irreducible representations of the $\SO$ group.
% \[
% k^{ij} = D^{j}(r)k^{jl}D^{l}(r)^{-1}
% \] 
% After vectorizing the kernel and applying a change of basis to block diagonalize all the elements, we produce an expression in terms of the matrices on the diagonal and transformed kernel bases $\eta_{i,j}(Rx)$ and $\eta_{i,j}(x)$.
% \[
% \eta^jl(rx) = \left[\bigoplus^{j+l}_{J = j-l} D^{J}(R)\right]\eta^{jl}(x)
% \]
% The solution to this equation is well known in group theory and physics as spherical harmonics of order $J$. Kernels defined by a sum of spherical harmonics can be considered a subset of the larger space of viable kernels, and intuitively, this subset is produced by restricting kernels to follow the rotation equivariance relationship.

\paragraph*{Steerable Feature Vectors}
Steerable feature vectors are vectors that transform via Wigner-D matrices \cite{aubert2013alternative, se3t, thomas2018tensor}, which are representations of $SO(3)$ and $SU(2)$. Wigner-D matrices are used to define any representation and are irreducible. A type-$l$ steerable vector space $V_l$ is a $(2l+1)$-dimensional vector space that is acted upon by a Wigner-D matrix of order $l$. For example, if $h$ is a type-$3$ vector in $V_3$, then it is transformed by $g \in SO(3)$ via  $h \rightarrow D^3(g)h$.
As mentioned above, SH is used to formulate a type-$l$ vector and is steerable via the Wigner-D matrix. 

Any vector $x \in \Real^3$ can be converted into a type-$l$ vector by the evaluation of spherical harmonics $Y_m^{l}: S^2 \rightarrow \Real$ at $n = \frac{x}{ \| x\|}$. In particular, for any $x \in \Real^3$, $\mathbf{Y}^l$ is a type-$l$ steerable vector. 
\begin{equation*}
    \mathbf{Y}^l = \left(Y_m^l\left(\frac{x}{\|x\|}\right) \right)^T_{m = -l, -l+1, \dots, l}
\end{equation*}

Consider a function in terms of spherical bases, with {\it coordinates} $a^l = [a_0^l, \cdots, a_l^l]^T$:
\begin{equation*}
    f_a = \sum_{l=0}^\infty \sum_{m=-l}^l a_m^l Y_m^l = \sum_{l=0}^\infty (\mathbf{a}^l)^T \mathbf{Y}^l,
\end{equation*}
where $\mathbf{a}^l = (a_{-l}^l, a_{-l+1}^l, \cdots, a_{l-1}^l, a_l^l)^T$.
It is steerable since we can show that   \cite{brandstetter2021geometric}
\begin{equation}\label{eq:Lgf}
\begin{split}
    L_g f_a(n) &=  f_{D(g)a} (n) \\&=\sum_{i=1}^n \alpha_i (g) \phi_i = \alpha^T(g) \Phi=(D(g) a)^T \Phi,
\end{split}
\end{equation}
 where $\alpha(g)=D(g) a$ and $\Phi= (Y_0^{0}, Y_{-1}^{1}, Y_0^{1}, \cdots)^T$. Alternatively,
\begin{equation}
    \begin{split}
        L_g f_a(n) &= f_a(g^{-1} \circ n) \\
        &= \sum_{l=0}^\infty (\mathbf{a}^l )^T D^l(g^{-1})\mathbf{Y}^l = \sum_{l=0}^\infty (\mathbf{a}^l )^T D^l(g)^T\mathbf{Y}^l\\
        &= \sum_{l=0}^\infty (D^l(g) \mathbf{a}^l)^T \mathbf{Y}^l
    \end{split}
\end{equation}
where the definition of left-regular representation is used, and property of the Wigner-D matrix, i.e., $D^l(g^{-1}) = D^l(g)^T$, for $g\in \SO$ is utilized \cite{lee2018real}. The $D(g)$ in \eqref{eq:Lgf} can be understood as block diagonal stack of $D^l(g)$, i.e., $D(g) = \text{blkdiag}(D^0(g), D^1(g), D^2(g) \cdots)$.

\subsubsection{Steerable Group Convolution}
 Consider an input feature map $f: \Real^3 \rightarrow \Real$.
In many applications, we want to perform template matching for arbitrary translations and rotations. We can then    define the roto-translation lifting correlation from $\Real^3$ (i.e., the original  feature map input space) to the space of $SE(3)$ with $g=(x,R)$ such as 
 \[
 \begin{split}
y(g)&=(\W \star_{SE(3)}  f )  (g) = \langle L_{g}\W, f \rangle_{\mathbb{L}_2 (\Real^3)}\\ &=  \langle L_{(x, R)}\W, f \rangle_{\mathbb{L}_2 (\Real^3)}= \langle L_{x} L_R \W, f \rangle_{\mathbb{L}_2 (\Real^3)} \\
&=\int_{\Real^3} \W(g^{-1} \circ  \tilde x)f(\tilde x) d \tilde x =\int_{\Real^3} \W(R^{-1} (\tilde x-x)) f(\tilde x) d \tilde x.
 \end{split}
 \]

The subsequent group convolution is then performed in the lifted higher dimensional feature maps of $SE(3)$.
\[
\begin{split}
y(g) 
 &= \langle L_{g}\W, f \rangle_{\mathbb{L}_2 (SE(3))}\\
&= 
 \int_{SE(3)} \W (g^{-1} \circ \tilde g) f(\tilde g) d \tilde g.
%&= \int_{\Real^3} \int_{S^2} \W(R^{-1} (\tilde x- x),  \tilde \theta -\theta) f(\tilde x, \tilde \theta) d \tilde x d \tilde \theta.
 \end{split}
  \]

Consider now a 3D convolution kernel that is expanded in a spherical
harmonic basis (up to degree $l$):  
\[
\W(x)=\W_{c (\| x\|)} (x):= \sum_{\ell=0}^L \sum_{m=-\ell}^{\ell} c_m^{(\ell)} (\| x\|) Y_m^{\ell} \left ( \frac{x}{\|x\|}\right ),
\]
where $c= (c_0^{(0)}, c_{-1}^{(1)}, c_0^{(1)}, \cdots)^T$ is the collection of basis coefficients that depends on $\|x\|.$
Due to \eqref{eq:Lgf}, we conclude that the kernel is steerable via the transformation of $c$ by its $SO(3)$ representation $D(R)$
\[
L_g  \W(x)=\W(g^{-1}x)=\W_c(R^{-1}x)=\W_{D(R)c(\| x\|)} (x).
\]
Using this steerable kernel, we perform $SE(3)$ lifting convolution, i.e., $g = (x,R) \in \SE$ such as
\[
\begin{split}
&y(g) =y(x,R)
= \langle L_{g}\W, f \rangle_{\mathbb{L}_2 (\Real^3)}\\
&=\int_{\Real^3} L_g \W(\tilde x) f(\tilde x) d \tilde x =\int_{\Real^3} \W( R^{-1}  (\tilde x-x)) f(\tilde x) d \tilde x\\
&=\int_{\Real^3} \W_{D(R)c} (\tilde x-x)  f(\tilde x) d \tilde x =\int_{\Real^3} ({D(R)c})^T \Phi (\tilde x- x)  f(\tilde x) d \tilde x\\
&=({D(R)c})^T \int_{\Real^3}  \Phi (\tilde x- x)  f(\tilde x) d \tilde x\\
&=({D(R)c})^T \hat f^{\Phi} (x)
\end{split}
\]

Here, any transformation $g \in G$ on $\W$ can be represented as a linear combination of a set of basis $\Phi$. Hence, $({D(R)c})^T $ can be pulled out of the convolutional integral. Therefore, $y(g)$ is a function of $g$ without further convolution since the feature vector is already convoluted with a collection of basis, which does not require discretization in $R$ as in (non-steerable) group convolution in \eqref{eq:LiftingCov}.

\subsubsection{Clebsch-Gordan Tensor Product}
Clebsch-Gordan (CG) tensor product is used in steerable linear layers, which map between steerable input and output vector spaces. Similar to regular neural networks, where matrix-vector multiplication is used to map between input and output vector spaces, the CG tensor product is used to map between steerable input and output vector spaces. The learnable CG tensor product is the key component of steerable neural networks, similar to the learnable weight matrix-feature multiplication in regular neural networks.

For any two steerable vectors $u \in  V_{\ell_1}$ (type-$l1$) and $v \in  V_{\ell_2}$ (type-$l2$), the CG tensor product’s output is
again steerable with a $SO(3)$ representation $D(R)$, $R\in \SO$ as follows. 
\[
D(R) (u \otimes v)= (D^{l_1} (R) u ) \otimes (D^{l_2} (R) v ),
\]
where $u \otimes v = u v^T$.

The output resulting vector $\text{vec} (u v^T)$ is steered by a representation $D(R) = D^{l_2}(R) \otimes D^{l_1}(R)$.
\[
\begin{split}
\text{vec} \left ( (D^{l_1} (R) u) (D^{l_2} (R) v)^T   \right ) &=\text{vec} \left ( (D^{l_1} (R) u) v^T D^{l_2} (R)^T   \right )\\
&=(D^{l_2} (R) ) \otimes (D^{l_1} (R)   )\text{vec} (u v^T)\\
&=D(g)  \text{vec} (u v^T),
\end{split}
\]
where $\text{vec}(AXB) = (B^T \otimes A) \text{vec}(X)$ was used in the second line, with $A \otimes B$ denoting Kronecker product of the two matrices. Moreover, $\text{vec}(\cdot)$ is a vectorize operator, which vectorizes the matrix by stacking its columns. 

Tensor products are also important because they can be used to construct new vectors of different types.
By a change of basis, the tensor product $ {u}\otimes  {v}$ can be decomposed into the direct sum of type-$l$ vectors using the \textit{Clebsch-Gordan coefficients} \cite{thomas2018tensor, zee, griffiths2018introduction}. Let this type-$l$ vector be $( {u}\otimes  {v})^{l}$. The $m$'th components of this vector is calculated as:
\begin{equation}
    ( {u}\otimes  {v})^{l}_m=\sum_{m_1=-l_1}^{l_1}\sum_{m_2=-l_2}^{l_2} C^{(l,m)}_{(l_1,m_1)(l_2,m_2)}u_{m_1}v_{m_2}
\end{equation}
where  $C^{(l,m)}_{(l_1,m_1)(l_2,m_2)}$ is the Clebsch-Gordan coefficients in real basis, which can only be nonzero for ${|l_1-l_2|\leq l \leq l_1+l_2}$.

\subsection{$SE(3)$-Equivariant Graph Neural Networks} \label{appendix_equiv_gnn}
Generated from RGBD input, 3D point clouds have become another major source of vision inputs. Unlike 2D images, where only the projected information is provided, 3D point clouds provide more spatial information. Importantly, the points in the point cloud can be interpreted as $\mathbb{R}^3$ vector, i.e., $x,y,z$ coordinates, equipped with feature vectors, e.g., RGB values of each point, the point clouds can be well handled by $SE(3)$ equivariant graph neural networks.

 Let $\mathcal{V}$ be a (steerable) vector space and $\mathcal{X}$ and $\mathcal{Y}$ be (point-cloud data) sets with a group action $\circ$ such that $g\circ (h\circ \dX)=(gh)\circ \dX$ and $g\circ (h\circ \dY)=(gh)\circ \dY$ where $\forall g,h\in G$, $\dX\in\mathcal{X}$, $\dY\in\mathcal{Y}$, and $\mathcal{O}$ denotes point-cloud data.
 A map $ {f}(\dX|\dY):\mathcal{X}\times\mathcal{Y}\rightarrow\mathcal{V}$ is said to be $G$-\textit{equivariant} if
 \begin{equation}
      {D}_{\mathcal{V}}(g) {f}(\dX|\dY)= {f}(g\circ \dX|g\circ \dY),
 \end{equation}
 where $ {D}_{\mathcal{V}}$ is a representation of $G$ acting on $\mathcal{V}$. In the special case where $ {D}_{\mathcal{V}}= {I}$, the map $ {f}(\dX|\dY)$ is said to be \textit{$G$-invariant}.

 A translation invariant and $SO(3)$-equivariant type-$l$ vector field, or simply an \textit{$SE(3)$-equivariant type-$l$ vector field}, $ {f}( {x}|\dX):\mathbb{R}^3\times\mathcal{X}\rightarrow\mathbb{R}^{2l+1}$ is a special case of $SE(3)$-equivariant map such that
 \begin{equation}
      {D}^l( {R}) {f}( {x}|\dX)= {f}( {R} {x}+ {p}|g\circ \dX)\quad \forall g=(  {p}, R)\in SE(3), 
 \end{equation}
 where  $ {p}\in\mathbb{R}^3$, $ {R}\in SO(3)$ and $g\circ {x}= {R} {x}+ {p}$.
 From now on, we simply denote the action of $g\in SE(3)$ on $ {x}\in\mathbb{R}^3$ as $g {x}$ instead of $g\circ  {x}$ for brevity. 
% A detailed recipe for constructing such $SE(3)$-equivariant vector fields when $\dX\in \mathcal{X}$ is given as a graph is described in the following subsection.
Graph neural networks are often used to model point cloud data \cite{wang2019dynamic, te2018rgcnn, shi2020point}. 
$SE(3)$-equivariant graph neural networks \cite{thomas2018tensor, se3t, liao2022equiformer,brandstetter2021geometric} exploit the roto-translation symmetry of graphs with spatial structures.
We briefly introduce Tensor Field Networks (TFNs) \cite{thomas2018tensor} and one of its variants, the $SE(3)$-transformers \cite{se3t}, as the backbone graph networks for equivariant deep learning models. Furthermore, we briefly introduce some works to reduce the computational complexity of the tensor product - Equivariant Spherical Channel Network (eSCN) and Gaunt Tensor Product.

\subsubsection{Tensor Field Networks} Tensor field networks (TFNs) \cite{thomas2018tensor} are $SE(3)$-equivariant models for generating representation-theoretic vector fields from a point cloud input. TFNs construct equivariant output feature vectors from equivariant input feature vectors and spherical harmonics. Spatial convolutions and tensor products are used for the equivariance.

Consider a featured point cloud input with $M$ points given by 
\[\dX=\{( {x}_1, {f}_1),\cdots,( {x}_M, {f}_M)\},\] where $ {x}_i\in\mathbb{R}^3$ is the position and $ {f}_i$ is the equivariant feature vector of the $i$-th point.
Let $ {f}_i$ be decomposed into $N$ vectors such that $ {f}_i=\bigoplus_{n=1}^{N} {f}_i^{(n)}$, where $ {f}_i^{(n)}$ is a type-$l_n$ vector, which is $(2l_n+1)$ dimensional.
Therefore, we define the action of $g=( p, {R})\in SE(3)$ on $\dX$ as
\begin{equation*}
   g\circ \dX=\{(g{x}_1, {D}( {R}) {f}_1),\cdots,(g {x}_M, {D}( {R}) {f}_M)\},
\end{equation*}
where ${p}\in\mathbb{R}^3$, ${R}\in SO(3)$,  and $ {D}( {R})=\bigoplus_{n=1}^{N} {D}_{l_n}( {R})$.

Consider the following input feature field $ {f}_{(in)}( {x}|X)$ generated by the point cloud input $X$ as
\begin{equation}
     {f}_{(in)}( {x}|X)=\sum_{j=1}^{M} {f}_{j}\delta^{(3)}( {x}- {x}_j),
\end{equation}
where $\delta^{(3)}( {x}- {y})=\prod_{\mu=1}^3\delta(x_\mu-y_{\mu})$ is the three-dimensional Dirac delta function centered at $ {x}_j$. 
Note that this input feature field is an $SE(3)$-equivariant field, that is:
\begin{equation*}
      {f}_{(in)}(g {x}|g\circ \dX) =  {D}( {R}) {f}_{(in)}( {x}|\dX)\quad\forall\ g=(p,  {R})\in SE(3).
\end{equation*}

Now consider the following output feature field by a convolution
\begin{equation}
\label{eqn:tfn}
    \begin{split}
     {f}_{(out)}&( {x}|\dX)=\bigoplus_{n'=1}^{N'} {f}_{(out)}^{(n')}( {x}| \dX)\\
    &=\int{d^3 {y}} {W}( {x}- {y}) {f}_{(in)}( {y}|\dX)=\sum_{j} {W}( {x}- {x}_j) {f}_{j},
    \end{split}
\end{equation}
where the convolution kernel $ {W}( {x}- {y})\in \mathbb{R}^{dim( {f}_{(out)})\times dim( {f}_{(in)})}$
 whose $(n',n)$-th block $ {W}^{(n',n)}( {x}- {y})\in\mathbb{R}^{(2l_{n'}+1)\times(2l_n+1)}$ is defined as follows:
\begin{equation}
    \label{eqn:tfn_kernel_const}
    \begin{split}
        \left[ {W}^{(n',n)}( {x})\right]^{m'}_{m}\!=\!\sum_{J=|l_{n'}-l_n|}^{l_{n'}+l_n}\phi^{(n',n)}_{J}(\| {x}\|)\sum_{k=-J}^{J}C^{(l_{n'},m')}_{(l_n,m)(J,k)}Y^{J}_{k}\left( {x}/\| {x}\|\right).
    \end{split}
\end{equation}
Here, $\phi^{(n',n)}_{J}(\| {x}\|):\mathbb{R}\rightarrow\mathbb{R}$ is some learnable radial function. 
The output feature field $ {f}_{(out)}( {x}|X)$ in \eqref{eqn:tfn} is proven to be $SE(3)$-equivariant \cite{thomas2018tensor, se3t}. 

\paragraph*{$SE(3)$-Transformers} The $SE(3)$-Transformers \cite{se3t} are variants of TFNs with self-attention. Consider the case in which the output field is also a featured sum of Dirac deltas
\begin{equation}
     {f}_{(out)}( {x}|X)\!=\!\sum_{j=1}^{M} {f}_{(out),j}\delta^{(3)}( {x}- {x}_j),
\end{equation}
where $ {x}_i$ is the same point as that of the point cloud input $X$. The $SE(3)$-Transformers apply type-0 (scalar) self-attention $\alpha_{ij}$ to \eqref{eqn:tfn}:
\begin{equation}
\begin{split}
     {f}_{(out),i}=\sum_{j\neq i}\alpha_{ij} {W}( {x}- {x}_j) {f}_{j}+\bigoplus_{n'}^{N'}\sum_{n=1}^{N} {W}_{(S)}^{(n',n)} {f}_{j}^{(n)},
\end{split}
\end{equation}
where the $ {W}_{(S)}^{(n',n)}$\ \ term is called the \textit{self-interaction} \cite{thomas2018tensor}. $ {W}_{(S)}^{(n',n)}$ is nonzero only when $l_n'=l_n$. The self-interaction occurs where $i=j$ such that $ {W}(x_i-x_j)=W(0)$. The self-interaction term is needed because $ {W}$ is a linear combination of the spherical harmonics,  which are not well defined in $ {x}=0$. Details about the calculation of the self-attention $\alpha_{ij}$ can be found in \cite{se3t}.
% \section{PAPER SIZE AND FORMAT}


\subsubsection{Handling Computational Complexity of Tensor Product}
Equivariant Spherical Channel Network (eSCN)~\cite{passaro2023reducing} introduces a mathematically equivalent alternative to the original tensor product operation in TFNs with improved efficiency. eSCN reduces the computational complexity of tensor product from $O(L^6)$ to $O(L^3)$ where $L$ is the highest feature type. This unlocks the utilization of much higher frequency features, which have been reported to improve the accuracy in robotic manipulation tasks \cite{gao2024riemann, hu2024orbitgrasp}. The details of the eSCN can be found in Appendix~\ref{sec:appendix_eSCN}. 

In \cite{luo2024enabling}, Clebsch-Gordan coefficients are connected to the Guant coefficients, which are integrals of products of three spherical harmonics. Through this transformation, the complexity of full CG tensor products is reduced from $O(L^6)$ to $O(L^3)$. 
% \HR{TODO: This section will review recently proposed Gaunt Tensor Product framework that reduces the complexity of C-G tensor product from $O(L^6)$ to $O(L^3)$}

% \begin{equation}
%     \begin{split}
%     \left[\mathbf{S_0}\right]_{m'm}&=\begin{cases}
%         \left[\mathbf{S_0}\right]_{-m-m} & \text{if }\ m'=m
%         \\
%         0 & \text{else}
%     \end{cases}
%     \\
%     \left[\mathbf{A_0}\right]_{m'm}&=\begin{cases}
%         -\left[\mathbf{A_0}\right]_{m'm} & \text{if }\ m'=-m
%         \\
%         0 & \text{else}
%     \end{cases}
%     \end{split}
% \end{equation}

\subsection{PointNet-based Equivariant Neural Network} PointNet \cite{qi2017pointnet} is a neural network architecture designed to process point clouds directly, ensuring permutation invariance so that the output remains consistent regardless of the order of the input points. PointNet introduces T-net, an affine transformation network, to learn automatic transformation. The motivation of the T-net is to somewhat mimic equivariance property, but there is no theoretical motivation or guarantee.

The Vector Neurons (VN)\cite{deng2021vector} extends scalar neurons to 3D vector neurons, enabling the construction of $SO(3)$-equivariant neural networks. VN introduces essential building blocks such as linear layers, non-linearities, pooling, and normalization, which ensure $SO(3)$-equivariance. Based on these building blocks, the VN framework constructs $SO(3)$-equivariant PointNet, known as VN-PointNet. 

% \JS{Introduce Vector Neuron here}

% \subsection{Wigner-Eckart Theorem of G-steerable Kernels}
% \HR{TODO: This section will review the general theory and recipe for building equivariant neural networks for arbitrary Lie groups.}

% \subsubsection{Peter-Weyl theorem}
% \HR{TODO: Theoretical background for steerable functions on a compact Lie group and their homogeneous spaces.}

==> Old_2024_1130/Section4_RelatedWorks.tex <==
% \JS{Literature review: The works that Hyunwoo mentioned can be briefly introduced here.}

% \JS{Then, we say: We introduce some works that are worth explanation(?)}

% \JS{Bi-equivariant-related works}

Equivariant neural networks can significantly improve data efficiency and generalizability in robot learning, where data collection is often expensive and large datasets are needed. Early efforts to leverage symmetry in this area include Transporter Network \cite{zeng2020transporter}, which utilized the $SO(2)$ symmetry of 2D top-down settings for pick-and-place tasks. This approach was later enhanced by Equivariant Transporter \cite{huang2022equivariant}, which improved sample efficiency by leveraging equivariant networks over $SO(2)\times SO(2)$. Fourier Transporter \cite{huang2024fourier} further advanced the field by enabling convolutions directly in $SE(3)$ non-Euclidean space, leveraging a parameterization in the Fourier space.

In grasp detection, Edge Grasp Network \cite{huang2023edge} introduced a novel approach utilizing the $SE(3)$-invariance for grasp quality evaluation. Orbit Grasp \cite{hu2024orbitgrasp} took this further by representing grasp directions with spherical harmonics, allowing the model to infer efficiently from a continuous range of directions.

Building on the Diffusion Policy (DP) \cite{chi2023diffusion}, which combines diffusion models with action chunking, EquiBot \cite{yang2024equibot} incorporates $SIM(3)$-equivariance using the Vector Neuron framework, as proposed by EquivAct \cite{yang2024equivact} into the DP framework. Similarly, the Equivariant Diffusion Policy \cite{wang2024equivariant} extends the DP framework by integrating $SO(2)$-equivariant noise prediction networks. This approach leverages irreducible representations to model how $SO(2)$ acts on an $SE(3)$ gripper pose. ET-SEED \cite{tie2024seed} also leverages $SE(3)$-equivariance but restricts equivariant operations to address the challenges in training caused by the strict constraints imposed by full equivariance.

Instead of diffusion models, ActionFlow \cite{funk2024actionflow} and EquiGraspFlow \cite{lim2024equigraspflow} utilize flow matching to quickly generate $SE(3)$-equivariant action sequences and grasp poses, respectively.

The equivariant neural networks can be utilized for symmetry in robot manipulation tasks. Numerous robot learning researchers have leveraged symmetry in $SE(3)$ \cite{zeng, huang2022equivariant, fourtran, ndf, ryu2022equivariant, ryu2024diffusion}. Especially, \cite{rndf, ryu2022equivariant, ryu2024diffusion, fourtran} introduced bi-equivariance of the pick and place task. 

Incorporating group equivariance into Reinforcement learning (RL) offers a promising approach to one of RL's key challenges: sample inefficiency due to extensive trial-and-error from scratch. Recent works \cite{rl3, finzi2021residual, theile2024equivariant, wang2022so, kohler2023symmetric, wang2022robot, wang2022equivariant, nguyen2023equivariant, tangri2024equivariant} have shown the potential of these methods to enhance both sample efficiency and performance. In particular, \cite{wang2022equivariant, wang2022so} introduced a novel theoretical framework, the group-invariant MDP, which proves the existence of group-invariant $Q$-functions in $Q$-learning methods.

In this section, we will provide a detailed review of a few notable works for two major categories of equivariant deep learning in robotics: imitation learning and reinforcement learning. 

\subsection{Imitation Learning}\label{il}
Imitation learning provides a way to teach a robot by showing it the desired behavior, simplifying the teaching process, and mitigating detailed programming or laborious reward function engineering. However, the cost of collecting data, such as expensive hardware, a well-oriented laboratory environment, expertise with the robot, and a significant amount of time, decreases the scalability and efficiency of the method. Neural Descriptor Fields (NDF)\cite{ndf} implement object representation with a category-level descriptor using Vector Neurons (VN) \cite{deng2021vector}, enabling the learning of manipulation tasks from 5–10 demonstrations in both simulation and real-world settings. However, NDFs require pre-trained object segmentation and do not operate in an end-to-end manner. On the other hand, Equivariant Descriptor Fields (EDF)\cite{ryu2022equivariant} achieve local equivariance by utilizing the locality of Equiformer\cite{liao2022equiformer} and $SE(3)$-Transformer\cite{se3t}. This enables EDFs to perform training in an end-to-end manner without pre-training and object segmentation. Furthermore, EDF introduces a bi-equivariant energy-based model on $SE(3)$ for the pick and place problem. The bi-equivariant energy-based model on $SE(3)$ is written as :
\[
P(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) = \frac{\exp{[-E(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp})]}}{Z}
\]
\[
Z = \int_{SE(3)} dg \exp[-E(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp})]
\]
where $P$ is an energy-based model on the $SE(3)$ manifold, $E$ is an energy function, $g = (p, R) \in SE(3), p \in \Real^3, R \in SO(3)$ and $\mathcal{O}$ denotes point clouds data.
By addressing equivariance in both the scene and the grasp, EDF achieves high sample efficiency and robustness when handling out-of-distribution data. The bi-equivariance condition of the model can be written as follows: 
\[
\begin{split}
P(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) &= P(\Delta g_w g | \Delta g_w \circ \mathcal{O}^{scene},\mathcal{O}^{grasp}) \\
&= P(g \Delta g_e^{-1}|\mathcal{O}^{scene}, \Delta g_e \circ \mathcal{O}^{grasp})
\end{split}
\]
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/bi_equiv_ed.jpg}
    \caption{Bi-equivariance. (a) The scene equivariance and (b) grasp equivariance consider the transformation of world and grasped object. The end-effector pose should be transformed equivariantly with the transformation.}
    \label{fig:biequiv}
\end{figure}
The energy-based model consists of $SE(3)$-equivariant type-$l_n$ vector field generated by observation.
\[
E(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) =
\]
\[
\int_{\mathbb{R}^3} d^3 x \; \rho(x|\mathcal{O}^{grasp})||\varphi(gx|\mathcal{O}^{scene})-D(R)\psi(x|\mathcal{O}^{grasp}) ||^2
\]
\JS{Define $\rho$, $\phi$, $\psi$ terms respectively}
Diffusion-EDFs\cite{ryu2024diffusion} improved the training time of EDFs, maintaining end-to-end training manner and data efficiency utilizing the bi-equivariance and locality of robotic manipulation. Diffusion-EDFs proposed a bi-equivariant score function given as follows:
\JS{Define $s$}
\[
s(\Delta g g | \Delta g \circ \mathcal{O}^{scene}, \mathcal{O}^{grasp}) = s(g | \mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
\[
s(g\Delta g^{-1}|\mathcal{O}^{scene}, \Delta g \circ \mathcal{O}^{grasp}) = [\Ad_{\Delta g}]^{-T}s(g | \mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
with 
\[
\quad \Ad_g = \begin{bmatrix}
            R & \hat{p} R \\
            0 & R
            \end{bmatrix}\\
\]
where $R \in \text{SO}(3)$, $p \in \Real^3$ and $\hat{p}$ is the skew-symmetric matrix of $p$.
Diffusion-EDFs split the score model into translation and rotational parts and propose the models of each part satisfying equivariance conditions.
\[
s_t(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) = [s_{\nu;t}\oplus s_{\omega ; t}](g|\mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
\[
s_{\nu ; t}(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) =
\]
\[
 \int_{\mathbb{R}^3} d^3 x \; \rho_{\nu ; t}(x|\mathcal{O}^{grasp})\Tilde{s}_{\nu ; t}(g, x|\mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
\[
 s_{\omega ; t}(g|\mathcal{O}^{scene}, \mathcal{O}^{grasp}) =
\]
\[
\int_{\mathbb{R}^3} d^3 x \; \rho_{\omega ; t}(x|\mathcal{O}^{grasp})\Tilde{s}_{\omega;t}(g, x|\mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
\[
+ \int_{\mathbb{R}^3} d^3 x \; \rho_{\nu ; t}(x|\mathcal{O}^{grasp})x \wedge \Tilde{s}_{\nu;t}(g, x|\mathcal{O}^{scene}, \mathcal{O}^{grasp})
\]
\JS{Define $s_{v,w}$, $\tilde{s}$, wedge operator, $\rho$}
The details of  bi-equivariant score model and diffusion-based learning on the $SE(3)$ manifold for visual robotic manipulation are provided in Diffusion-EDFs.

RiEMann\cite{girolami2011riemann} is a $SE(3)$-equivariant robot manipulation framework with near real-time. RiEMann learns an affordance map with one type-0 vector field to get a point cloud ball $B_{ROI}$ with $SE(3)$-Transformer \cite{se3t}.
\[
f_{in}(x) = \bigoplus_{i=0}^{3}f_0^{i}(x)
\]
The region is extracted from the affordance map with predefined radius. This leads to reduction of computation complexity and memory usage. Position and orientation network use the points in the region. RiEMann designed the output feature of translation and rotation matrix with 1 type-0 vector field and 3 type-1 vector fields each.
\[
f_{out}(x) = f_0(x) + \bigoplus_{j=0}^{3}f_1^j(x)
\]

Fourier Transporter \cite{fourtran} proposed $SE(3)$ bi-equivariant model using 3D convolutions and a Fourier representation of rotation for pick and place problems. 
Similar to EDFs \cite{ryu2022equivariant} and Diffusion-EDFs \cite{ryu2024diffusion}, the proposed method utilize coupled SE($d$)$\times$SE($d$)-symmetries for the problem. 
Let's assume $d = 3$, the 3D pick and place problem. The policy for pick and place is formulated as $p(a_t|o_t) = p(a_{place}|o_t, a_{pick})p(a_{pick}|o_t)$. 
The SE(3)-equivariant pick network is a function $f_{pick} : o_t \mapsto p(a_{pick}|o_t)$, where $p(a_{pick}|o_t)$ is a steerable field. 
The base space of the steerable field determines the pick location $\Real^3$, and the fiber space encodes the distribution of pick orientations $\text{SO}(3)$. We can represent the distribution $p(a|o_t)$ as $\Real^3 \rightarrow \{\text{SO}(3) \rightarrow \Real \}$. Especially, $L_g(p)(h) = p(g^{-1} \circ h)$ is the transformation of the distribution with left-action. $L_g$ notation is a left-regular representation of group element $g$ to distribution, and $\circ$ is a group action of $g$ with respect to $h$.

The pick pose distribution should follow a transformation on observation.
\[
f_{pick}(g\circ o_t) = \text{Ind}_{\rho_L}(g) f_{pick}(o_t), \quad \forall g \in \text{SE}(3)
\]
The action of $g$ via representation $\rho$ on steerable feature vector fields $f$ is defined as $\text{Ind}_{\rho}(g)(f)(x) = \rho(g) f(\rho_1 (g)^{-1} x)$. $\rho(g)$ is the fiber action which transforms the pick orientation, and the base space action $\beta (g)f(x) = f(\rho_1 (g)^{-1}x)$ rotates the pick location. The standard representation $\rho_1$ of $\text{SO}(3)$ for one group element is a standard $3 \times 3$ rotation matrix. The irreducible representation $\rho_1$ of $\text{SO}(3)$ is the Wigner D-matrix $D^1 (\alpha, \beta , \gamma)$, a $3 \times 3$ matrix when expressed in terms of Euler angles. The grasped object can be represented as a voxel patch centered on the pick location with the assumption that the object does not move or deform. The place network is $f_{place}: (c, o_t) \to p(a_{place}|o_t, a_{pick})$ where $c$ is the cropped image centered at the pick location. The network should satisfy the bi-equivariance constraint in the pick and place problem. 
\[
\begin{split}
    &f_{place}(g_1 \circ c, g_2 \circ o_t) = \text{Ind}_{\rho_L}(g_2)\rho_{R}(g_1^{-1})f_{place}(c, o_t), \\
    &\forall g_1, g_2 \in \text{SE}(3)
\end{split}
\]

The place action should transform equivariantly with actions on the picked object and actions on the observation. The template matching method is used to realize place symmetry. The cross-correlation between a dynamic kernel $\kappa(c)$ and a feature map $\phi(o_t)$ is used for pick action probability as $f_{place}(c, o_t) = \kappa(c) \star \phi(o_t)$, where $\star$ denotes the cross-correlation.

The dynamic kernel $\kappa(c)$ is introduced and utilized to perform convolutions on the Fourier space. The dynamic kernel is composed of dense feature maps, which are lifted with a finite number of rotations and Fourier transforms to the channel space. The dense feature map of crop $c$ is  $\psi(c)$. We rotate the dense feature map with a finite number of rotations $\Tilde{G} = \{g_i | g_i \in \text{SO}(3)\}_{i=1}^m$ and stack the rotated feature maps. The stack of fully rotated signals can be defined as follows:
% A stack of rotated feature maps 
\[
\begin{split}
    &\mathcal{L}^{\uparrow}[f](x) = \{ f(g_1^{-1}x), f(g_2^{-1}x) \dots , f(g_m^{-1}x)\},\\
    &\forall x \in \mathbb{R}^n , g_i \in \Tilde{G},
\end{split}
\]
The stack of fully rotated dense feature maps of the cropped image is $\mathcal{L}^{\uparrow}(\psi(c))$.

The Fourier transform over $\text{SO}(3)$ is defined as $\mathcal{F}(f) = (\hat{f}^l)_{l=0}^{\infty}$ where 
\[
\forall g \in \text{SO}(3), \quad f(g) = \sum_{l=0}^{\infty}\sum_{k,k'=-l}^{l}\hat{f}^l_{kk'}D^l_{kk'}(g)
\]
and $f : \text{SO}(3) \rightarrow \Real$, $D^l$ are the Wigner D-matrices.
Let $\mathcal{F}^{+}$ denote Fourier transform to the channel-space. Then, $\mathcal{F}^{+}$ is applied to $\mathcal{L}^{\uparrow}(\psi(c))$ . Finally, the dynamic kernel becomes $\kappa (c) = \mathcal{F}^{+} [\mathcal{L}^{\uparrow} (\psi(c))] $.

The cross-correlation between the feature map $\phi(o_t)$ and the dynamic kernel $\kappa(c)$ is performed in the Fourier space. The place network is bi-equivariant if the $\psi(c)$ and the $\phi(o_t)$ satisfy the equivariant property and $\kappa(c)$ is a steerable convolutional kernel with $\rho_0$-type input. The details of $\SO$-Fourier Transform and proof of propositions are provided in Fourier Transporter \cite{fourtran}.

\subsection{Equivariant Reinforcement Learning}\label{rl}
\begin{figure}%[h!]
  \centering
\includegraphics[width=.8\linewidth]{Figures/GinvMDP.png}
  \caption{\textbf{Group-invariant MDP}. In a robot manipulation task, if the reward is 1 when the gripper achieves the goal, the group invariant MDP preserves the reward function and transition probability invariance under group actions.}
  \label{gimdp}
\end{figure}

{\color{red} [JC] should we replace all $\rho(g)$ in this section with $\circ$ for consistency? It appears that $\circ$ has been used in previous sections.} \JS{That's right, we shall use $\circ$ instead. We also need to update the same notation on 4.1. However, write down at some point that ``$g\circ s$ or $g\circ a$ is often denoted as $\rho_s(g) s$'' or something similar to this. It would be beneficial to add an example case of such group representation applied to the observation or action. (if possible)} 
Many equivariant reinforcement learning methods are based on the fundamental concept of group-invariant Markov decision process (MDP) \cite{wang2022so}, denoted as $\mathcal{M}_G=(S,A,P,R,G)$. 
% \JC{Added how the contraction is enabled}
It is based on the MDP homomorphisms \cite{ravindran2001symmetries, ravindran2004approximate}, a mapping that relates the original MDP, $M=(S,A,P,R,\gamma)$, to another abstract MDP, $M'=(S',A',P',R',\gamma)$. This homomorphism consists of two subjective functions $\alpha: S\rightarrow S'$ and $\beta: A\rightarrow A'$, which relate the state and action space of $M$ to the corresponding abstractions in $M'$. The policy in $M'$ can be utilized to derive a corresponding policy in $M$, which is given by:
\[
\begin{split}
    \pi(a|s)=\frac{\pi'(a'|\alpha(s))}{|\beta^{-1}(a')|}
\end{split}
\]
where $s\in S, a\in A, a'\in A'$ and $\pi'$ is the policy from the abstract MDP $M'$. Previous work has shown that if the abstract policy $\pi'$ is optimal, it can be used to derive the optimal policy in the original MDP, $M$ \cite{ravindran2001symmetries}.
Moreover, when the homomorphism follows a group framework, the optimal policy derived from the group-transformed MDP can be mapped back to induce the optimal policy in the original MDP. This approach leverages the symmetry within the problem to improve learning efficiency. The group-invariant MDP maintains its properties under the group-invariance of both the transition probability and the reward function, which can be expressed as:
\begin{itemize}
    \item Reward function: $R(s,a) = R(\rho_s(g) s,\rho_a(g)a)$
    \item Transition probability: \\
    \hspace*{\fill}
    $P(s'|s,a)=P(\rho_s(g)s'|\rho_s(g)s,\rho_a(g)a)$
\end{itemize}
where $g$ represents the group action in any group $\mathbb{G}$, and $\rho_s(g)$ and $\rho_a(g)$ represent the group actions $g$ on the state and action space, respectively. Due to the invariances, the optimal $Q$ function $Q^*(s,a)$ also becomes group-invariant and the optimal policy $\pi^*(s)$ is equivariant, which can be expressed as:
\begin{itemize}
    \item Q function: $Q^*(s,a)=Q^*(\rho_s(g)s,\rho_a(g)a)$
    \item Policy: $\pi^*(\rho_s(g)s)=\rho_{a}(g)\pi^*(s)$
\end{itemize}

Consider the Bellman optimality equation: 
\[
Q^*(s,a)=R(s,a)+\gamma\; \sup_{a'}\int_{s'}ds'P(s'|s,a)Q^*(s',a').
\]
Then, $Q^*$ of the transformed state-action pair, i.e., \\$Q^*(\rho_s(g)s', \rho_a(g)a')$ is given as:\\
\[
\begin{split}
    &Q^*(\rho_s(g)s,\rho_a(g)a)=R(\rho_s(g)s, \rho_a(g)a)\\ &+\gamma\; \sup_{a'}\int_{s'}ds'P(\rho_s(g)s'|\rho_s(g)s,\rho_a(g)a)Q^*(\rho_s(g)s', \rho_a(g)a').
\end{split}
\]
The reward function and transition probabilities are group-invariant, we can reindex the integral by setting $s'=\rho_s(g)s''$. Under the re-indexing, the optimal $Q^*$ function for the transformed state-action pair can be rewritten as 
\[
\begin{split}
    &Q^*(\rho_s(g)s,\rho_a(g)a)=R(\rho_s(g)s, \rho_a(g)a)\\
    &+\gamma\;\sup_{a'}\int_{s'}ds'P(\rho_s(g)s'|\rho_s(g)s, \rho_a(g)a)Q^*(\rho_s(g)s', \rho_a(g)a')\\
    &=R(s, a)+\gamma\;\sup_{a'}\int_{s'}ds'P(s'|s, a)Q^*(\rho_s(g)s', \rho_a(g)a').
\end{split}
\]
Introducing a new function $\bar{Q}(s,a)=Q(\rho_s(g)s, \rho_a(g)a)$, it follows that 
\[
\begin{split}
    \bar{Q}^*(s,a)=R(s, a) +\gamma\;\sup_{a'}\int_{s'}ds'P(s'|s, a)\bar{Q}^*(s', a').
\end{split}
\] Note that $Q^*(s,a)=Q^*(\rho_s(g)s, \rho_a(g)a)$ by the uniqueness of the Bellman optimal equation. Now, consider the optimal policy $\pi$ that maximizes $Q^*(s,a)$: $\pi^*(s)=\arg\max_{a}Q^*(s,a)$. One can relate this to the transformed state $\rho_s(g)s$. The policy in the transformed state is given by: 
\[
    \pi^*(\rho_s(g)s)=\arg\max_{a}Q^*(\rho_s(g)s,a).
\]
Using the fact that $Q^*(\rho_s(g)s,a)=Q^*(s,\rho_a(g^{-1})a)$, as implied from the uniqueness of the Bellman equation, we can rewrite: 
\[
    \pi^*(\rho_s(g)s)=\arg\max_{a}Q^*(s,\rho_a(g^{-1})a).
\] 
Letting $a=\rho_a(g)\bar{a}$, the equation can be expressed as: 
\[
\begin{split}
    \pi^*(\rho_s(g)s)&=\rho_a(g) \arg\max_{\bar{a}}Q^*(s,\rho_a(g^{-1})\rho_a(g)\bar{a})\\
    &=\rho_a(g)\pi^*(s)
\end{split}    
\]

Based on the group-invariant MDP, the authors in the prior work \cite{wang2022so} propose $SO(2)$-equivariant $Q$ learning methods. To construct group-invariant and equivariant layers for group-invariant vision-based $Q$ networks, they employ the networks from \cite{weiler2019general}, which encode the equivariant constraint on the kernel to achieve the equivariance. Using these equivariant networks, they construct equivariant networks for Deep $Q$-Networks (DQN), and both group-invariant critics and equivariant policies for Soft Actor-Critic (SAC). Experimental results demonstrate that the equivariant RL achieves superior sample efficiency compared to vanilla Q-learning methods, even when data augmentation or the auxiliary methods \cite{laskin2020reinforcement, kostrikov2020image, laskin2020curl} are employed. Additionally, the prior work shows better generalization over the group actions, outperforming other methods when given a fixed orientation of the input image rather than a random orientation.

In another prior work, \cite{kohler2023symmetric} builds upon the work by \cite{wang2022so} to propose an equivariant policy for the visual-force problems. Their approach utilizes the force input, in addition to the visual input, to facilitate equivariant policy learning. The experimental results indicate that the proposed method outperforms the baseline approaches. Furthermore, an ablation study reveals that incorporating additional sensory inputs, such as force or proprioception, enhances sample efficiency and performance, although this improvement is task-dependent. Finally, they also show that even when visual input quality is poor, the force input can compensate for it.

In \cite{nguyen2023equivariant}, the authors extend the equivariance to partially observable Markov decision process (POMDP), denoted as $\mathcal{P}_G=(S,A,P,R,\Omega,O,b_0)$. Here, $S,A,P,$ and $R$ represent the state space, action space, transition probability, and reward function, analogous to those in $\mathcal{M}_G$. The additional components $\Omega$ (observation space), $O$ (stochastic observation function), and $b_0$ (initial belief) incorporate group-invariant conditions. These include $O(\rho_a(g)a, \rho_s(g)s',\rho_o(g)o)$ for the observation function and $b_0(\rho_s(g)s)=b_0(s)$ for the initial belief. The history $h_t=(o_0,a_0,...,a_{t-1},o_t)$ is shown to remain invariant under group action $g\in G$, and the optimal value function $V^*(h)$ and policy $\pi^*$ also exhibit symmetric properties. Using an equivariant actor-critic actor-critic framework, the authors demonstrate superior performance over non-equivariant methods in simulations and validate their approach by successfully transferring policies to real hardware in a zero-shot manner.

Equivariant networks have also been applied to offline reinforcement learning \cite{tangri2024equivariant}. This work leverages equivariant networks within specific methods like Conservative Q-Learning \cite{kumar2020conservative} and Implicit Q-Learning \cite{kostrikov2021offline} and tackles the challenge of outperforming the behavior policy that generated the offline datasets. They show their approach's enhanced sample efficiency and performance through simulations involving robot manipulation tasks.


==> Old_2024_1130/Section5_GeometricImpedanceControl.tex <==
We introduce geometric impedance control (GIC) \cite{seo2023geometric, seo2024comparison} here and show that it serves as a $\SE$ group equivariant control law. 
% {\color{red} SML: "In this note": What is it referring to? "Furthermore": no preceding argument} In this note, 
Moreover, we also show that under the framework of variable impedance control, GIC can be considered as an $\SE$ group equivariant force-based policy. The main contents of this section are already published in \cite{seo2024comparison}. Readers can consider this section as the more detailed explanation version of \cite{seo2024comparison}.

\paragraph*{Necessity of geometric formulation}
As can be seen in \eqref{eq:manipulator_dynamics}, the underlying coordinate of the manipulator is described in the joint space. However, as suggested in \cite{khatib1987unified}, the manipulator will execute a task on the workspace, i.e., end-effector space. Therefore, the task can be described more intuitively in the end-effector space. The pose of the end-effector can be calculated via forward kinematics (Sec~\ref{sec:Prelim}), and thereby, it can be well described by utilizing a group structure of $\SE$. 

Conventional impedance control designs do not consider the full geometric structure of $\SE$. For instance, the papers from the early stage of robot control \cite{hogan1985impedance, khatib1987unified} could be considered. In \cite{hogan1985impedance}, the end-effector coordinate $x \in \mathbb{R}^6$ is just utilized without explicitly mentioning its definition. To correctly define the rotational errors, many representations are studied in \cite{caccavale1999six}, including Euler-angle representation, axis-angle representation of $\SO$, and quaternion representation. Similarly, in \cite{khatib1987unified}, the translational and rotational parts of the $x$ vector were separately considered. 

In this regard, by incorporating a full geometric structure of $\SE$ into the control design, one can expect a further increase in performance. 
% {\color{red} SML: Lowercase for "Section"; Suggestions: "Additionally, as we will explain later in this section"; comma misplacement ("equivariant force, velocity-based policy structures"); suggestion: "can be obtained" -> "will be clarified"} 
Moreover, the intuition for the equivariant force or velocity-based policy will be clarified later in this section. 
% Moreover, as we are going to describe in the later part of this Section, the intuition for the equivariant force, velocity-based policy structures can be obtained. 

\subsection{Manipulator Dynamics}
\subsubsection{Manipulator Dynamics in joint space}
The manipulator dynamics in the joint space is written as follows.
\begin{equation} \label{eq:manipulator_dynamics}
    M(q)\ddot{q} + C(q,\dot{q})\dot{q} + G(q) = \tau + \tau_e,
\end{equation}
where $q\in\mathbb{R}^n$ is a joint coordinate in position, $\dot{q} \in \mathbb{R}^n$ is joint velocity, $\ddot{q}\in\mathbb{R}^n$ is joint acceleration, $M(q)\in\mathbb{R}^{n\times n}$ is inertia matrix, $C(q,\dot{q})\in\mathbb{R}^{n\times n}$ is Coriolis matrix, $G(q) \in \mathbb{R}^n$ is gravity force vector in joint space, $\tau \in \mathbb{R}^n$ is joint torque as a control input, and $\tau_e \in \mathbb{R}^n$ is external disturbance acting in the form of joint torque. 

\subsubsection{Manipulator Dynamics in Workspace on $\SE$}
As the task that the manipulator performs is done by the end-effector, it is often preferable to define the task in the workspace, not in the joint space. Thus, we are now interested in the framework that regards the operational space as $\SE$. 
Employing the operational space formula from \cite{khatib1987unified}, the manipulator dynamics using the body-frame velocity $V^b$ is given by:
\begin{align} \label{eq:robot_dynamics_eef}
    &\tilde{M}(q)\dot{V}^b + \tilde{C}(q,\dot{q})V^b + \tilde{G}(q) = \tilde{T} + \tilde{T}_e, \text{ where}\\
   & \tilde{M}(q)= J_b(q)^{-T} M(q) J_b(q)^{-1}, \nonumber\\
    &\tilde{C}(q,\dot{q})=J_b(q)^{-T}(C(q,\dot{q}) \!-\! M(q) J_b(q)^{-1}\dot{J})J_b(q)^{-1}, \nonumber\\
   & \tilde{G}(q)= J_b(q)^{-T} G(q),\; \tilde{T}= J_b(q)^{-T} T,\; \tilde{T}_e= J_b(q)^{-T} T_e.\nonumber,
\end{align}
where $J_b$ is a body-frame Jacobian matrix which relates body velocity and joint velocity by $V^b = J_b \dot{q}$. See \cite{seo2023geometric, seo2024comparison} for more details. 

\subsection{Error Functions: Distance-like Metrics on $\SE$}
Lyapunov stability theory provides a foundation for describing the stability property of the given autonomous or control system. 
The key idea behind the Lyapunov stability theory is to represent the dynamics of a high-dimensional nonlinear ordinary differential equation (ODE) without solving it. 
% {\color{red} SML: A scalar Lyapunov function is defined using the state of the ODE as input, and its convergence properties are analyzed to describe the behavior of the original system.} 
Instead, a scalar Lyapunov function is defined using the state of the ODE as input, and its convergence properties are analyzed to describe the behavior of the original system.
% the scalar function (Lyapunov function), which gets the state of the ODE as input, is defined, and the convergence property of the Lyapunov function is analyzed to describe the property of the original system. 
% {\color{red} SML: In mechanical control systems, the total mechanical energy (the sum of potential and kinetic energy) is traditionally used as a Lyapunov candidate \cite{koditschek1989application}} 
In mechanical control systems, the total mechanical energy, which is defined as the sum of potential and kinetic energy, is traditionally used as a Lyapunov candidate \cite{koditschek1989application}
% For the mechanical control system, total mechanical energy (potential energy + kinetic energy) is traditionally considered as the Lyapunov candidate \cite{koditschek1989application}. 
Here, the kinetic energy is composed of the velocity parts of the states, while the potential energy is composed of the position parts. It is quite straightforward to find out that the potential energy is closely related to the distance of two points, as the potential function and the distance metrics are both defined from the \emph{difference} of two points. 

Defining the difference between two points in Euclidean space is straightforward. Consider $x_1, x_2 \in \mathbb{R}^n$ in Euclidean space. Then, a \emph{vector} to describe the difference between two points can be considered as $v = x_1 - x_2$, and the Euclidean norm can be utilized to describe the distance, i.e., $d = \|v\|_2$.

On the other hand, the difference between the two points on the manifold (Lie group) is more subtle. Before we introduce the notion of difference in $\SE$, one must first note that the unit of the two elements $\SO$, $\mathbb{R}^3$ are not the same. 
% {\color{red} SML: "we have no choice" seems strong and informal} 
As the unit of $\SO$ and $\mathbb{R}^3$, does not match, we are urged to use the notion of the \emph{error function}, $\Psi: \SE \times \SE \to \mathbb{R}$, instead of using the terminology of distance. For this reason, we will now use the word ``\textbf{error function}'' to describe the scalar variable between two elements on $\SE$ that represents the ``distance'' between two points.
There are two major perspectives to represent such error function on $\SE$ \cite{seo2024comparison}: 
% {\color{red} SML: change period to colon and add a period at the end of 2. Colon seems necessary to relate the claim with the two perspectives.}

% {\color{red} Choi: We should make either $\SE$$ or $\SE$ to be consistent.}

\begin{enumerate}
    \item Using the fact that $\SE$ is a General Linear (matrix) group
    \item Using the property of Lie algebra 
\end{enumerate}
Two different perspectives of error function lead to different perspectives of potential functions, resulting in different control laws. The first aspect leads to the definition of distance and potential function on the Lie group \cite{seo2023geometric, bullo1999tracking, lee2010geometric}. On the other hand, the Lie algebra-based potential function can be constructed \cite{teng2022lie, bullo1995proportional}. 
We note that the error function in this paper means the squared distance-like metric.

\subsubsection{Configuration Error}
Before we define the error function, we need to first have a notation to define the difference between two configurations. The transformation matrix between the desired $g_d = (p_d,R_d)$ and current configuration $g = (p, R)$ is defined as
\[
    g_{de} = g_d^{-1}g.
\]
We will call $g_{de}$ as the \emph{configuration error}, and this will be utilized to define the error in the configuration in many of the geometric control literature, e.g., \cite{seo2023geometric, bullo1995proportional, lee2010geometric,bullo1999tracking,teng2022lie,lee2012exponential}.

\subsubsection{Error Function from Matrix Group Perspective}
One can just focus on the fact that a homogeneous matrix representation is nothing but a matrix. This concept was first proposed in \cite{koditschek1989application}, further developed in \cite{bullo1999tracking}, revisited in \cite{lee2010geometric}, and widely utilized thereafter, especially on $\SO$, i.e., UAV field. In $\SO$, a error function on this perspective $\Psi(R,R_d)$ is given by
\[
    \Psi(R,R_d) = \text{tr}(I - R_d^T R)
\]
However, what is overlooked from the error function $\Psi(R,R_d)$ is that it originates from the Frobenius norm. In the $\SO$ case, the following equality holds \cite{huynh2009metrics}:
\begin{equation*}
    \Psi(R,R_d) = \text{tr}(I - R_d^T R) = \dfrac{1}{2}\text{tr} \left((I - R_d^T R)^T(I - R_d^T R)\right) 
\end{equation*}
The definition of the Frobenius norm, i.e., $\|A\|_F^2 = \text{tr}(A^T A)$, can be used to derive
\begin{equation} \label{eq:Frob_norm_SO3}
    \Psi(R,R_d) = \dfrac{1}{2}\|I - R_d^T R\|_F^2.
\end{equation}

Let us chew on \eqref{eq:Frob_norm_SO3}. When $R = R_d$, then $R_d^TR = I$; $\Psi(R,R_d) = \|0\|_F = 0$. Thus, what it means is that we first see the difference between two points in $\SO$, compare the difference rotation matrix with the identity matrix, and quantify its discrepancy from the identity as the Frobenius norm. Recalling that the transpose operator in $\SO$ is the same as the inverse operator, one could extend \eqref{eq:Frob_norm_SO3} defined on $\SO$ to the $\SE$ as the following formula, which is also based on the Frobenius norm. 
\begin{align} \label{eq:Frob_norm_SE3}
        &\Psi_1(g,g_d) = \dfrac{1}{2}\|I - g_d^T g\|_F^2 \\
        &= \tfrac{1}{2} \tr\left((I - g_d^{-1}g)^T(I - g_d^{-1}g)^T \right) = \tfrac{1}{2} \tr (X^T X) \nonumber,
\end{align}
with $X$ defined as
\begin{equation*}
    X = X(g,g_d) = \begin{bmatrix}
    (I - R_d^TR) & -R_d^T(p - p_d) \\
    0 & 0 
    \end{bmatrix}. \nonumber
\end{equation*}
By further unraveling the equation, one can show that
\begin{equation} \label{eq:error_function_SE3}
    \Psi_1(g,g_d) = \tr(I - R_d^TR) + \tfrac{1}{2}(p - p_d)^T(p - p_d)
\end{equation}
Therefore, we can see that the error function in $\SE$ is composed of $\SO$ and $\mathbb{R}^3$ similar to the first perspective. 

\subsubsection{Error Function from Lie Algebra Perspective}
The central intuition here is that the Lie algebra can be considered as the local chart of the $\SE$ manifold. Note that Lie algebra is defined as the element on the tangent space of the identity. Thus, Lie algebra is vector space but not (necessarily) attached to the tangent space of the current configuration.  As we can see from the Euclidean space example, the first intuitive way to define distance is by using a vector.
In \cite{teng2022lie}, the Lyapunov candidate was proposed using this concept. The implication is that the proposed Lyapunov candidate function is a potential function (for the first-order system case), and if we remove the \emph{weights} in the potential, then it can be considered as the distance metric (squared). The vector representation $\xi_{de} \in \mathbb{R}^6$ of a configuration error is defined as
\begin{equation}
    \xi_{de} = \log{(g_{de})}^\vee = 
    \begin{bmatrix}
        \hat{\psi}_{de} & b_{de} \\
        0 & 0
    \end{bmatrix}^\vee = \begin{bmatrix}
        b_{de} \\ \psi_{de}
    \end{bmatrix}
\end{equation}
where (See pp. 413-414 of \cite{murray1994mathematical})
\begin{align*}
    &\hat{\psi}_{de} = \log(R_d^TR), \quad b_{de} = A^{-1}(\psi_{de}) R_d^T(p - p_d)\\
    &A^{\text{-}1}(\psi) \!=\! I \!-\! \dfrac{1}{2}\hat{\psi} + \dfrac{2\sin\|\psi\| - \|\psi\|(1 + \cos\|\psi\|)}{2 \|\psi\|^2 \sin \|\psi\|} \hat{\psi}^2,
\end{align*}
when $\psi \neq 0$.
Note that the logarithm of the matrix is not unique \cite{Matrix_log_wiki}, and there are many alternative definitions, e.g., \cite{seo2024comparison, bullo1995proportional}
\begin{align*}
    A^{-1}(\psi) &= I - \dfrac{1}{2}\hat{\psi} + \left(1 - \alpha(\|\psi\|)\right) \dfrac{\hat{\psi}^2}{\|\psi\|^2},\\ &\text{with} \; \alpha(y) = (y/2)\cot{(y/2)}.
\end{align*}

As mentioned in \cite{bullo1995proportional}, the inner product on $\so$ is well defined. Moreover, it also has good properties of positive definiteness and bi-invariance. The inner product of two elements $\hat{\psi}_1, \hat{\psi}_2 \in \so$ can be defined using the Killing form, a bilinear operator defined by $\langle \cdot, \cdot \rangle _K: \so \times \so \to \mathbb{R}$, as \cite{park1995distance}
\begin{equation*}
    \begin{split}
        \langle\hat{\psi}_1, \hat{\psi}_2\rangle_{\so} &\triangleq -\tfrac{1}{4} \langle\hat{\psi}_1, \hat{\psi}_2\rangle_K, \;
        \langle\hat{\psi}_1, \hat{\psi}_2\rangle_K \triangleq \tr( \ad_{\psi_1} \ad_{\psi_2} ).
    \end{split}    
\end{equation*}
where $\ad$ is an adjoint (small adjoint) operator, where if $\psi \in \so$, $\ad_{\psi}= \hat{\psi}$.

On the other hand, there is no symmetric bilinear form on $\se$ that is both positive definite and bi-invariant \cite{bullo1995proportional, park1995distance}.
However, one can still define a left-invariant (or right-invariant) inner product on $\se$ by exploiting the fact that $\se$ is isomorphic to $\mathbb{R}^6$. We will denote the inner product by $\langle \hat{\xi}_1, \hat{\xi}_2\rangle_{(P,I)}$, as follows \cite{park1995distance, teng2022lie, vzefran1996choice, belta2002euclidean}:
\begin{equation}
\label{eq:inner_product_$\SE$}
    \langle \hat{\xi}_1, \hat{\xi}_2 \rangle_{(P,I)} = \xi_1^T P \xi_2
\end{equation}
where $\hat{\xi}_1, \hat{\xi}_2 \in \se$, and $P \in \mathbb{R}^{6\times 6}$ is symmetric positive definite matrix. 
The subscript $P$ in \eqref{eq:inner_product_$\SE$} denotes that the inner product is equipped with the Riemannian metric $P$, while the subscript $I$ means that the Lie algebra $\se$ is defined on the tangent space at the identity element of $\SE$. The introduction of these subscriptions is to fill the discrepancies between the definition of the inner product of Lie algebra and Riemannian metric; the inner product of the Lie algebra is defined literally on the Lie algebra, but the Riemannian metric is defined on the tangent space attached to each point on the manifold. 

An important factor to note is that the tangent vector on $g \in \SE$ is not the same as the Lie algebra $\se$. This can be revealed by observing $\dot{g}$, with $g = (p,R)$ and $V = (v,\hat{w})$:
\begin{equation*}
    \dot{g} = g \hat{V}^b = \begin{bmatrix}
        R & p \\
        0 & 1 
    \end{bmatrix} \begin{bmatrix}
        \hat{w} & v \\ 
        0 & 1
    \end{bmatrix} = \begin{bmatrix}
        R\hat{w} & Rv \\ 
        0 & 1
    \end{bmatrix},
\end{equation*}
but as $R\hat{w} \notin \so$, i.e., not skew-symmetric, we can conclude that $\dot{g} \notin \se$, but $\dot{g} \in T_g\SE$.


With this definition, we can define the Riemannian metric on $\SE$ on the point $g \in G$,
using the inner product on $\se$ $\langle \cdot, \cdot \rangle_{(P,g)} : T_gG\times T_gG \to \mathbb{R}$, as follows. Consider two tangent \emph{vectors} on the tangent space at point g, $\delta g_i \in T_gG$, such that $\delta g_i = g \hat{\xi}_i$ with $\hat{\xi}_i = (b_i, \hat{\psi}_i)$ for $i = \{1,2\}$.
The Riemannian metric is then defined as \cite{park1995distance, vzefran1996choice, belta2002euclidean}
\begin{equation} \label{eq:Riemannian_metric}
    \langle \delta g_1, \delta g_2 \rangle_{(P,g)} \!=\! \langle g^{-1} \delta g_1, g^{-1} \delta g_2 \rangle_{(P,I)} = \langle \hat{\xi}_1, \hat{\xi}_2 \rangle_{(P,I)}
\end{equation}
The Riemannian metric \eqref{eq:Riemannian_metric} herein is often referred to as a left-invariant Riemannian metric because $g^{-1} \delta g_i = \hat{\xi}_i$ is left invariant, i.e., for any arbitrary left transformation matrix $g_l$, $(g_l g)^{-1} (g_l g) \hat{\xi}_i = \hat{\xi}_i$. 

Finally, we can define an error function on $\SE$ from Lie-algebra perspective by letting $P = \tfrac{1}{2}I_{6\times6}$ as follows:
\begin{equation} \label{eq:error_function_SE3_algebra}
    \Psi_2(g,g_d) = \langle g_{de}\hat{\xi}_{de}, g_{de}\hat{\xi}_{de} \rangle_{\left(0.5I, g_{de}\right)} = \tfrac{1}{2} \|\psi_{de}\|^2 + \tfrac{1}{2}\|b_{de}\|^2
\end{equation}
where $\hat{\xi}_{de} = \log(g_{de}) = (b_{de}, \hat{\psi}_{de})$. 
\eqref{eq:error_function_SE3_algebra} can also be obtained as presented in \cite{belta2002euclidean} and \cite{liu2013finite}, by considering $\SE$ as a general affine group. 

\subsection{Error Vectors on $\SE$}
\subsubsection{Positional Error Vectors on $\SE$}
\paragraph*{Geometrically Consistent Error Vector (GCEV)} GCEV was proposed in \cite{seo2023geometric} and serves as a positional error vector in $\SE$. Note that this error vector formulation is derived from the Lie group-based error function. The error vector derivation on $\SO$ was first proposed in \cite{lee2010geometric}. We first perturb a configuration $g \in \SE$ with a right translation in the direction of an arbitrary vector $\eta$, as was done in \cite{lee2010geometric} for $\SO$.
\begin{equation*}\begin{aligned}
    g_{\hat{\eta}}= g e^{\hat{\eta}\epsilon}\!, \quad \eta=\begin{bmatrix}\eta_1\\ \eta_2\end{bmatrix}\!\in\!\mathbb{R}^6 \implies \hat{\eta}\!\in\! \SE, \;\epsilon\!\in\!\mathbb{R},
\end{aligned}\end{equation*}
where $\eta_1, \eta_2\!\in\!\mathbb{R}^3$ refer to translational and rotational components, respectively. The perturbed configuration matrix $\delta g$ can be found by
\begin{equation*}
    \begin{split}
        \delta g &= \left.\dfrac{d}{d\epsilon}(g e^{\hat{\eta}\epsilon})\right|_{\epsilon=0} = \left. g \hat{\eta}  e^{\hat{\eta}\epsilon}\right|_{\epsilon = 0} = g \hat{\eta} \in T_g \SE, \\
        &\implies \begin{bmatrix}
        \delta R & \delta p \\
        0 & 0 
        \end{bmatrix}  = \begin{bmatrix}
        R\hat{\eta}_2 & R \eta_1 \\ 0 & 0 
        \end{bmatrix}.
    \end{split}    
\end{equation*}
The perturbed error function $\delta \Psi(g,g_d)$ can be obtained and evaluated by
\begin{equation*} \label{eq:perturbation_of_error_metric}
    \begin{split}
    \delta \Psi(g,g_d)&=\dfrac{1}{2}\tr\begin{bmatrix}\!
    -\delta R^T R_d-R_d^T \delta R & \ast \nonumber
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(p-p_d)^T \delta p
    \end{bmatrix} \nonumber \\
    &=\!\dfrac{1}{2}\tr\begin{bmatrix}
    -\hat{\eta}_2^T R^TR_d-R_d^T R \hat{\eta}_2 & \ast
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(p-p_d)^T R \eta_1 
    \end{bmatrix}\nonumber \\
    &= -\tr(R_d^T R \hat{\eta}_2) + (p-p_d)^T R \eta_1 \nonumber \\
    &= (R_d^T R - R^T R_d)^\vee \cdot \eta_2 + (p - p_d)^T R \eta_1,
    \end{split}
\end{equation*}
where $\cdot$ is an inner product between two vectors. We can describe the perturbation of the error function in $\SE$ $\delta \Psi$ using the Lie derivative from \eqref{eq:lie_deriv_group}:
\begin{equation*}
    \delta \Psi = \Lie_{\hat{\eta}} \Psi(g,g_d) = \dfrac{d}{d\varepsilon} \left. \Psi(g e^{\hat{\eta}\varepsilon}, g_d)\right|_{\varepsilon = 0}.
\end{equation*}
Note also that we only evaluate the Lie derivative on the point $g$, not the point $g_d$.

We now define the \emph{position} error vector or Geometrically Consistent Error Vector (GCEV) $\eg$
as
\begin{equation}\begin{aligned}\label{eq:eg}
    \eg = \begin{bmatrix}
    e_p \\ e_R
    \end{bmatrix} = \begin{bmatrix}
    R^T(p - p_d) \\
    (R_d^T R - R^T R_d)^\vee 
    \end{bmatrix} \in \mathbb{R}^6,
\end{aligned}\end{equation}
so that $\delta \Psi(g,g_d) = \eg ^T \eta$ and
\begin{equation*}\begin{aligned}
    \hat{e}_g = \begin{bmatrix}
    R_d^T R - R^T R_d & R^T (p - p_d) \\
    0 & 0 
    \end{bmatrix} \in \se.
\end{aligned}\end{equation*}

\paragraph*{Lie algebra-based Error Vector}
Similar to the way that the GCEV is derived from its Lie group-based error function, we can also derive the positional error vector from the Lie algebra-based error function. To put a conclusion, such a positional error vector is a log map of the configuration error $g_{de}$, \cite{teng2022lie}.

\subsubsection{Velocity Error Vector}
Velocity error vector should be defined properly on the $\SE$ manifold, as the two tangent vectors $\dot{g} = g \hat{V}^b$ and $\dot{g}_d = g_d \hat{V}^b_d$ do not lie on the same tangent spaces. Specifically, for the Frobenius-norm-based error function, the desired velocity vector $V_d^b$ is translated using the following formula (See Ch 2.4 of \cite{murray1994mathematical} for the details. See also \cite{seo2023geometric, lee2010geometric}): 
\begin{equation*}\begin{aligned}
    \hat{V}_d^* = g_{ed} \hat{V}_d^b g_{ed}^{-1}, \text{ where } g_{ed} = g^{-1}g_d.
\end{aligned}\end{equation*}
Then, it is straightforward to have in the vector form:
\begin{equation}\begin{aligned}\label{eq:Ad_velo}
    V_d^* = \text{Ad}_{g_{ed}}V_d^b, \text{ with } \text{Ad}_{g_{ed}} = \begin{bmatrix}
   R_{ed} & \hat{p}_{ed} R_{ed} \\ 0 & R_{ed}
    \end{bmatrix},
\end{aligned}\end{equation}
where $\text{Ad}_{g_{ed}}: \mathbb{R}^6 \to \mathbb{R}^6$ is an Adjoint map, $R_{ed} = R^T R_d$, and $p_{ed} =-R^T(p - p_d)$. 

Based on this, we define the \emph{velocity} error vector $\ev$ as 
\begin{equation}\begin{aligned} \label{eq:ev}
    \ev = \underbrace{\begin{bmatrix}
    v^b \\ w^b \end{bmatrix}}_{V^b} - \underbrace{\begin{bmatrix}
     R^TR_d v_d + R^T R_d \hat{\omega}_d R_d^T (p - p_d)\\
     R^T R_d \omega_d \end{bmatrix}}_{V_d^*} = \begin{bmatrix}
    e_v \\ e_\Omega \end{bmatrix}.
\end{aligned}\end{equation}

This procedure to calculate velocity error vector originates from the fact that the two tangent vectors $\dot{g} \in T_g\SE$ and $\dot{g}_d \in T_{g_d}\SE$ cannot be directly compared since they are defined on the different points on the manifold. In \cite{lee2010geometric}, $\dot{g}_d$ is first translated via right multiplication $g_d^{-1}g$. This right multiplication can be interpreted in the following procedures, with $\dot{g}_d = g_d \hat{V}_d^b$:
\begin{enumerate}
    \item Apply left transformation on tangent space $dL_{g_d^{-1}}(\dot{g}_d)$by $g_d^{-1}\dot{g}_d = \hat{V}_d$.
    \item Apply coordinate transformation on $\se$ via $\hat{V}_d^{*} = g_{ed} \hat{V}_d^b g_{ed}^{-1}$, with $g_{ed} = g^{-1}g_d$
    \item Translate to the point $g$ by $dL_g(\hat{V}_d^*) = g \hat{V}_d^{*}$
    \item Compare two tangent vectors $g \hat{V}^b - g \hat{V}_d^{*} = g \hat{e}_V$
\end{enumerate}

The other perspective is to interpret the configuration error $g_{de}$ as an element on the manifold $\SE$, and the time-derivative of $g_{de} = g_d^{-1}g$ is handled as follows \cite{teng2022lie}:
\begin{align*}
    \dfrac{d}{dt}(g_d^{-1}g) &=  g_d^{-1}\dot{g} + \dot{g}_d^{-1} g = g_d^{-1}\dot{g} -  g_d^{-1}\dot{g}_d g_d^{-1} g \nonumber \\
    &= g_d^{-1}g \hat{V}^b - g_d^{-1}g_d\hat{V}_d^b g_d^{-1}g \\
    &= g_d^{-1}g \left(\hat{V}^b - (g_d^{-1}g)^{-1}\hat{V}_d^b (g_d^{-1}g)\right) \triangleq g_d^{-1}g (\hat{e}_V) \nonumber\\
    \implies \dot{g}_{de} &= g_{de} \hat{e}_V \in T_{g_{de}}\SE\nonumber
\end{align*}
Notice that $g_{de} = g_d^{-1}g$, $g_{de}^{-1} = g_{ed}$, and $(g \hat{\xi} g^{-1})^\vee = \Ad_g\xi$, for $g \in \SE$ and $\xi \in \se$. Also, $\tfrac{d}{dt}M^{-1} = M^{-1} \tfrac{dM}{dt} M^{-1}$. To conclude, the tangent vector is directly derived on the tangent space $\dot{g}_{de} \in T_{g_{de}}\SE$, and it turns out that both approaches lead to the same velocity error vector.

Therefore, we conclude that although both approaches have different rationales, they share the same structure of velocity error vector, which leads to the same Kinetic energy function and the same impedance control law. We refer to the description from \cite{seo2024comparison} for the details of the velocity error vector.

\subsection{Energy Functions on $\SE$}
We consider two energy functions for our control design: potential energy function and kinetic energy function.

\subsubsection{Potential Energy Function} 
We interpret the potential energy function as a weighted distance metric. This concept is motivated by the potential energy of the spring in the Euclidean space. Consider a linear spring with one end attached to the origin $x_0 = 0 \in \mathbb{R}^3$ and the other end attached to $x \in \mathbb{R}^3$. Then, the potential energy stored in the spring can be written by 
\begin{equation*}
    P = \frac{1}{2} x^T K x = \frac{1}{2}\|x\|_K^2
\end{equation*}
where $K \in \mathbb{R}^{3\times 3}$ is a symmetric positive definite stiffness matrix, and the potential energy can be interpreted as the weighted 2-norm or weighted squared Euclidean distance. Recalling that we have derived the error metric in $$\SE$$ in two different ways, we will define the potential functions on $$\SE$$ accordingly. 

\paragraph*{Potential Energy Function from Matrix Group Perspective} We weight the distance metric in \eqref{eq:Frob_norm_SE3} by first introducing a weighted matrix $X_K$ given by:
\begin{equation}
    X_K = \begin{bmatrix}
        \sqrt{K_R}(I - R_d^TR) & -\sqrt{K_p}R_d^T(p - p_d)\\
        0 & 0
    \end{bmatrix}
\end{equation}
where $K_p, K_R \in \mathbb{R}^{3\times3}$ are symmetric positive definite stiffness matrices for translational and rotational parts, respectively, and the square root of the matrix can be defined from the standard singular value decomposition. Note that the square root of the matrix is utilized to recover the original matrix in the potential energy form.
Then, the potential function $P_1(g,g_d)$ from Lie group $\SE$ perspective is defined in the following way:
\begin{equation} \label{eq:potential_lie_group}
    \begin{split}
        & P_1(g,g_d) = \tfrac{1}{2}\tr(X_K^T X_K) \\
        &\;\;= \tr(K_R(I - R_d^T R)) + \tfrac{1}{2}(p - p_d)^T R_d K_p R_d^T (p - p_d) 
    \end{split}
\end{equation}

\paragraph*{Potential Energy Function from Lie algebra perspective}
Given the inner product on $\se$ and the error function defined previously, the potential function from the Lie algebra perspective can be given as \cite{teng2022lie, seo2024comparison}:
\begin{equation} \label{eq:potential_lie_algebra}
    P_2(g,g_d) = \langle \hat{\xi}_{de}, \hat{\xi}_{de}\rangle_{(0.5K_\xi, I)} = \tfrac{1}{2}\xi_{de}^T K_{\xi} \xi_{de},
\end{equation}
where $P=\tfrac{1}{2}K_{\xi}$ and $K_\xi \in \mathbb{R}^{6\times6}$ is symmetric positive definite. Henceforth, we interpret $K_\xi$ as a stiffness matrix. We emphasize that $P_1(g,g_d)$ and $P_2(g,g_d)$ are left-invariant, positive definite, and quadratic. Left-invariance of these potential functions will be utilized later in this Section to prove the $\SE$-Equivariance. 

\subsubsection{Kinetic Energy on $\SE$}
The kinetic energy function on $\SE$ for the impedance control design can be formulated by using a velocity error vector $\ev$ and inertia matrix in the following form:
\begin{equation} \label{eq:kinetic_energy}
    K(t,q,\dot{q}) = \tfrac{1}{2}e_V^T \tilde{M} e_V,
\end{equation}

\subsection{Geometric Impedance Control}
We now introduce a geometric impedance control law (GIC) based on the potential and kinetic energy functions. The main idea behind the GIC is that the total mechanical energy function (potential + kinetic energy) should be dissipated over time. 

\subsubsection{Impedance Control as a Dissipative Control Law}
The total mechanical energy function, our Lyapunov function is defined as
\begin{equation} \label{eq:lyapunov}
    V_i(t,q,\dot{q}) = K(t,q,\dot{q}) + P_i(t,q), \quad i \in \{1,2\}
\end{equation}
where $K$ and $P_i$ are the kinetic and potential energy components of the Lyapunov function. Note that $P_1$ is given in \eqref{eq:potential_lie_group} and $P_2$ is in \eqref{eq:potential_lie_algebra}. The desired property of the impedance control to be dissipative control law \cite{kronander2016stability} is defined as
\begin{equation} \label{eq:dissipative}
    \dot{V}_i = -e_V^T K_d e_V
\end{equation}
where $K_d \in \mathbb{R}^6$ is symmetric positive definite damping matrix. 
To satisfy \eqref{eq:dissipative}, the impedance control laws for each potential function are
\begin{equation} \label{eq:control_law}
        \tilde{T}_i \!=\! \tilde{M}\dot{V}^*_{d} \!+\! \tilde{C}{V}^*_{d} + \tilde{G} \!-\! f_{_{G,i}} \!-\! K_d e_V, \;\text{for}\; i \in \{1,2\}
\end{equation}
where $f_{_{G,i}} \in \mathbb{R}^6$, $\hat{f}_{_{G,i}}\in \se^*$, are given respectively by
\begin{equation}
    \begin{split}
        f_{_{G,1}} &= \begin{bmatrix}
        f_p \\ f_R
        \end{bmatrix} = \begin{bmatrix}
            R^T R_d K_p R_d^T (p - p_d)\\
            (K_R R_d^T R - R^T R_d K_R)^\vee
        \end{bmatrix} \\ 
        f_{_{G,2}} &= K_\xi \xi_{de}.
    \end{split}    
\end{equation}
The derivation process of $f_{_{G,1}}$ is shown in \cite{seo2023geometric} and $f_{_{G,2}}$ in \cite{seo2024comparison}.
We can show that both control laws satisfy almost global asymptotic stability. We refer to \cite{seo2023geometric, seo2024comparison} for the details of such properties.

\subsubsection{Geometric Impedance Control is $\SE$-Equivariant Control}
One of the crucial advantages of the GICs is that the control law is $\SE$ equivariant if it is described on the spatial frame. In \cite{seo2023contact}, the GIC law with learning gain scheduling policy is proved to be equivariant if the gain scheduling policy is left-invariant. Without any gain scheduling law, i.e., fixed impedance gains, similar analysis is also possible. Take $f_{_{G,1}} : \SE \times \SE \to se^*(3)$ for example, the left-invariance of $f_{_{G,1}}(g,g_d)$ can be shown as follows:
\begin{align}
    &f_{_{G,1}}(g_lg,g_lg_d) \nonumber\\&= \begin{bmatrix}
        (R_l R)^T R_l R_d K_p (R_l R_d)^T (R_l p + p_l - R_l p_d - p_l)\\
        (K_R(R_l R_d)^TR_lR - (R_l R)^T R_l R_d K_R)^\vee
    \end{bmatrix} \nonumber \\
    &= \begin{bmatrix}
        R^T R_d K_p R_d(p - p_d)\\
        (K_R R_d R - R^T R_d K_R)^\vee
    \end{bmatrix} = f_{_{G,1}}(g,g_d),
\end{align}
Note that the elastic force $f_{_{G,1}}$ is described on the body-frame coordinate. Similarly for $f_{_{G,2}}$,
\begin{equation}
    \begin{split}
        f_{_{G,2}}(g_lg, g_lg_d) &= K_\xi \log{((g_l g_d)^{-1} (g_l g_e))} \\
    &= K_{\xi} \log{(g_d^{-1} g_e)} = K_{\xi}\xi_{de}.
    \end{split}
\end{equation}

Then, the feedback terms of the GIC law are $\SE$ equivariant if they are described in the spatial frame, as can be shown from Proposition 2 of \cite{seo2023contact}. We will skip the proof in this note, as it has already been proved in the paper. 
However, it is worth mentioning that a generalized recipe for the velocity and force-based policy to be $\SE$-equivariant can be obtained. According to \cite{seo2023contact}, such a general recipe is given by:
\begin{enumerate}
    \item The policy is left-invariant.
    \item The policy is described on the body-frame coordinate.
\end{enumerate}
Although in \cite{seo2023contact} only mentioned velocity and force-based policy, it can be trivially extended to displacement $\Delta g$ within a sampling period. 

==> Old_2024_1130/Section6_FutureWorks.tex <==
\subsection{Towards Vision-to-Force SE(3)-Equivariance}
Current vision-based approaches are formulated on the philosophical foundation that every manipulation can be considered as the sequence of pick-and-places \cite{shridhar2022cliport}. Although this argument well describes the manipulation tasks for simple tabletop manipulation, many real-life tasks require force interaction and compliance. For example, if a robot wants to twist off a bottle, the simple vision-based model cannot obtain the necessary accuracy and handle delicate force interaction. Many examples of assembly tasks also require force interaction, such as bolt-nut assembly or brute-force tight-fit assembly. Forces, or wrenches, can be interpreted as two type-1 vectors steered by the large adjoint map on the dual space of $\SE$ manifold. The handling of such wrenches is implied in the diffusion process in Diff-EDF \cite{ryu2024diffusion} but for the twists rather than wrenches. Therefore, we hypothesize that incorporating equivariance can significantly enhance the sample efficiency of the learning problem for the manipulation tasks associated with force interaction. The GIC proposed in \cite{seo2023geometric, seo2024comparison} and its application to assembly tasks \cite{seo2023contact} can be considered as a good baseline for such force-related equivariant assembly method.

\subsection{Symmetry Breaking in Robotics and  Systems}
The robot's end-effector has an SE(3) manifold structure with symmetry properties that can be exploited. However, the symmetry in the end-effector space of the manipulator only holds when there is enough manipulability. For instance, if the manipulator approaches the singular configuration, the dynamics cannot be well-described by \eqref{eq:robot_dynamics_eef}. Therefore, the kinematic constraint is the main reason for symmetry breaking.
From the control perspective, such symmetry-breaking scenarios can be easily observed when there are constraints in the control system, e.g., constraints on the input. 

% \JC{Updated - symmetry breaking in observation space due to the camera angle and occlusions, and symmetry breaking in RL: (Good)}
Symmetry breaking can arise from imperfections in the observation space, such as images captured from a 3D scene using a camera. Equivariant networks, which model rotational symmetry from 2D inputs, typically rely on a perfect top-down view to fully exploit this symmetry. However, practical deviations, such as tilted camera angles, disrupt the assumed symmetry, resulting in suboptimal performance compared to ideal settings. While equivariant networks outperform unstructured networks under these conditions \cite{wang2022surprising}, they remain sensitive to such imperfections. Additionally, occlusions in the observation space can further disrupt symmetry, diminishing the ability to leverage it effectively.

Symmetry breaking also occurs in equivariant reinforcement learning based on group-invariant MDP (Section \ref{rl}). Group-invariant MDP assumes group-invariant reward functions and transition probabilities; however, these can be corrupted by factors such as the kinematic constraints of a robotic manipulator.


==> Old_2024_1130/Section7_Conclusions.tex <==
\JS{TBD}


==> Old_2024_1130/Section_buffer.tex <==
\subsection{Group Equivariant Neural Networks}\label{genn}
Convolutional neural networks are advantageous due to their translation-equivariant property. However, these equivariant properties are not guaranteed for other geometric symmetries, such as rotation or reflection. To address this limitation and extend CNNs to a broader range of symmetries, Group-equivariant Convolution Neural Networks (G-CNNs)\cite{cohen2016group} are proposed. They introduce the group equivariant convolution layer $\Phi: X \to Y$, which satisfies the condition $\Phi(\rho_X(g) \cdot x)=\rho_Y(g) \cdot \Phi(x)$, where $x \in X$, $y \in Y$. Here $\rho_X(g)$ and $\rho_Y(g)$ are group representations of the group $G$, satisfying $\rho(gh)=\rho(g)\rho(h)$, $\forall g, h \in G$. The convolution (i.e., correlation) in G-CNNs can be divided into the lifting convolution, which is the first layer convolution, and the full Group convolution (G-convolution). Lifting and full G-convolution can be represented as follows:
% \JS{We use $\rho(g)$ for the group representation, so please change accordingly, but it seems that the other also needs to be unified. What we should use is actually define space, $x \in X$, $y \in Y$, and use notation $\rho_X(g)$, $\rho_Y(g)$, with $\Phi: X \to Y$. In this notation, $\rho_X(g)$ is representation of group element $g$ acting on the set $X$.} \HA{Revised all the notation correctly.}
%
\[
\begin{split}
    y(g) &= \sum_{x \in X} \W (g^{-1} \circoo x) f(x), \quad 
    \text{Lifting convolution} \\
    y(g) &= \sum_{g \in G} \W (g^{-1} \circoo g) f(g), \quad 
    \text{Full G-convolution} \\
\end{split}
\]
%
Where $\W$ and $f$ are kernels and feature maps, respectively. In the case of G-CNNs, the process of lifting correlations results in high-dimensional feature maps, which increases the computational cost and makes it challenging to handle groups with high dimensions.
% \JS{what is ``large'' group? The meaning is very unclear. Is the large for computational power or a number of dimensions?} 
% \HA{Revised clearly.} 
% \JS{Too long sentence and hard to understand->} \HA{Revised for easy understanding, more details will be updated.} 
To address this issue, Steerable CNNs \cite{cohen2016steerable} utilize the fact that the space of the feature map is a vector space. They do not use lifting correlations, instead using kernels as linear maps between the input features and output features. To ensure that the output feature is steerable, the kernels are designed with the constraint such that $\rho_{out}(g) \W = \W \rho_{in}(g)$. Since the equivariance constraint is linear in $\W$, the kernel space forms a vector space as well.

G-CNNs and Steerable CNNs introduced equivariant neural networks for discrete groups in two-dimensional space. 
% \JS{Does steerable CNN also assume discrete group action in the 2D image?} \HA{They mentioned it is possible to develop in a more general setting, but for simplicity, they only consider steerability with respect to discrete groups.} 
In the field of robotics, however, many applications involve transformations in three-dimensional space, raising the necessity of network designs that can accurately represent transformations in three-dimensional space. Tensor Field Networks (TFNs) \cite{thomas2018tensor} address this issue using SE(3)-equivariant graph neural networks specifically designed for the SE(3) group. These networks can represent rigid body transformations in three-dimensional space with point clouds as input. \JS{We first keep the TFN and SE(3)-transformer here without much description. There are more details in the later sections, but let's merge them after reformatting.} The convolution process in TFN is formulated as:
\[
\begin{split}
{f}_{(out)}&( {x}|\dX)=\int{d^3 {y}} \; {W}( {x}- {y}) {f}_{(in)}( {y}|\dX)
\end{split}
\]

SE(3)-transformers \cite{se3t} enhance the TFN by incorporating self-attention mechanisms into their convolution process: 
\[
\begin{split}
    {f}_{(out),i}=\sum_{j\neq i}\alpha_{ij} {W}( {x}- {x}_j) {f}_{j}+\bigoplus_{n'}^{N'}\sum_{n=1}^{N} {W}_{(S)}^{n'n} {f}_{j}^{(n)}
\end{split}
\]
\JS{The details of the TFN and SE(3)-transformer will be elaborated in the later section after introducing the required concepts.}

